Inverse Kinematics for Serial Kinematic Chains via Sum of Squares Optimization

Inverse kinematics is a fundamental problem for articulated robots: fast and accurate algorithms are needed for translating task-related workspace constraints and goals into feasible joint configurations. In general, inverse kinematics for serial kinematic chains is a difficult nonlinear problem, for which closed form solutions cannot be easily obtained. Therefore, computationally efficient numerical methods that can be adapted to a general class of manipulators are of great importance. % to motion planning and workspace generation tasks. In this paper, we use convex optimization techniques to solve the inverse kinematics problem with joint limit constraints for highly redundant serial kinematic chains with spherical joints in two and three dimensions. This is accomplished through a novel formulation of inverse kinematics as a nearest point problem, and with a fast sum of squares solver that exploits the sparsity of kinematic constraints for serial manipulators. Our method has the advantages of post-hoc certification of global optimality and a runtime that scales polynomialy with the number of degrees of freedom. Additionally, we prove that our convex relaxation leads to a globally optimal solution when certain conditions are met, and demonstrate empirically that these conditions are common and represent many practical instances. Finally, we provide an open source implementation of our algorithm.

==> macros.tex <==
% Matt's additions
% Norms
\newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\frob}[1]{\|#1\|_{\scriptscriptstyle F}}

% Bold for matrix/vector variables
\newcommand{\mbf}[1]{\mathbf{#1}}
%\newcommand{\ones}[1]{\mathbf{1}_{#1}}
%\newcommand{\vect}[1]{\text{vec}(#1)}

\newcommand{\GG}{\mathcal{G}}
\newcommand{\GGi}{\mathcal{G}_{\normalfont\text{init}}}
\newcommand{\LLi}{\mathbf{L}_{\normalfont\text{init}}}
\newcommand{\Hgraph}{\mathcal{H}}
\newcommand{\GGQ}{\mathcal{G}_{[\mathcal{Q}]}}
\newcommand{\OPT}{\mathsf{OPT}}
\newcommand{\opt}{\mathsf{opt}}
\newcommand{\GRD}{{\normalfont\text{greedy}}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\esp}{$\mathrm{ESP}$}
\newcommand{\desp}{${\mathrm{ESP}^\ast}$}
\newcommand{\GGc}{{G}^\circ}
\newcommand{\EEc}{{E}^\circ}
\newcommand{\EEi}{{\EE}_{\normalfont\text{init}}}
\newcommand{\rvp}{\mathbf{r_\mathrm{vp}}}
\newcommand{\Jvp}{\mathbf{J_\mathrm{vp}}}
\newcommand{\JvpK}{\mathbf{J_\mathrm{vp}^\mathrm{K}}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\T}{{T}}
\newcommand{\K}{{K}}
%\newcommand{\EE}{{\large\mathpzc{E}}}
\newcommand{\EE}{{\mathcal{E}}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\sss}{\mathbf{s}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\dd}{\mathbf{d}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\ff}{{f}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\LLo}{\mathbf{L}_\circ}
\newcommand{\KK}{\mathbf{C}}
\newcommand{\KKK}{\mathcal{K}}
\newcommand{\DD}{\mathbf{D}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\NN}{\mathbf{N}}
\newcommand{\PP}{\mathbf{P}}
\newcommand{\ES}{\mathbf{S}}
\newcommand{\HH}{\mathbf{H}}
\newcommand{\cHH}{\mathcal{H}}
\newcommand{\cSS}{\mathcal{S}}
\newcommand{\bHH}{\tilde{\mathbf{H}}}
\newcommand{\bKs}{\bHH_1^\dagger}
\newcommand{\bJJ}{\tilde{\mathbf{J}}}
\newcommand{\WW}{\mathbf{W}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\brr}{\tilde{\mathbf{r}}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\bzz}{\tilde{\mathbf{z}}}
\newcommand{\ww}{\boldsymbol\epsilon}
\newcommand{\hh}{\mathbf{h}}
\newcommand{\pp}{\mathbf{p}}
\newcommand{\ppp}{\boldsymbol\pi}
\newcommand{\AAA}{\mathbf{A}}
\newcommand{\AAAtop}{\AAA^{\hspace{-0.1cm}\top}}
\newcommand{\AAo}{\mathbf{A}_\circ}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Aintra}{\mathcal{A}_\text{\normalfont intra}}
\newcommand{\Ainit}{\mathcal{A}_\text{\normalfont init}}
\newcommand{\Ainter}{\mathcal{A}_\text{\normalfont inter}}
\newcommand{\Mintra}{\mathcal{M}_\text{\normalfont intra}}
\newcommand{\Minter}{\mathcal{M}_\text{\normalfont inter}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\aaa}{\mathbf{a}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\BB}{\mathbf{A}_\text{odo}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\II}{\mathbf{I}}
\newcommand{\RR}{\mathbf{R}}
\newcommand{\CC}{\boldsymbol\Sigma}
\newcommand{\CCC}{\mathcal{C}}
\newcommand{\QQ}{\mathbf{Q}}
\newcommand{\cRR}{\mathbf{\Gamma}}
\newcommand{\cQQ}{\mathcal{Q}}
\newcommand{\tSS}{\mathbf{S}}
\newcommand{\tRR}{\tilde{\mathbf{R}}}
\newcommand{\OO}{{\Omega}}
\newcommand{\DDD}{\boldsymbol{\Delta}}
\newcommand{\trr}{\mathbf{\tilde{\rr}}}
\newcommand{\thth}{{\boldsymbol\theta}}
\newcommand{\mumu}{{\boldsymbol\mu}}
\newcommand{\bRR}{\mathbf{\bar{{R}}}}
\newcommand{\tJJ}{\mathbf{\tilde{J}}}
\newcommand{\JJ}{\mathbf{{J}}}
\newcommand{\Zcal}{{\mathcal{Z}}}
\newcommand{\III}{\mathkk{I}}
\newcommand{\bII}{\bar{\mathbf{\mathcal{I}}}}
%\newcommand{\logtree}{\mathsf{LogTree}_{n,w}}
\newcommand{\logtree}{\tau_{n,w}}
%\newcommand{\tree}{\mathsf{Tree}_{n,w}}
\newcommand{\tree}{t_{n,w}}
\newcommand{\logTG}{\Phi_{w}}
\newcommand{\logtreeu}{\mathsf{Log\,Tree}_{n}}
\newcommand{\treeu}{\mathsf{tree}_{n}}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\newcommand{\HHH}{\mathbfcal{H}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\ksucc}{\hspace{-0.1cm}\succ\hspace{-0.1cm}}
\newcommand{\ksucceq}{\hspace{-0.1cm}\succeq\hspace{-0.1cm}}
\newcommand{\ifff}{if and only if}
\newcommand{\RE}{\mathrm{RE}}
\newcommand{\Cov}{\mathbb{C}\mathrm{ov}}
\newcommand{\Inf}{\mathkk{I}}
\newcommand{\np}{n_p}
\newcommand{\nf}{n_f}
\newcommand{\PPP}{\mathbf{\Pi}}
\newcommand{\AAAw}{\mathbf{A}^{\hskip-0.05cm w}}
\newcommand{\AAAwp}{\mathbf{A}^{\hskip-0.05cm w_p}}
\newcommand{\LLw}{\mathbf{L}^{\hskip-0.05cm w}}
\newcommand{\LLwp}{\mathbf{L}^{\hskip-0.05cm w_p}}
\newcommand{\LLwt}{\mathbf{L}^{\hskip-0.05cm w_\theta}}

\newcommand{\gsq}{\textcolor{green}{$\bullet$}}
\newcommand{\ysq}{\textcolor{yellow}{$\bullet$}}
\newcommand{\rsq}{\textcolor{red}{$\bullet$}}
\newcommand{\cg}{\cellcolor{green!10!white}}
\newcommand{\crr}{\cellcolor{red!10!white}}


\DeclareMathOperator{\wrap}{wrap}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\Null}{null}
\DeclareMathOperator*{\range}{range}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\diag}{diag}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}

\newcommand{\Plus}{\texttt{\normalfont +}}
\newcommand{\Minus}{\texttt{-}}
\newcommand{\Cplus}{\CCC^\Plus}
\newcommand{\Cminus}{\CCC^\Minus}
\newcommand{\espPlus}{\mathrm{ESP}^\Plus}
\newcommand{\respPlus}{\mathrm{RESP}^\Plus}
\newcommand{\despPlus}{\mathrm{ESP}^\ast}
\newcommand{\espMinus}{\mathrm{ESP}^\Minus}




\newcommand{\globalmin}{\textsf{\small\bfseries Global Min}}
\newcommand{\localmin}{\textsf{\small\bfseries Local Min}}
\newcommand{\notconverged}{\textsf{\small\bfseries Not Converged}}

\newcommand\Tstrut{\rule{0pt}{2.2ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\newcommand{\ggo}{\texttt{g2o}}
\newcommand{\cholmod}{{CHOLMOD}}

\newcommand*{\matminus}{%
  \leavevmode
  \hphantom{0}%
  \llap{%
    \settowidth{\dimen0 }{$0$}%
    \resizebox{1.1\dimen0 }{\height}{$-$}%
  }%
}


\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\kscan}{k_\textsf{register}}
\newcommand{\kfound}{k_\textsf{found}}
\newcommand{\kcomm}{k_\text{\tiny\faWifi}}
\newcommand{\fcomm}{f_\text{\tiny\faWifi}}
\newcommand{\kcomp}{k_\text{\tiny\faLaptop}}
\newcommand{\fcomp}{f_\text{\tiny\faBalanceScale}}
\newcommand{\Gex}{\GG}
\newcommand{\Lcaltotal}{\mathcal{L}_\textsf{total}}
%\let\oldsim\sim
%\renewcommand{\sim}{\overset{\Lcal}{\oldsim}}

\newcommand\kk[1]{\textcolor{blue!80!gray}{\textbf{KK: }\ul{#1}}}
% for Matt
\newcommand\mg[1]{\textcolor{magenta!70!yellow}{\textbf{MG: }\ul{#1}}}


\newcommand{\bipgraph}[2]{%
    \begin{tikzpicture}[every node/.style={circle,fill,scale=0.4,draw}]
    \foreach \xitem in {1,2,...,#1}
    {%
    % first set
    \node at (\xitem,0) (a\xitem) {};
    % second set
    \node at (\xitem,1) (b\xitem) {};   
    }%

    % connections
    \foreach \x [count=\xi] in {#2}
    {% 
    \foreach \tritem in \x % <-- Here no braces to make it a foreach list also not \xi but \x
    \draw(a\xi) -- (b\tritem);
    }
    \end{tikzpicture}  
}

	\newcommand\DoubleLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,line width=0.25mm,black] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	  \draw[->,line width=0.25mm,black] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	}
	\newcommand\DoubleLineOneDirectional[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[->,line width=0.75mm,black] ($(h1)!#1!90:(h2)$)  to ["#4"]
	  ($(h2)!#1!-90:(h1)$);
	  \draw[->,very thick,densely dashed,black!50!white, bend right=15] ($(h1)!#1!-100:(h2)$) to
	  ["#5" '] ($(h2)!#1!100:(h1)$);
	}
	\newcommand\xDoubleDashedLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[->,very thick,densely dashed,black!50!white,bend left=90] ($(h1)!#1!90:(h2)$)  to ["#4"]
	  ($(h2)!#1!-90:(h1)$);
	  \draw[<-,very thick,densely dashed,black!50!white, bend right=80] ($(h1)!#1!-100:(h2)$) to
	  ["#5" '] ($(h2)!#1!100:(h1)$);
	}
	\newcommand\DoubleDashedLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,very thick,black!50!white,densely
	  dashed,sloped,anchor=south] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	  \draw[->,very thick,  black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	}
	\newcommand\DoubleDashedLineRev[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,very thick,  black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	  \draw[->,very thick,black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	}



\definecolor{kkGreen}{RGB}{201,232,206}
\definecolor{kkRed}{RGB}{255,196,215}
\definecolor{kkBlue}{RGB}{214,226,255}


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Andrasfai.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/NamedGraphs/doc/NamedGraphs-main.tex
\newpage\section{Andrasfai graph}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                               Andrasfai
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grAndrasfai}{\oarg{options}\var{$k$}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/AndrasfaiGraph.html} 

\emph{The k-Andrásfai graph is a circulant graph on $3k-1$ nodes whose indices are given by the integers 1,\dots,$3k-1$  that are congruent to 1 (mod 3).
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
}

\medskip
\end{NewMacroBox}

\bigskip

\subsection{\tkzname{Andrásfai graph : k=7, order 20}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.7]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{7}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Andrásfai graph :  k=8, order 23}}

\bigskip\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{8}
  \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage
\subsection{\tkzname{Andrásfai graph :  k=9, order 26}}

\bigskip\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{9}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Balaban.tex <==
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage\section{Balaban}\label{balaban}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––   Balaban's graph  ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grBalaban}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/Balaban10-Cage.html} 

\emph{The Balaban 10-cage is one of the three(3,10)-cage graphs (Read 1998, p. 272). The Balaban (3,10)-cage was the first known example of a 10-cage (Balaban 1973; Pisanski 2001). Embeddings of all three possible (3,10)-cages (the others being the Harries graph and Harries-Wong graph) are given by Pisanski et al. (2001). Several embeddings are illustrated below, with the three rightmost being given by Pisanski and Randić (2000)
It is a Hamiltonian graph and has  Hamiltonian cycles. It has 1003 distinct LCF notations, with four of length two (illustrated above) and 999 of length 1.
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
}
\end{NewMacroBox}

\subsection{\tkzname{Balaban graph : first form}}
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}[scale=.6]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
 \grBalaban[form=1,RA=7,RB=3,RC=3]
 \end{tikzpicture}
\end{tkzexample}

\end{center}


\vfill\newpage
\subsection{\tkzname{Balaban graph : second form}}
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{gray}{blue!50}
 \grBalaban[form=2,RA=7,RB=7,RC=4,RD=2.5]
 \end{tikzpicture}
\end{tkzexample}

\end{center}

\vfill\newpage
\subsection{\tkzname{Balaban graph : third form} }
\begin{center}
 \begin{tkzexample}[vbox]
  \begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{brown}{orange}
  \grBalaban[form=3,RA=7,RB=6.5,RC=5.6,RD=5.6,RE=4.6]
  \end{tikzpicture}
 \end{tkzexample}

\end{center}


\vfill\newpage

\subsection{\tkzname{Balaban graph : Balaban 11-Cage}}


The Balaban 11-cage is the unique 11-cage graph, discovered by Balaban (1973) and proven unique by McKay and Myrvold (2003). It has 112 vertices, 168 edges, girth 11 (by definition),  diameter 8 and chromatic number 3.


\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}[scale=.7]
  \renewcommand*{\VertexInnerSep}{3pt}
  \renewcommand*{\VertexLineWidth}{0.4pt}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red!50}{blue!50!black}
 \grLCF[Math,RA=7]{%
 44,26,-47,-15,35,-39,11,-27,38,-37,43,14,28,51,-29,-16,41,-11,%
 -26,15,22,-51,-35,36,52,-14,-33,-26,-46,52,26,16,43,33,-15,%
  17,-53,23,-42,-35,-28,30,-22, 45,-44,16,-38,-16,50,-55,20,28,%
  -17,-43,47, 34,-26,-41,11,-36,-23,-16,41,17,-51,26,-33,47,17,%
  -11,-20 ,-30,21,29,36,-43,-52,10,39,-28,-17,-52,51,26,37,-17,%
  10,-10,-45,-34,17,-26,27,-21,46,53,-10,29,-50,35,15,-47,-29,-41,%
  26,33,55,-17,42,-26,-36,16}{1}
 \end{tikzpicture}
\end{tkzexample}

\end{center}




\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Bipartite.tex <==
\newpage\section{Complete BiPartite Graph}\label{bipart}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––  Complete BiPartite graph  ––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grCompleteBipartite}{\oarg{options}\var{$p$}\var{$q$}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/CompleteBipartiteGraph.html}

\emph{A complete bipartite graph is a bipartite graph (i.e., a set of graph vertices decomposed into two disjoint sets such that no two graph vertices within the same set are adjacent) such that every pair of graph vertices in the two sets are adjacent. If there are $p$ and $q$ graph vertices in the two sets, the complete bipartite graph (sometimes also called a complete bigraph) is denoted $K_{p,q}$ . The below figures show $K_{3,2}$ and $K_{3,3}$. $K_{3,3}$ is also known as the utility graph (and the circulant graph $Ci_{1,3}(6)$), and is the unique 4-cage graph.} 
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Complete_bipartite_graph}

\emph{In the mathematical field of graph theory, a complete bipartite graph or biclique is a special kind of bipartite graph where every vertex of the first set is connected to every vertex of the second set. the graph $K_{1,3}$ is also called a claw.}
\end{NewMacroBox}

\subsection{\tkzname{Complete bipartite graphs $K_{3,2}$ and $K_{3,3}$} }
 %G=LCF_graph(6,[3,-3],3)   
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \grCompleteBipartite[RA=2,RB=2,RS=3]{3}{2}
\end{tikzpicture}\hspace*{2cm}
\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \grCompleteBipartite[RA=2,RB=2,RS=3]{3}{3}
 \end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{\tkzname{Complete bipartite graphs $K_{3,5}$}}
\begin{center}
\begin{tkzexample}[vbox] 
\begin{tikzpicture}[scale=1.5]
  \GraphInit[vstyle=Art]
  \grCompleteBipartite[RA=3,RB=2,RS=5]{3}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center} 

\vfill\newpage

\subsection{\tkzname{Complete bipartite graph : $K_{18,18}$ }}

The complete bipartite graph  illustrated below plays an important role in the novel Foucault's Pendulum by Umberto Eco.

\href{http://mathworld.wolfram.com/CycleGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\vfill
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90,scale=1.4]
  \GraphInit[vstyle=Art]
  \grCompleteBipartite[RA=0.5,RB=0.5,RS=9]{18}{18}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill\newpage
A complete bipartite graph $K_{n,n}$ is a circulant graph (if the order is equal to $2n$ then $L=1,3,\dots,n$).
The code is on the next page

\bigskip
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{6}{1,3}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{8}{1,3}
\end{tikzpicture}

\vspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{10}{1,3,5}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{12}{1,3,5}
\end{tikzpicture}

\vspace*{12pt}
\begin{tikzpicture}
 \GraphInit[vstyle=Art]
 \grCirculant[RA=3]{14}{1,3,5,7}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
 \grCirculant[RA=3]{16}{1,3,5,7}
\end{tikzpicture} 

\vfill\newpage
\begin{tkzexample}[code only]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{6}{1,3}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{8}{1,3}
\end{tikzpicture}

\vspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{10}{1,3,5}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCirculant[RA=3]{12}{1,3,5}
\end{tikzpicture}

\vspace*{12pt}
\begin{tikzpicture}
       \GraphInit[vstyle=Art]
\grCirculant[RA=3]{14}{1,3,5,7}
\end{tikzpicture}\hspace*{12pt} 
\begin{tikzpicture}
       \GraphInit[vstyle=Art]
\grCirculant[RA=3]{16}{1,3,5,7}
\end{tikzpicture}
\end{tkzexample}


\endinput



==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Bull.tex <==
\newpage\section{Bull}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                               Bull
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
The bull graph, 5 vertices, 5 edges, resembles to the head of a bull if drawn properly. 
The bull graph is a simple graph on 5 nodes and 5 edges whose name derives from its resemblance to a schematic illustration of a bull 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[node distance=4cm]
  \GraphInit[vstyle=Shade]
  \Vertex{a0}
  \NOEA(a0){a2}
  \NOEA(a2){a4}
  \NOWE(a0){a1}
  \NOWE(a1){a3}
  \Edges(a0,a1,a3)
  \Edges(a0,a2,a4)
  \Edge(a1)(a2)
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Cage.tex <==
\newpage\section{Cage}\label{cage}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   Cage                –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{Cage Graphs}{}

\medskip
From Wikipedia  \url{http://en.wikipedia.org/wiki/Cage_(graph_theory)}\\
\emph{In the mathematical area of graph theory, a cage is a regular graph that has as few vertices as possible for its girth.\\
Formally, an $(r,g)$-graph is defined to be a graph in which each vertex has exactly $r$ neighbors, and in which the shortest cycle has length exactly $g$. It is known that an $(r,g)$-graph exists for any combination of $r \geq 2$ and $g \geq 3$. An $(r,g)$-cage is an $(r,g)$-graph with the fewest possible number of vertices, among all $(r,g)$-graphs.}

\medskip
From MathWorld \url{http://mathworld.wolfram.com/CageGraph.html}\\
\emph{A $(r,g)$-cage graph is a $v$-regular graph of girth $g$ having the minimum possible number of nodes. When $v$ is not explicitly stated, the term "$g$-cage" generally refers to a $(3,g)$-cage.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
Examples :

\medskip
\begin{tabular}{ll}
  \bottomrule
$(r,g)$ & Names                                                     \\
\midrule
$(3,3)$     & complete graph $K_4$                                  \\
$(3,4)$     & complete bipartite graph $K_{3,3}$ Utility Graph\ref{bipart} \\
$(3,5)$     & Petersen graph \ref{petersen}                          \\
$(3,6)$     & Heawood graph  \ref{heawood}                           \\
$(3,7)$     & McGee graph \ref{mcgee}                                \\
$(3,8)$     & Levi graph \ref{levi}                                  \\
$(3,10)$    & Balaban 10-cage     \ref{balaban}                      \\
$(3,11)$    & Balaban 11-cage     \ref{balaban}                      \\
$(3,12)$    & Tutte 12-cage                                          \\
$(4,3)$     & complete graph $K_5$                                   \\
$(4,4)$     & complete bipartite graph $K_{4,4}$ \ref{bipart}          \\
$(4,5)$     & Robertson graph\ref{robertson}                         \\
$(4,6)$     & Wong (1982)\ref{wong}                                  \\
\end{tabular}
\end{NewMacroBox}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Chvatal.tex <==
\newpage\section{Chvatal}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grChvatal}{\oarg{options}}

\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Václav_Chvátal} 

\emph{Chvátal first learned of graph theory in 1964, on finding a book by Claude Berge in a Pilsen bookstore, and his first mathematical publication, at the age of 19, concerned directed graphs that cannot be mapped to themselves by any nontrivial graph homomorphism.\hfill\break
Gallery Theorem—which determines the number of guards required to survey the 
walls of a polygonal art gallery (and has prompted much research), and constructed the smallest triangle-free 4-chromatic 4-regular graph, a beautiful graph now known as the Chvatal graph.}


\medskip
From MathWord : \url{http://mathworld.wolfram.com/ChvatalGraph.html}  

\emph{The Chvátal graph is a quartic graph on 12 nodes and 24 edges. It has chromatic number 4, and girth 4.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Chvátal graph is implemented in \tkzname{tkz-berge} as \tkzcname{grChvatal} with three forms.
\end{NewMacroBox}

\medskip
\subsection{\tkzname{Chvatal  graph I}}

\bigskip

\begin{center}
  \begin{tkzexample}[vbox]
    \begin{tikzpicture}[scale=.7]
       \GraphInit[vstyle=Shade]
       \SetVertexNoLabel
       \SetGraphShadeColor{blue!50!black}{blue}{gray} 
       \grChvatal[RA=6,RB=2]
    \end{tikzpicture}  
  \end{tkzexample}

\end{center}

\vfill\newpage
\subsection{\tkzname{Chvatal  graph II}}

\bigskip
\begin{center}
  \begin{tkzexample}[vbox]
    \begin{tikzpicture}
      \GraphInit[vstyle=Art]
      \SetGraphArtColor{blue!50!black}{gray}
      \grChvatal[form=2,RA=7,RB=4,RC=1.4] 
    \end{tikzpicture}
  \end{tkzexample}

\end{center}


\vfill\newpage
\subsection{\tkzname{Chvatal  graph III}}

\bigskip
\begin{center}
  \begin{tkzexample}[vbox]
    \begin{tikzpicture}
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{blue!50!black}{gray}  
     \grChvatal[form=3,RA=7] 
    \end{tikzpicture}
  \end{tkzexample}

\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Cocktail_Party.tex <==
\newpage\section{Cocktail Party graph}\label{cocktail}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––   Cocktail Party  –––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grCocktailParty}{\oarg{options}\var{integer}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/CocktailPartyGraph.html}  

\emph{The cocktail party graph of order , also called the hyperoctahedral graph (Biggs 1993, p. 17) is the graph consisting of two rows of paired nodes in which all nodes but the paired ones are connected with a graph edge. It is the graph complement of the ladder graph , and the dual graph of the hypercube graph.\hfill\break
This graph arises in the handshake problem. It is a complete n-partite graph that is denoted  by Brouwer et al. (1989, pp. 222-223), and is distance-transitive, and hence also distance-regular.\hfill\break
The cocktail party graph of order  is isomorphic to the circulant graph.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Chvátal graph is implemented in \tkzname{tkz-berge} as \tkzcname{grCocktailParty} with two forms.
\end{NewMacroBox}

\subsection{\tkzname{Cocktail Party graph form 1 }}
\tikzstyle{VertexStyle}   = [shape          = circle,
                             shading         = ball,%
                             ball color      = green,%
                             minimum size    = 24pt,%
                             draw]
\SetVertexMath
\tikzstyle{EdgeStyle}     = [thick,%
                             double          = orange,%
                             double distance = 1pt] 
\begin{center}
   \begin{tkzexample}[vbox]
    \begin{tikzpicture}
       \grCocktailParty[RA=3,RS=5]{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Cocktail Party graph form 2 }}

\vspace*{2cm}
\begin{center}
   \begin{tkzexample}[vbox]
   \begin{tikzpicture}
      \grCocktailParty[form=2,RA=4,RS=6]{4}
     \end{tikzpicture}
\end{tkzexample} 
\end{center}
\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Coxeter.tex <==
\newpage\section{Coxeter}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Coxeter  ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
From MathWorld : \url{http://mathworld.wolfram.com/CoxeterGraph.html}

The Coxeter graph is a nonhamiltonian cubic symmetric graph on 28 vertices and 42 edges.


\subsection{\tkzname{Coxeter graph I}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90,scale=1]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{magenta}{gray}
  \grCycle[RA=5,prefix=a]{7}
  \begin{scope}[rotate=-20]\grEmptyCycle[RA=4,prefix=b]{7}\end{scope}
  \grCirculant[RA=3,prefix=c]{7}{2}
  \grCirculant[RA=1.4,prefix=d]{7}{3}
  \EdgeIdentity{a}{b}{7} 
  \EdgeIdentity{b}{c}{7} 
  \EdgeIdentity{b}{d}{7} 
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage
\subsection{\tkzname{Coxeter graph II}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{magenta}{gray}
  \grCycle[RA=7,prefix=b]{24}
  \grEmptyStar[RA=3,prefix=a]{4}
  \EdgeDoubleMod{a}{3}{0}{1}{b}{24}{0}{8}{2}
  \EdgeDoubleMod{a}{3}{0}{1}{b}{24}{7}{8}{2}
  \EdgeDoubleMod{a}{3}{0}{1}{b}{24}{18}{8}{2}
  \EdgeDoubleMod{a}{4}{3}{0}{b}{24}{22}{8}{2}
  \EdgeInGraphMod*{b}{24}{6}{5}{8}
  \EdgeInGraphMod*{b}{24}{11}{1}{8}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage

\subsection{\tkzname{Coxeter graph III}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{magenta}{gray}
  \grCycle[RA=7,prefix=c]{7}
  \grEmptyCycle[RA=6,prefix=b]{7}
  \begin{scope}[rotate=12.85]\grEmptyCycle[RA=5,prefix=a]{14}\end{scope}
  \EdgeIdentity{b}{c}{7}
  \EdgeDoubleMod{b}{7}{0}{1}{a}{14}{0}{2}{6}
  \EdgeDoubleMod{b}{7}{0}{1}{a}{14}{13}{2}{6}
  \EdgeInGraphModLoop{a}{14}{4}{0}{0}
  \EdgeInGraphModLoop{a}{14}{6}{1}{1}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   Tutte-Coxeter graph    ––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\vfill\newpage
\subsection{\tkzname{Tutte-Coxeter graph I}}

\tikzstyle{VertexStyle} = [very thin,draw,
                           shape                =  circle,
                           color                =  white,
                           fill                 =  black,
                           inner sep            =  0pt,
                           minimum size         =  18pt]
\tikzstyle{EdgeStyle}   = [thick,
                           double               = brown,
                           double distance      = 1pt]

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=3]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{blue}{cyan}
  \begin{scope}[rotate=5]\grCycle[RA=2.5,prefix=a]{10}\end{scope}
  \begin{scope}[rotate=-10]\grCirculant[RA=1.8,prefix=b]{10}{5}\end{scope}
  \begin{scope}[rotate=36]\grCirculant[RA=1.1,prefix=c]{10}{3}\end{scope}
  \EdgeIdentity{a}{b}{10} 
  \EdgeIdentity{b}{c}{10} 
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
% 

\vfill\newpage
\subsection{\tkzname{Tutte-Coxeter graph II}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{blue}{darkgray}
     \grLCF[RA=7]{-13,-9,7,-7,9,13}{5}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Crown.tex <==
\newpage\section{Crown}\label{crown}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Crown    ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grCrown}{\oarg{options}\var{integer}}


\medskip
From MathWord : \url{http://mathworld.wolfram.com/CrownGraph.html}  

\emph{The Crown graph  for an integer  is the graph with vertex set
$\{x_0,x_1,\dots,x_{n-1},y_0,y_1,\dots,y_{n-1}\}$\hfill\break
and edge set \hfill\break
$\{(x_i,x_j): 0\leq i,j\leq n-1,i \not=j\}$.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Crown graph is implemented in \tkzname{tkz-berge} as \tkzcname{grCrown} with two forms.
\end{NewMacroBox}


\subsection{\tkzname{Crown graph form 1}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
\tikzstyle{VertexStyle}   = [shape           = circle,
                             shading         = ball,
                             ball color      = green,
                             minimum size    = 24pt,
                             draw]
\tikzstyle{EdgeStyle}     = [thick,
                             double          = orange,
                             double distance = 1pt] 
\SetVertexLabel\SetVertexMath   
\grCrown[RA=3,RS=6]{4}
 \end{tikzpicture}
\end{tkzexample} 

\end{center}

\vfill\newpage
\subsection{\tkzname{Crown graph form 2}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grCrown[form=2,RA=4,RS=6]{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-CubicSymmetric.tex <==
\newpage\section{Cubic Symmetric Graphs}
%<––––––––––––––––––––––––––––––––––––––––––––––––––--–––––––––––––––––––––––>
%<–––––––––––––––––––––––Cubic Symmetric Graphs     –––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
A cubic symmetric graph is a symmetric cubic (i.e., regular of order 3). Such graphs were first studied by Foster (1932). They have since been the subject of much interest and study. Since cubic graphs must have an even number of vertices, so must cubic symmetric graphs.

The circulant graph , is illustrated below.

\subsection{\tkzname{Cubic Symmetric Graph form 1}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
     \SetVertexNoLabel
     \grLCF[RA=6]{3,-3}{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage

\subsection{\tkzname{Cubic Symmetric Graph form 2}}

\vspace*{1cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
  \tikzstyle{VertexStyle} = [shape                =  circle,%
                             color                =  white,
                             fill                 =  black,
                             very thin,
                             inner sep            =  0pt,%
                             minimum size         =  18pt,
                             draw]
  \tikzstyle{EdgeStyle}   = [thick,%
                             double               = brown,%
                             double distance      = 1pt] 
  \grLCF[Math,RA=6]{3,-3}{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Desargues.tex <==
\newpage\section{Desargues}\label{desargues}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Desargues –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grDesargues}{\oarg{options}}

\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Desargues_graph} 

\emph{ In the mathematical field of graph theory, the Desargues graph is a 3-regular graph with 20 vertices and 30 edges, formed as the Levi graph of the Desargues configuration.The Desargues graph can also be formed as a double cover of the Petersen graph, as the generalized Petersen graph G(10,3), or as the bipartite Kneser graph $H_{5,2}$.}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/DesarguesGraph.html}  

\emph{ The Desargues graph is a cubic symmetric graph distance-regular graph on 20 vertices and 30 edges, illustrated above in several embeddings. It can be represented in LCF notation as  (Frucht 1976) and is isomorphic to the bipartite Kneser graph . It is the incidence graph of the Desargues configuration.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Desargues graph is implemented in \tkzname{tkz-berge} as \tkzcname{grDesargues} with two forms.
\end{NewMacroBox}


\tikzstyle{VertexStyle} = [shape                = circle,%
                           color                = white,
                           fill                 = black,
                           very thin,
                           inner sep            = 0pt,%
                           minimum size         = 18pt,
                           draw]
\tikzstyle{EdgeStyle}   = [thick,%
                           double               = brown,%
                           double distance      = 1pt]
\SetVertexMath
\subsection{\tkzname{The Desargues graph : form 1}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6]
    \grDesargues[Math,RA=6]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{The Desargues graph : form 2}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grDesargues[form=2,Math,RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage  
\subsection{The Desargues graph wth \tkzname{LCF notation}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
   \grLCF[Math,RA=6]{5,-5,9,-9}{5}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage  
\subsection{The Desargues graph with \tkzcname{grGeneralizedPetersen}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
  \tikzstyle{VertexStyle} = [shape                = circle,%
                             color                = white,
                             fill                 = black,
                             very thin,
                             inner sep            = 0pt,%
                             minimum size         = 18pt,
                             draw]
  \tikzstyle{EdgeStyle}    = [thick,%
                              double               = brown,%
                              double distance      = 1pt]  
  \grGeneralizedPetersen[Math,RA=6]{10}{3}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Doyle.tex <==
\newpage\section{Doyle}\label{doyle}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Doyle  ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grDoyle}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/DoyleGraph.html}  

\emph{The Doyle graph, sometimes also known as the Holt graph (Marušič et al. 2005), is the symmetric quartic graph on 27 nodes illustrated. It is a Symmetric Graph. Three embeddings are illustrated below.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Doyle graph is implemented in \tkzname{tkz-berge} as \tkzcname{grDoyle} with three forms.
\end{NewMacroBox}

\subsection{\tkzname{The Doyle graph : form 1}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6] 
  \GraphInit[vstyle=Shade]
  \SetGraphShadeColor{red}{Maroon}{fondpaille}  
  \SetVertexNoLabel  
  \grDoyle[RA=7,RB=5,RC=3]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{The Doyle graph : form 2}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetGraphShadeColor{red}{Magenta}{white} 
   \SetVertexNoLabel
   \grDoyle[form=2,RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{The Doyle graph : form 3}}
\begin{center}
 \begin{tkzexample}[vbox]
\begin{tikzpicture} 
  \SetGraphArtColor{red}{Magenta}{red}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel 
   \grDoyle[form=3,RA=7,RB=2]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage

\subsection{27 nodes but not isomorphic to the Doyle graph}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6] 
   \tikzstyle{VertexStyle} = [shape           = circle,
                              ball color      = gray!60,
                              minimum size    = 16pt,draw]
   \tikzstyle{EdgeStyle}   = [thick,color=black,%
                              double          = orange,%
                              double distance = 1pt] 
   \SetVertexNoLabel
   \grCycle[RA=7.5]{9}
   \grEmptyCycle[prefix=b,RA=5.5]{9}
   \grCirculant[prefix=c,RA=3.5]{9}{4}
   \EdgeIdentity{b}{c}{9}
   \EdgeMod{a}{c}{9}{1}
   \EdgeMod{a}{b}{9}{1}
   \EdgeInGraphMod{b}{9}{2}
   \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Dyck.tex <==
\newpage\section{Dyck graph}\label{dyck}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Nauru    ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grDick}{\oarg{options}} 
  
From Wikipedia \url{http://en.wikipedia.org/wiki/Dyck_graph}

\emph{In the mathematical field of graph theory, the Dyck graph is a 3-regular graph with 32 vertices and 48 edges, named after Walther von Dyck. It has chromatic number 2,  radius 5, diameter 5 and girth 6. It is also a 3-vertex-connected and a 3-edge-connected graph.
}

\medskip
From MathWorld \url{http://mathworld.wolfram.com/DyckGraph.html}

\emph{The Dyck graph is unique cubic symmetric graph on 32 nodes, illustrated below in one of embeddings.}       

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
\end{NewMacroBox} 

\subsection{\tkzname{Dyck graph}}

It can be represented in LCF notation as  $\big[5,-5,13,-13\big]^8$



\subsection{\tkzname{Dyck graph with LCF notation}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grLCF[RA=7]{5,-5,13,-13}{8}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Folkman.tex <==
\newpage\section{Folkman}\label{folkman}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Folkman            –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grFolkman}{\oarg{options}}

\medskip
From MathWorld : \url{http://mathworld.wolfram.com/FolkmanGraph.html}

\emph{The Folkman graph is a semisymmetric graph that has the minimum possible number of nodes 20.} 
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
\end{NewMacroBox}


\subsection{\tkzname{Folkman Graph LCF embedding}}
The code is

\begin{tkzexample}[code only]
\grLCF[RA=7]{5,-7,-7,5}{5}\end{tkzexample}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.8]
      \GraphInit[vstyle=Art]
      \SetGraphArtColor{blue}{darkgray}
      \grFolkman[RA=6]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage


\subsection{\tkzname{Folkman Graph embedding 1}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=45]% 
     \tikzstyle{VertexStyle} = [shape           = circle,
                                shading         = ball,
                                ball color      = gray!60,
                                inner sep       = 3pt,
                                draw]
     \tikzstyle{EdgeStyle}  = [thick,orange]
     \SetVertexNoLabel 
     \grCycle[prefix=a,RA=3]{4}%
     \grCycle[prefix=b,RA=4]{4}%
     \grCycle[prefix=c,RA=5]{4}%
     \grCycle[prefix=d,RA=6]{4}%
     \grCycle[prefix=e,RA=7]{4}%
     \foreach \r/\s/\t in {a/d/e,b/e/a,c/a/b,d/b/c,e/c/d}{%
        \Edges(\r0,\s1,\r2,\t3,\r0)
        }
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage

\subsection{\tkzname{Folkman Graph embedding 1 new code}}
{  \tikzstyle{VertexStyle} =[shape        = circle,%
                            shading       = ball,%
                            inner sep     = 4pt,%
                            draw]
  \tikzstyle{EdgeStyle}  = [thin,blue]

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
\begin{scope}[shift={(1,1)},rotate=45]\grEmptyPath[prefix=a,RA=1]{5}
  \end{scope}
\begin{scope}[shift={(-1,1)},rotate=135]\grEmptyPath[prefix=b,RA=1]{5}
  \end{scope}
\begin{scope}[shift={(-1,-1)},rotate=225]\grEmptyPath[prefix=c,RA=1]{5}
  \end{scope}
\begin{scope}[shift={(1,-1)},rotate=315]\grEmptyPath[prefix=d,RA=1]{5}
  \end{scope}
  \EdgeIdentity*{a}{b}{0,...,4}  \EdgeIdentity*{b}{c}{0,...,4}
  \EdgeIdentity*{c}{d}{0,...,4}  \EdgeIdentity*{d}{a}{0,...,4}
  \EdgeDoubleMod{a}{5}{0}{1}{b}{5}{3}{1}{1}
  \EdgeDoubleMod{a}{5}{2}{1}{b}{5}{0}{1}{2}
  \EdgeDoubleMod{a}{5}{1}{1}{d}{5}{0}{1}{3}
  \EdgeDoubleMod{c}{5}{2}{1}{b}{5}{0}{1}{2}
  \EdgeDoubleMod{c}{5}{0}{1}{b}{5}{3}{1}{1}
  \EdgeDoubleMod{c}{5}{1}{1}{d}{5}{0}{1}{3}
  \Edges(a0,d4,c0)
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
}
\vfill\newpage

\subsection{\tkzname{Folkman Graph embedding 3}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.8]
   \SetVertexNoLabel
   \tikzstyle{VertexStyle} = [shape           = circle,
                              shading         = ball,
                              ball color      = gray!60,
                              inner sep       = 3pt,
                              draw]
   \tikzstyle{EdgeStyle}    = [thick,orange]  
   \grEmptyCycle[prefix=a,RA=1.85]{5} \grEmptyCycle[prefix=b,RA=3.7]{5}
   \grCycle[prefix=c,RA=6]{10}
   \EdgeDoubleMod{a}{5}{0}{1}{b}{5}{1}{1}{4}
   \EdgeDoubleMod{a}{5}{0}{1}{b}{5}{4}{1}{4}
   \EdgeDoubleMod{b}{5}{0}{1}{c}{10}{9}{2}{4}
   \EdgeDoubleMod{b}{5}{0}{1}{c}{10}{1}{2}{4}
   \EdgeDoubleMod{a}{5}{0}{1}{c}{10}{8}{2}{4}
   \EdgeDoubleMod{a}{5}{0}{1}{c}{10}{2}{2}{4}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Foster.tex <==
\newpage\section{Foster}\label{foster}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Foster            –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grFoster}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/FosterGraph.html}

\emph{The Foster graph is a graph on 90 vertices and 135 arcs.  It has a unique order-15 LCF notations.}

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 
 \end{NewMacroBox}

\subsection{\tkzname{Foster graph}}

The macros is based on 

\begin{tkzexample}[code only]
\grLCF[Math,RA=7]{17, -9, 37, -37, 9, -17}{15}\end{tkzexample}

\vspace*{1cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6]
  \renewcommand*{\VertexInnerSep}{2pt}
  \renewcommand*{\EdgeLineWidth}{0.5pt}
  \GraphInit[vstyle=Art] 
  \tikzset{VertexStyle/.append style={minimum size=2pt}} 
  \SetGraphColor{red}{blue}
  \grLCF[Math,RA=6]{17, -9, 37, -37, 9, -17}{15}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Franklin.tex <==
\newpage\section{Franklin}\label{franklin}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Franklin  ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grFranklin}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/FranklinGraph.html}  

\emph{The Franklin graph is the 12-vertex cubic graph shown above whose embedding on the Klein bottle divides it into regions having a minimal coloring using six colors, thus providing the sole counterexample to the Heawood conjecture.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 

\medskip
The Franklin graph is implemented in \tkzname{tkz-berge} as \tkzcname{grFranklin}.
\end{NewMacroBox}

\tikzstyle{VertexStyle} = [shape                =  circle,%
                           color                =  white,
                           fill                 =  black,
                           very thin,
                           inner sep            =  0pt,%
                           minimum size         =  18pt,
                           draw]
\tikzstyle{EdgeStyle}    = [thick,%
                            double               = brown,%
                            double distance      = 1pt]
\newcounter{tempi}\setcounter{tempi}{0}

\subsection{\tkzname{The Franklin graph : embedding 1}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.7]
   \grFranklin[Math,RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{The Franklin graph : embedding 2}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grCycle[Math,RA=4,prefix=a]{6}
  \grCycle[Math,RA=6,prefix=b]{6}
  \foreach \x in {0,...,5}{%
    \ifthenelse{\isodd{\x}}{%
     \pgfmathsetcounter{tempi}{\x-1}}{%
     \pgfmathsetcounter{tempi}{\x+1}}
     \Edge(a\x)(b\thetempi)
}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage
\subsection{\tkzname{The Franklin graph : with LCF notation embedding 3}}

\space*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grLCF[Math,RA=7]{-5,-3,3,5}{3}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Gray.tex <==
\newpage\section{Gray}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   Gray                –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
From MathWorld :\url{ http://mathworld.wolfram.com/GrayGraph.html}

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 
           
           
The Gray graph is a cubic semisymmetric graph on 54 vertices. It was discovered by Marion C. Gray in 1932, and was first published by Bouwer (1968). Malnic et al. (2004) showed that the Gray graph is indeed the smallest possible cubic semisymmetric graph.

It is the incidence graph of the Gray configuration.

The Gray graph has a single order-9 LCF Notation  and five distinct order-1 LCF notations.

The Gray graph has girth 8, graph diameter 6

It can be   represented in LCF notation as  $\big[-25,7,-7,13,-13,25\big]^9$ 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{gray}{red}
    \grLCF[Math,RA=6]{-25,7,-7,13,-13,25}{9}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Groetzsch.tex <==
\newpage\section{Groetzsch}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   groetzsch            ––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grGrotzsch}{\oarg{options}\var{$k$}}

\medskip
From  Wikipedia : \url{http://en.wikipedia.org/wiki/Grötzsch_graph}  

\emph{The Grötzsch graph is a triangle-free graph with 11 vertices, 20 edges, and chromatic number 4. It is named after German mathematician Herbert Grötzsch, and its existence demonstrates that the assumption of planarity is necessary in Grötzsch's theorem (Grötzsch 1959) that every triangle-free planar graph is 3-colorable.}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/GroetzschGraph.html} 

\emph{The Grötzsch graph is smallest triangle-free graph with chromatic number four. It is identical to the Mycielski Graph of order four.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 

\end{NewMacroBox}


%GrotzschGraph
\tikzstyle{VertexStyle} = [shape           = circle,
                           shading         = ball,
                           ball color      = gray!60,
                           inner sep       = 3pt,
                           draw]
\SetVertexNoLabel
\tikzstyle{EdgeStyle}        = [thick,orange] 

\subsection{\tkzname{Grotzsch Graph : first form}}

\begin{center}
    \begin{tkzexample}[vbox]
  \begin{tikzpicture}
   \grGrotzsch[RA=3,RB=6]{6}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage\null 
\subsection{\tkzname{Grotzsch Graph : second form}}
\SetVertexLabel
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grGrotzsch[form=2,RA=6,RB=3]{6}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}



\vfill\newpage\null
\subsection{\tkzname{Grotzsch Graph : third form}} 
From Wikipedia : \url{http://en.wikipedia.org/wiki/Complete_bipartite_graph} 

\tikzstyle{VertexStyle} = [shape           = circle,
                           shading         = ball,
                           ball color      = blue!60,
                           inner sep       = 6pt,
                           draw]
\SetVertexNoLabel
\tikzstyle{EdgeStyle}    = [thick,double= red,
                            double distance = 1pt] 

\begin{center}
  \begin{tkzexample}[vbox]
    \begin{tikzpicture}[rotate=-18]
     \draw[scale=.5,samples at={-6.4,-6.3,...,6.4},
                smooth,thick,
                variable=\t,
                double= red,
                double distance = 1pt]
           plot ({3*(1.5*cos(\t r) +3*cos(1.5*\t r))},%
                 {3*(1.5*sin(\t r) -3*sin(1.5*\t r))});
    \begin{scope}[rotate=36]
       \grStar[prefix=a,RA=2.2]{6}%
       \grEmptyCycle[prefix=b,RA=4.4]{5}%
    \end{scope}
    \end{tikzpicture}
  \end{tkzexample}

\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Harries.tex <==
\newpage\section{Harries graph}\label{harries}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Nauru    ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grHarries}{\oarg{options}} 
  
From Wikipedia \url{http://en.wikipedia.org/wiki/Harries_graph}

\emph{In the mathematical field of graph theory, the Harries graph or Harries (3-10)-cage is a 3-regular undirected graph with 70 vertices and 105 edges.
The Harries graph has chromatic number 2, chromatic index 3, radius 6, diameter 6, girth 10 and is Hamiltonian. It is also a 3-vertex-connected and 3-edge-connected non-planar cubic graph.}

\medskip
From MathWorld \url{http://mathworld.wolfram.com/HarriesGraph.html}

\emph{The Harries graph  has 678 distinct LCF notations, two of which are order 5 (illustrated below) and 674 of which are order 1..}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
\end{NewMacroBox} 

\subsection{\tkzname{Harries graph} with \tkzcname{grHarries}}

The macro uses the  LCF notation :  $\big[-29,-19,-13,13,21,-27,27,33,-13,13,19,-21,-33,29\big]^5$

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grHarries[RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\subsection{\tkzname{Harries graph with LCF notation}}
It can be also  represented in LCF notation as  $\big[-35,9,15,-15,23,-27,27,-35,15,-15,-9,-27,27,-23\big]^5$ 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grLCF[RA=7]{-35,9,15,-15,23,-27,27,-35,15,-15,-9,-27,27,-23}{5}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Heawood.tex <==
\newpage\section{Heawood graph}\label{heawood}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    HEAWOOD  ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grHeawood}{\oarg{options}}

\medskip
From Wikipedia \url{http://en.wikipedia.org/wiki/Heawood_graph}

\emph{The Heawood graph is an undirected graph with 14 vertices and 21 edges. Each vertex is adjacent to exactly three edges (that is, it is a cubic graph), and all cycles in the graph have six or more edges.  Percy John Heawood (1861-1955) was an English mathematician who spent a large amount of time on questions related to the four colour theorem.}

\medskip
From MathWorld \url{http://mathworld.wolfram.com/HeawoodGraph.html}

\emph{The Heawood graph is the unique $(3,6)$-cage graph and Moore graph and is  graph illustrated below in one of his embeddings.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
\end{NewMacroBox}

\subsection{\tkzname{Heawood graph}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Shade]
   \grHeawood[RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
It can be represented in LCF notation as  $\big[5,-5\big]^7$

\tkzcname{grLCF[RA=5]\{5,9\}\{7\}} gives the result because  $-5 = 9\ mod\  14$.

\subsection{\tkzname{Heawood graph with LCF notation}}\label{lcf2}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grLCF[RA=7]{5,9}{7}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Hypercube.tex <==
\newpage\section{Hypercube}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––  Hypercube            –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
From Wikipedia :\url{http://en.wikipedia.org/wiki/Hypercube_graph}

In the mathematical field of graph theory, the hypercube graph $Q_n$ is a  special regular graph with $2n$ vertices, which correspond to the subsets of a set with $n$ elements. Two vertices labelled by subsets S and T are joined by an edge if and only if S can be obtained from T by adding or removing a single element. Each vertex of $Q_n$ is incident to exactly $n$ edges (that is, $Q_n$ is $n$-regular), so the total number of edges is $2^{n-1}n$.
The name comes from the fact that the hypercube graph is the one-dimensional skeleton of the geometric hypercube.
Hypercube graphs should not be confused with cubic graphs, which are graphs that are 3-regular. The only hypercube that is a cubic graph is $Q_3$.

\tikzstyle{VertexStyle}       = [shape        = circle,%
                                 fill         = red,%
                                 inner sep    = 3pt,%
                                 outer sep    = 0pt,%
                                 draw]
\SetVertexNoLabel

\subsection{\tkzname{The hypercube graph $Q_4$} }

The code is on the next page.

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grCycle[RA=8]{8}
  \pgfmathparse{8*(1-4*sin(22.5)*sin(22.5))}
  \let\tkzbradius\pgfmathresult
  \grCirculant[prefix=b,RA=\tkzbradius]{8}{3}
  \makeatletter
  \foreach \vx in {0,...,7}{%
    \pgfmathsetcounter{tkz@gr@n}{mod(\vx+1,8)}
    \pgfmathsetcounter{tkz@gr@a}{mod(\vx+7,8)}
    \pgfmathsetcounter{tkz@gr@b}{mod(\thetkz@gr@n+1,8)}
    \Edge(a\thetkz@gr@n)(b\thetkz@gr@b)
    \Edge(b\thetkz@gr@a)(a\vx)
    }
  \makeatother
\end{tikzpicture}
\end{tkzexample}
\end{center}
\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Koenisberg.tex <==
\newpage\section{The Seven Bridges of Königsberg}\label{seven}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––         Königsberg       ––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grKonisberg}{\oarg{options}\var{$k$}}

\medskip
From MathWorld : \url{http://mathworld.wolfram.com/KoenigsbergBridgeProblem.html}

\emph{The Königsberg bridge problem asks if the seven bridges of the city of Königsberg (left figure; Kraitchik 1942), formerly in Germany but now known as Kaliningrad and part of Russia, over the river Preger can all be traversed in a single trip without doubling back, with the additional requirement that the trip ends in the same place it began. This is equivalent to asking if the multigraph on four nodes and seven edges (right figure) has an Eulerian circuit. This problem was answered in the negative by Euler (1736), and represented the beginning of graph theory.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 

\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Seven_Bridges_of_Königsberg}

\emph{The paper written by Leonhard Euler on the Seven Bridges of Königsberg and published in 1736 is regarded as the first paper in the history of graph theory.\hfill\break
The Seven Bridges of Königsberg is a famous solved mathematics problem inspired by an actual place and situation. The city of Königsberg, Prussia (now Kaliningrad, Russia) is set on the Pregel River, and included two large islands which were connected to each other and the mainland by seven bridges. The problem is to decide whether it is possible to walk a route that crosses each bridge exactly once.\hfill\break
In 1736, Leonhard Euler proved that it was not possible. In proving the result, Euler formulated the problem in terms of graph theory, by abstracting the case of Königsberg — first, by eliminating all features except the landmasses and the bridges connecting them; second, by replacing each landmass with a dot, called a vertex or node, and each bridge with a line, called an edge or link. The resulting mathematical structure is called a graph.}
\end{NewMacroBox}

\subsection{\tkzname{Königsberg graph} with \tkzcname{grKonisberg}}
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}[node distance=4cm]
  \grKonisberg
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzcname{Königsberg graph} : fine embedding}
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}
   \renewcommand*{\VertexBallColor}{orange!50!red} 
   \renewcommand*{\EdgeDoubleDistance}{2pt} 
   \SetGraphUnit{4}
   \GraphInit[vstyle=Shade]
   \tikzset{LabelStyle/.style =   {draw,
                                   fill  = yellow,
                                   text  = red}}
   \Vertex{A}
   \EA(A){B}
   \EA(B){C}
   {\SetGraphUnit{8} 
   \NO(B){D}}
   \Edge[label=1](B)(D)
   \tikzset{EdgeStyle/.append style = {bend left}}
   \Edge[label=4](A)(B)
   \Edge[label=5](B)(A)
   \Edge[label=6](B)(C)
   \Edge[label=7](C)(B)
   \Edge[label=2](A)(D)
   \Edge[label=3](D)(C)
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Levi.tex <==
\newpage\section{Levi Graph}\label{levi}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––      Levy             –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grLevi}{\oarg{options}}

\medskip

From Wikipedia \url{http://en.wikipedia.org/wiki/Levi_graph}

\emph{In combinatorics a Levi graph or incidence graph is a bipartite graph associated with an incidence structure. From a collection of points and lines in an incidence geometry or a projective configuration, we form a graph with one vertex per point, one vertex per line, and an edge for every incidence between a point and a line.\hfil\break 
In the mathematical field of graph theory, the Tutte–Coxeter graph or Tutte eight-cage is a 3-regular graph with 30 vertices and 45 edges. As the unique smallest cubic graph of girth 8 it is a cage and a Moore graph. It is bipartite, and can be constructed as the Levi graph of the generalized quadrangle. }

From MathWord : \url{http://mathworld.wolfram.com/LeviGraph.html} 

\emph{It has 30 nodes and 45 edges. It has girth 8, diameter 4, chromatic number 2. The Levi graph is a generalized polygon which is the point/line incidence graph of the generalized quadrangle . The graph  was first discovered by Tutte (1947), and is also called the Tutte-Coxeter graph , Tutte's cage  or "Tutte's (3,8)-cage".The Levi graph is the unique (3,8)-cage graph.\hfil\break
The incidence graph of a generic configuration is sometimes known as a Levi graph (Coxeter 1950).} 

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
           
Some examples of Levi Graphs with this definition are~: 
\begin{itemize}
\item Desargues graph
\item Heawood graph
\item Heawood graph
\item Pappus graph
\item Gray graph 
\item Tutte eight-cage 
\end{itemize}

\end{NewMacroBox}

The two forms can be draw with :

 \begin{tkzexample}[code only]
   \grLevi[RA=7]\end{tkzexample}

and

 \begin{tkzexample}[code only]
    \grLevi[form=2,RA=7,RB=5,RC=3]\end{tkzexample}

You can see on the next pages, the two forms.
\vfill\newpage
Now I show you how to code this graph.

\subsection{\tkzname{Levy graph :form 1}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
  \begin{tikzpicture}
    \GraphInit[vstyle=Art]
    \grLCF[prefix=a,RA=6]{-13,-9,7,-7,9,13}{5}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\newpage

\subsection{\tkzname{Levy graph :form 2}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCycle[prefix=a,RA=7]{10}
  \EdgeInGraphMod{a}{10}{5}
  \grEmptyCycle[prefix=b,RA=5]{10}
  \grEmptyCycle[prefix=c,RA=3]{10}
  \EdgeInGraphMod{c}{10}{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-McGee.tex <==
\newpage\section{Mc Gee}\label{mcgee}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Mc Gee             –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grMcGee}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/McGeeGraph.html}  

\emph{The McGee graph is the unique 7-cage graph. It has 24 nodes, 36 edges, girth 7, diameter 4, and is a cubic graph. It has chromatic number 3.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}} 

\end{NewMacroBox}

\bigskip
\subsection{\tkzname{McGee graph with }\tkzcname{grMcGee}}

\bigskip
The same  result is obtained with 

\begin{tkzexample}[code only]
 \grLCF[Math,RA=6]{-12,7,-7}{8}\end{tkzexample}

\medskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grMcGee[Math,RA=6]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
Others embeddings
\subsection{\tkzname{McGee graph with }\tkzcname{grLCF}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grLCF[Math,RA=6]{-12,-6,6,-12,7,-7,-12,6,-6,-12,7,-7}{2}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{McGee graph with }\tkzcname{grLCF}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grLCF[Math,RA=6]{-12,6,-7,-12,7,-8,11,-6,6,-11,8,%
                      -7,-12,7,-6,-12,7,-11,-8,7,-7,8,11,-7}{1}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Moebius.tex <==
\newpage\section{Möbius-Kantor Graph}\label{moebius}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   Moebius             –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grMobiusKantor}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/Moebius-KantorGraph.html} 

\emph{The unique cubic symmetric graph on 16 nodes, illustrated above in several embeddings. It is 24 edges, girth 6, diameter 4, chromatic number 2, and is nonplanar but Hamiltonian. It can be represented in LCF notation  and is identical to a generalized Petersen graph .
} 

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
\end{NewMacroBox}




\subsection{\tkzname{Möbius Graph : form I}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetGraphArtColor{red}{olive} 
   \SetVertexNoLabel
   \grMobiusKantor[RA=7]
\end{tikzpicture} 
\end{tkzexample}
\end{center}
 
\vfill\newpage
\subsection{\tkzname{Möbius Graph : form II}}
 
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=22.5]
   \GraphInit[vstyle=Shade]
  \SetGraphArtColor{red!50}{brown!50} 
   \SetVertexNoLabel
   \grMobiusKantor[form=2,RA=7,RB=3]
 \end{tikzpicture}
\end{tkzexample} 
\end{center} 

\vfill\newpage
 \subsection{\tkzname{Möbius Graph : form III}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \grMobiusKantor[form=3,RA=7,RB=2]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
 
\vfill\newpage
\subsection{\tkzname{Möbius Graph with LCF notation}} 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
 \grLCF[RA=7]{5,-5}{8}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Möbius Graph with \tkzcname{grGeneralizedPetersen}} } 

\begin{center}
\begin{tkzexample}[vbox] 
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel  
  \grGeneralizedPetersen[RA=7,RB=4]{8}{3} 
 \end{tikzpicture}
\end{tkzexample} 
\end{center}  

\vfill\newpage
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––   Moebius     Ladder   –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
A Möbius ladder of order $2n$ is a simple graph obtained by introducing a twist in a prism graph of order $2n$ that is isomorphic to the circulant graph  with order $2n$   and $L=\{1,n\}$

\url{http://mathworld.wolfram.com/MoebiusLadder.html}

\subsection{\tkzname{Möbius Ladder Graph}} 


\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \grMobiusLadder[RA=7,RB=2]{8}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center} 


\vfill\newpage  
\subsection{\tkzname{Circulant Graph isomorphic to the last graph}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \grCirculant[RA=7]{16}{1,8}%
\end{tikzpicture}  
\end{tkzexample}
\end{center} 

\endinput

\newpage\section{Möbius-Kantor Graph}\label{MK}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––Möbius-Kantor Graph –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{%
\newmacro{Möbius-Kantor Graph : \tkzcname{grMobiusKantor}}}{lightgray}
 \tkzcname{grMobiusKantor[|RA|=\meta{Number}]\var{Number}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/Moebius-KantorGraph.html}  

\emph{The unique cubic symmetric graph on 16 nodes, illustrated above in two embeddings. It is 24 edges, girth 6, diameter 4, chromatic number 2, and is nonplanar but Hamiltonian. It is identical to the generalized Petersen graph.}
\href{http://mathworld.wolfram.com/Moebius-KantorGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
The Möbius-Kantor Graph is implemented in \tkzname{tkz-berge} as \tkzcname{grMobiusKantor}.
\end{NewMacroBox}

\subsection{Möbius-Kantor Graph with \tkzcname{grGeneralizedPetersen}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade] 
   \SetVertexNoLabel
   \grGeneralizedPetersen[RA=7,RB=4]{3}{1}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage\null 


\subsection{\tkzname{MobiusKantor graph}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Shade] 
   \SetVertexNoLabel
  \grMobiusKantor[RA=5]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Nauru.tex <==
\newpage\section{Nauru graph}\label{nauru}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Nauru    ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grNauru}{\oarg{options}} 
  
From Wikipedia \url{http://en.wikipedia.org/wiki/Nauru_graph}

\emph{TIn the mathematical field of graph theory, the Nauru graph is a symmetric bipartite cubic graph with 24 vertices and 36 edges. It was named by David Eppstein after the twelve-pointed star in the flag of Nauru. It has chromatic number 2, , diameter 4, radius 4 and girth 6. It is also a 3-vertex-connected and 3-edge-connected graph.}

\medskip
From MathWorld \url{http://mathworld.wolfram.com/NauruGraph.html}

\emph{The Nauru graph is the name given by Eppstein (2007) to the generalized Petersen graph GP(12,5) , which is also cubic symmetric graph , the permutation star graph of order 4, and the incidence graph of the Coxeter configuration. The name derives from the resemblance of the central star polygon in the generalized Petersen embedding to the 12-point star on the flag of the Pacific island nation of Nauru. The Nauru graph is  graph illustrated below in one of his embeddings.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
\end{NewMacroBox} 

\subsection{\tkzname{Nauru graph}}

It can be represented in LCF notation as  $\big[5, −9, 7, −7, 9, −5\big]^4$

\tkzcname{grLCF[RA=5]\{5,9\}\{7\}} gives the result because  $-5 = 9\ mod\  14$.

\subsection{\tkzname{Nauru graph with LCF notation}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grLCF[RA=7]{5, −9, 7, −7, 9, −5}{4}%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\vfill\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Pappus.tex <==
\newpage\section{Pappus}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––    Pappus   ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grPappus}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/PappusGraph.html}

\emph{A cubic symmetric distance-regular graph on 18 vertices, illustrated below in three embeddings. It can be represented in LCF notation $[5,7,-7,7,-7,-5]^3$  (Frucht 1976).}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   

From Wikipedia : \url{http://en.wikipedia.org/wiki/Pappus_graph}
\emph{In the mathematical field of graph theory, the Pappus graph is a 3-regular graph with 18 vertices and 27 edges, formed as the Levi graph of the Pappus configuration. It is a distance-regular graph, one of only 14 such cubic graphs according to Cubic symmetric graphs.}

This macro can be used with three different forms.
\end{NewMacroBox}

\bigskip


\subsection{\tkzname{Pappus Graph : form 1}} 
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.7]
   \GraphInit[vstyle=Art]
   \grPappus[RA=7]
\end{tikzpicture} 
\end{tkzexample}  
\end{center}
 
\vfill\newpage     
\subsection{\tkzname{Pappus Graph : form 2}} 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{olive}
   \grPappus[form=2,RA=7,RB=5,RC=3]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Pappus Graph : form 3}} 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{gray}{blue}
   \grPappus[form=3,RA=7,RB=5,RC=2.5] 
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Petersen.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/NamedGraphs/doc/NamedGraphs-main.tex
\newpage\section{Petersen}\label{petersen} 
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Petersen            –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grPetersen}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/PetersenGraph.html}

\emph{The Petersen graph is the graph , illustrated below in several embeddings, possessing 10 nodes, all of whose nodes have degree three. The Petersen graph is implemented in \tkzname{tkz-berge} as \tkzcname{grPetersen}.
The Petersen graph has girth 5, diameter 2, edge chromatic number 4, chromatic number 3.}

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   

From Wikipedia : \url{http://en.wikipedia.org/wiki/Petersen_graph}

\emph{In graph theory, the Petersen graph is an undirected graph with 10 vertices and 15 edges. It is a small graph that serves as a useful example and counterexample for many problems in graph theory. The Petersen graph is named for Julius Petersen, who in 1898 constructed it to be the smallest bridgeless cubic graph with no three-edge-coloring. Although the graph is generally credited to Petersen, it had in fact first appeared 12 years earlier, in 1886.}

This macro can be used with three different forms.
\end{NewMacroBox}

 \subsection{\tkzname{Petersen graph : form 1}}
\begin{center}
\begin{tkzexample}[latex=8cm]
\begin{tikzpicture}[scale=.8]
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{red}{olive}
    \grPetersen[form=1,RA=5,RB=3]%
 \end{tikzpicture}
\end{tkzexample} 
\end{center}
\vfill\newpage
\subsection{\tkzname{Petersen graph : form 2}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{olive}
   \grPetersen[form=2,RA=7,RB=3]%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill\newpage
\subsection{\tkzname{Petersen graph : form 3}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{red}{olive}
    \grPetersen[form=3,RA=7]%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill\newpage
\subsection{\tkzname{The line graph of the Petersen graph}}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
\GraphInit[vstyle=Art]\SetGraphArtColor{white}{blue}
  \begin{scope}[rotate=-90] \grCirculant[RA=1.5,prefix=a]{5}{2}\end{scope}
  \begin{scope}[rotate=-18] \grEmptyCycle[RA=4,prefix=b]{5}{2} \end{scope}
  \begin{scope}[rotate=18]  \grCycle[RA=7,prefix=c]{5}         \end{scope}
  \EdgeIdentity{a}{b}{5} 
  \EdgeIdentity{b}{c}{5}
  \EdgeDoubleMod{b}{5}{0}{1}{a}{5}{2}{1}{5}
  \EdgeDoubleMod{c}{5}{0}{1}{b}{5}{1}{1}{5}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Petersen   Gen     –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grGeneralizedPetersen}{\oarg{RA=\meta{Number},RB=\meta{Number}}\var{integer}\var{integer}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/GeneralizedPetersenGraph.html}

\emph{The generalized Petersen graph , also denoted $GP(n,k)$  , for $n \geq 3$ and $1\leq k \leq \lfloor (n-1)/2\rfloor $ is a graph consisting of an inner star polygon  (circulant graph ) and an outer regular polygon  (cycle graph ) with corresponding vertices in the inner and outer polygons connected with edges.  has  nodes and  edges. The Petersen graph is implemented in \tkzname{tkz-berge} as \tkzcname{grGeneralizedPetersen}.}
\href{http://mathworld.wolfram.com/GeneralizedPetersenGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Petersen_graph}
\emph{In 1950 H. S. M. Coxeter introduced a family of graphs generalizing the Petersen graph. These graphs are now called generalized Petersen graphs, a name given to them in 1969 by Mark Watkins. In Watkins' notation, $G(n,k)$ is a graph with vertex set\hfill\break
 ${u_0, u_1,\dots, u_{n-1}, v_0, v_1, \dots, v_{n-1}}$\hfill\break
and edge set\hfill\break
${u_i u_{i+1}, u_i v_i, v_i u_{i+k}: i = 0,\dots,n-1}$\hfill\break
where subscripts are to be read modulo $n$ and $k<n/2$. Coxeter's notation for the same graph would be $\{n\}+\{n/k\}.$
The Petersen Graph itself is $G(5,2)$ or $\{5\}+\{5/2\}$.
}

This macro can be used with three different forms.
\end{NewMacroBox}

\subsection{\tkzname{Generalized Petersen graph} GP(5,1)}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90,scale=.6]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{4pt}
  \grGeneralizedPetersen[RA=5,RB=2]{5}{1}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{The Petersen graph} GP(5,2)}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
    \renewcommand*{\VertexInnerSep}{8pt}
    \grGeneralizedPetersen[RA=7,RB=4]{5}{2}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Generalized Petersen graph} GP(6,2)}

\vspace*{2cm}\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{8pt}
  \grGeneralizedPetersen[RA=7,RB=4]{6}{2}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Generalized Petersen graph} GP(7,3)}

\vspace*{2cm}\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{8pt}
  \grGeneralizedPetersen[RA=7,RB=4]{7}{3}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Generalized Petersen graph} GP(11,5)}

\vspace*{2cm}\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90]
  \renewcommand*{\VertexInnerSep}{8pt}
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \grGeneralizedPetersen[RA=7,RB=4]{11}{5}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Platonic.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/NamedGraphs/doc/NamedGraphs-main.tex
\newpage\section{ The five Platonics Graphs}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––  Platonic graphs      –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

The Platonic Graphs are the graphs formed by the edges and vertices of the five regular Platonic solids. The five Platonics Graphs  are illustrated below.  

\begin{enumerate}
  \item tetrahedral
  \item octahedral
  \item cube
  \item icosahedral
  \item dodecahedral
\end{enumerate} 


%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grTetrahedral}{\oarg{RA=Number}}
From MathWord : \url{http://mathworld.wolfram.com/TetrahedralGraph.html} 

\emph{\tkzname{Tetrahedral Graph}  is the unique polyhedral graph on four nodes which is also the complete graph  and therefore also the wheel graph . It is implemented as \tkzcname{grTetrahedral}}
\href{http://mathworld.wolfram.com/TetrahedralGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}
}
It has :

\begin{enumerate}
 \item  4 nodes,
 \item  6 edges,
 \item  graph diameter 1.
\end{enumerate}

The  Tetrahedral Graph is 3-Regular
\end{NewMacroBox}

\subsection{\tkzname{Tetrahedral}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6]
      \GraphInit[vstyle=Shade]
      \renewcommand*{\VertexInnerSep}{4pt} 
      \SetVertexNoLabel\SetGraphShadeColor{red!50}{black}{red}
      \grTetrahedral[RA=5]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage
\subsection{\tkzname{Tetrahedral LCF embedding}}

\vspace*{2cm}
\begin{center}
  \begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18]
     \renewcommand*{\VertexInnerSep}{8pt} 
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{red!50}{orange}
     \grLCF[RA=7]{2,-2}{2}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage   
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grOctahedral}{\oarg{RA=\meta{Number},RB=\meta{Number}}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/OctahedralGraph.html} 

\emph{\tkzname{Octahedral Graph}  is isomorphic to the circulant graph $CI_{[1,2]}(6)$ . Two embeddings of this graph are illustrated below. It is implemented as \tkzcname{grOctahedral} or as \tkzcname{grSQCycle\{6\}}.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   

It has :

\begin{enumerate}
 \item  6 nodes,
 \item  12 edges,
 \item  graph diameter 2.
\end{enumerate}

\medskip
 The  Octahedral Graph is 4-Regular.
\end{NewMacroBox}


\medskip
\subsection{\tkzname{Octahedral}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grOctahedral[RA=6,RB=2]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage\null
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
       \grSQCycle[RA=5]{6}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage\null
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\medskip
\begin{NewMacroBox}{grCubicalGraph}{\oarg{RA=\meta{Number},RB=\meta{Number}}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/CubicalGraph.html} 

\emph{\tkzname{Cubical Graph}  is isomorphic to a generalized Petersen graph  $PG_{[4,1]}$, to a bipartite Kneser graph , to a crown graph and it is equivalent to the Cycle Ladder $CL(4)$. Two embeddings of this graph are illustrated below. It is implemented as \tkzcname{grCubicalGraph} or \tkzcname{grPrism\{4\}}.}
\href{http://mathworld.wolfram.com/CubicalGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

It has :

\begin{enumerate}
 \item  8 nodes,
 \item  12 edges,
 \item  graph diameter 3.
\end{enumerate}

 The  Cubical Graph is 3-Regular.
\end{NewMacroBox}

\subsection{\tkzname{Cubical Graph : form 1}}
\begin{center}
  \begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grCubicalGraph[RA=5,RB=2]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage\null 
\subsection{\tkzname{Cubical Graph : form 2}}
\begin{center}
  \begin{tkzexample}[vbox]
\begin{tikzpicture}
  \grCubicalGraph[form=2,RA=7,RB=4]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Cubical LCF embedding}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18]
    \GraphInit[vstyle=Art]\renewcommand*{\VertexInnerSep}{8pt} 
    \SetGraphArtColor{red!50}{orange}
    \grLCF[RA=7]{3,-3}{4}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grIcosahedral}{\oarg{RA=\meta{Number},RB=\meta{Number},RC=\meta{Number}}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/IcosahedralGraph.html} 

\emph{The \tkzname{Icosahedral Graph}  is the Platonic graph whose nodes have the connectivity of the icosahedron, illustrated above in a number of embeddings. The icosahedral graph has 12 vertices and 30 edges. Since the icosahedral graph is regular and Hamiltonian, it has a generalized LCF notation.}
\href{http://mathworld.wolfram.com/IcosahedralGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
It has :

\begin{enumerate}
 \item  12 nodes,
 \item  30 edges,
 \item  graph diameter 3.
\end{enumerate}

\medskip
 The  Icosahedral Graph is 5-Regular.
\end{NewMacroBox}

\medskip

\subsection{\tkzname{Icosahedral forme 1 }}

\tikzstyle{EdgeStyle}= [thick,%
                        double          = orange,%
                        double distance = 1pt] 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.8]
 \GraphInit[vstyle=Art]\renewcommand*{\VertexInnerSep}{4pt} 
 \SetGraphArtColor{red}{orange}
 \grIcosahedral[RA=5,RB=1]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage    

\subsection{\tkzname{Icosahedral forme 2 }}
\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=-30]
   \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt} 
   \SetGraphArtColor{red!50}{orange}
   \grIcosahedral[form=2,RA=8,RB=2,RC=.8]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage

\subsection{\tkzname{Icosahedral} \tkzname{RA=1} et \tkzname{RB=7}}
\begin{center}
\begin{tkzexample}[vbox]
 \begin{tikzpicture}
    \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt} 
    \SetGraphArtColor{red!50}{orange}
    \grIcosahedral[RA=1,RB=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage    
\subsection{\tkzname{Icosahedral LCF embedding 1}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18]
    \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt} 
    \SetGraphArtColor{red!50}{orange}
    \grLCF[RA=7]{-4,-3,4}{6}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage    
\subsection{\tkzname{Icosahedral LCF embedding 2}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grLCF[RA=7]{-2,2,3}{6}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage 
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{NewMacroBox}{grDodecahedral}{\oarg{RA=\meta{Number},RB=\meta{Number},RC=\meta{Number},RD=\meta{Number}}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/DodecahedralGraph.html} 

\emph{The \tkzname{Icosahedral Graph}  is the Platonic graph corresponding to the connectivity of the vertices of a dodecahedron, illustrated above in four embeddings. The left embedding shows a stereographic projection of the dodecahedron, the second an orthographic projection, the third is from Read and Wilson, and the fourth is derived from LCF notation.}
\href{http://mathworld.wolfram.com/DodecahedralGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\medskip
It has :

\begin{enumerate}
 \item  20 nodes,
 \item  30 edges,
 \item  graph diameter 5.
\end{enumerate}

\medskip
 The  Dodecahedral Graph is 3-Regular.
\end{NewMacroBox}

\medskip
\subsection{\tkzname{Dodecahedral}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18,scale=.6]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grDodecahedral[RA=7,RB=4,RC=2,RD=1]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\subsection{\tkzname{Dodecahedral other embedding}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCycle[RA=7,prefix=a]{10}
   \grSQCycle[RA=4,prefix=b]{10}
     \foreach \v in {0,...,9}
       {\Edge(a\v)(b\v)}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill\newpage
\subsection{\tkzname{Dodecahedral LCF embedding}}

\vspace*{2cm}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=18]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grLCF[RA=7]{10,7,4,-4,-7,10,-4,7,-7,4}{2}
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput


==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Robertson.tex <==
\newpage\section{Robertson}\label{robertson}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Robertson          –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grRobertson}{\oarg{options}\var{$k$}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/RobertsonGraph.html} 

\medskip
\emph{The Robertson graph is the unique (4,5)-cage graph, illustrated below. It has 19 vertices and 38 edges. It has girth 5, diameter 3, chromatic number 3, and is a quartic graph.} 
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   

\end{NewMacroBox}

\subsection{\tkzname{Robertson  graph with \tkzcname{grRobertson} }}

The cage 

\medskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.6]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{black}{gray}
  \grRobertson[RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

\clearpage\newpage
\subsection{\tkzname{Fine embedding of the Robertson  graph from RV}}

\begin{center}
 \begin{tikzpicture}[scale=.8]
     \tikzstyle{TempEdgeStyle}= [thick,black,%
                               double               = gray,%
                               double distance      = 1.5pt]%
   \SetVertexNoLabel
   \renewcommand*{\VertexBigMinSize}{10pt}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \SetUpEdge[style  = {thick,%
                        double          = orange,%
                        double distance = 1pt}]
   \SetGraphShadeColor{gray}{black}{gray}
   \tikzstyle{EdgeStyle} = [TempEdgeStyle]
   \begin{scope}[rotate=-30]
     \grEmptyCycle[RA=5.4]{3}
   \end{scope}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right=10]
   \grCycle[prefix=b,RA=4]{12}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle]
   \grCirculant[prefix=c,RA=2]{4}{2}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend left]
   \EdgeDoubleMod{c}{4}{0}{1}%
                 {b}{12}{4}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right]
    \EdgeDoubleMod{c}{4}{0}{1}
                  {b}{12}{8}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{11}{4}{3}
    \EdgeDoubleMod{c}{4}{0}{1}%
                  {b}{12}{0}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend left=60]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{8}{4}{3}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right=60]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{2}{4}{3}
    \tikzstyle{EdgeStyle}=[TempEdgeStyle,in=-50,out=-120,
                           relative,looseness=2.5]
    \EdgeDoubleMod{a}{3}{0}{1}%
                   {b}{12}{5}{4}{3}
   \end{tikzpicture}
\end{center}

\clearpage\newpage
Code for the Robertson Graph

\medskip
\begin{tkzexample}[code only]
\begin{tikzpicture}[scale=.9]
  \tikzstyle{TempEdgeStyle}= [thick,black,%
                              double               = gray,%
                              double distance      = 1.5pt]%
   \SetVertexNoLabel
   \renewcommand*{\VertexBigMinSize}{14pt}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \SetUpEdge[style  = {thick,%
                        double          = orange,%
                        double distance = 1pt}]

   \SetGraphShadeColor{gray}{black}{gray}
   \tikzstyle{EdgeStyle} = [TempEdgeStyle]
   \begin{scope}[rotate=-30]
     \grEmptyCycle[RA=5.4]{3}
   \end{scope}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right=10]
   \grCycle[prefix=b,RA=4]{12}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle]
   \grCirculant[prefix=c,RA=2]{4}{2}
   \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend left]
   \EdgeDoubleMod{c}{4}{0}{1}%
                 {b}{12}{4}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right]
    \EdgeDoubleMod{c}{4}{0}{1}
                  {b}{12}{8}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{11}{4}{3}
    \EdgeDoubleMod{c}{4}{0}{1}%
                  {b}{12}{0}{3}{4}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend left=60]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{8}{4}{3}
    \tikzstyle{EdgeStyle}= [TempEdgeStyle,bend right=60]
    \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{2}{4}{3}
    \tikzstyle{EdgeStyle}=[TempEdgeStyle,in=-50,out=-120,
                           relative,looseness=2.5]
    \EdgeDoubleMod{a}{3}{0}{1}%
                   {b}{12}{5}{4}{3}
 \end{tikzpicture}
\end{tkzexample}  

\clearpage\newpage   
\subsection{\tkzname{Robertson  graph with new styles}}

The code  with new styles, the result is on the next page.

\bigskip
\begin{tkzexample}[code only]
  \begin{tikzpicture}[scale=1]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{gray}{red}
  \begin{scope}[rotate=-30]
    \grEmptyCycle[RA=5]{3}
  \end{scope}
  {\tikzset{EdgeStyle/.append style = {bend right=10}}
  \grCycle[prefix=b,RA=3.5]{12}}
  \grCirculant[prefix=c,RA=2]{4}{2}
  {\tikzset{EdgeStyle/.append style = {bend left}}
  \EdgeDoubleMod{c}{4}{0}{1}%
                {b}{12}{4}{3}{4}}
  {\tikzset{EdgeStyle/.append style = {bend right}}
   \EdgeDoubleMod{c}{4}{0}{1}
                 {b}{12}{8}{3}{4}}
   \EdgeDoubleMod{a}{3}{0}{1}%
                 {b}{12}{11}{4}{3}
   \EdgeDoubleMod{c}{4}{0}{1}%
                 {b}{12}{0}{3}{4}
  {\tikzset{EdgeStyle/.append style = {bend left=60}}
   \EdgeDoubleMod{a}{3}{0}{1}%
                 {b}{12}{8}{4}{3}}
  {\tikzset{EdgeStyle/.append style = {bend right=60}}
   \EdgeDoubleMod{a}{3}{0}{1}%
                 {b}{12}{2}{4}{3}}
   {\tikzset{EdgeStyle/.append style = {in=-50,out=-120,%
                                        relative,looseness=2.5}}
   \EdgeDoubleMod{a}{3}{0}{1}%
                  {b}{12}{5}{4}{3}}
 \end{tikzpicture}
\end{tkzexample} 

\begin{center}
\begin{tikzpicture}[scale=1]
\GraphInit[vstyle=Art]
\SetGraphArtColor{gray}{red}
\begin{scope}[rotate=-30]
  \grEmptyCycle[RA=5]{3}
\end{scope}
{\tikzset{EdgeStyle/.append style = {bend right=10}}
\grCycle[prefix=b,RA=3.5]{12}}
\grCirculant[prefix=c,RA=2]{4}{2}
{\tikzset{EdgeStyle/.append style = {bend left}}
\EdgeDoubleMod{c}{4}{0}{1}%
              {b}{12}{4}{3}{4}}
{\tikzset{EdgeStyle/.append style = {bend right}}
 \EdgeDoubleMod{c}{4}{0}{1}
               {b}{12}{8}{3}{4}}
 \EdgeDoubleMod{a}{3}{0}{1}%
               {b}{12}{11}{4}{3}
 \EdgeDoubleMod{c}{4}{0}{1}%
               {b}{12}{0}{3}{4}
{\tikzset{EdgeStyle/.append style = {bend left=60}}
 \EdgeDoubleMod{a}{3}{0}{1}%
               {b}{12}{8}{4}{3}}
{\tikzset{EdgeStyle/.append style = {bend right=60}}
 \EdgeDoubleMod{a}{3}{0}{1}%
               {b}{12}{2}{4}{3}}
 {\tikzset{EdgeStyle/.append style = {in=-50,out=-120,%
                                      relative,looseness=2.5}}
 \EdgeDoubleMod{a}{3}{0}{1}%
                {b}{12}{5}{4}{3}}
\end{tikzpicture} 
\end{center} 
\clearpage\newpage
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––    Robertson  Wegner  –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{NewMacroBox}{grRobertsonWegner}{\oarg{options}\var{$k$}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/Robertson-WegnerGraph.html} 

\medskip
\emph{he Robertson-Wegner graph is of the four (5,5)-cage graphs, also called Robertson's cage . Like the other (5,5)-cages, the Robertson-Wegner graph has 30 nodes. It has 75 edges, girth 5, diameter 3, and chromatic number 4.}
\href{http://mathworld.wolfram.com/Robertson-WegnerGraph.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\end{NewMacroBox}

\subsection{\tkzname{Robertson-Wegner graph}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90,scale=.6]
    \GraphInit[vstyle=Art]
    \tikzset{VertexStyle/.append style={minimum size=2pt}} 
    \grRobertsonWegner[RA=6]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}

The next code gives the same result

\begin{tkzexample}[code only]
\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art] 
    \grLCF[RA=6]{6,12}{15}
    \EdgeInGraphMod{a}{30}{9}{1}{6} \EdgeInGraphMod*{a}{30}{15}{2}{6}
    \EdgeInGraphMod*{a}{30}{9}{3}{6}
 \end{tikzpicture}
\end{tkzexample} 


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Tutte.tex <==
\newpage\section{Tutte-Coxeter}\label{tutte}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––      Tutte             –––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>


\begin{NewMacroBox}{grTutteCoxeter}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/LeviGraph.html}

\emph{The Levi graph is the unique (3,8)-cage graph and Moore graph. It is also distance-regular and is also called the Tutte-Coxeter graph or Tutte's 8-cage.}

\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
           
\medskip
From Wikipedia : \url{http://en.wikipedia.org/wiki/Tutte–Coxeter_graph}

\emph{In the mathematical field of graph theory, the Tutte–Coxeter graph or Tutte eight-cage is a 3-regular graph with 30 vertices and 45 edges. As the unique smallest cubic graph of girth 8 it is a cage and a Moore graph. It is bipartite, and can be constructed as the Levi graph of the generalized quadrangle. The graph is named after William Thomas Tutte and H. S. M. Coxeter; it was discovered by Tutte (1947) but its connection to geometric configurations was investigated by both authors in a pair of jointly published papers (Tutte 1958; Coxeter 1958a).}
\end{NewMacroBox}

\subsection{\tkzname{Tutte-Coxeter graph (3,8)-cage or Levi graph}}
An other method to get the same result is~:

\medskip
\begin{tkzexample}[code only]
 \grLCF[RA=7]{-13,-9,7,-7,9,13}{5}\end{tkzexample}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.7]
   \GraphInit[vstyle=Art] 
   \tikzset{VertexStyle/.append style={minimum size=2pt}}  
   \SetGraphArtColor{blue}{darkgray}
   \grTutteCoxeter
\end{tikzpicture}
\end{tkzexample}

\end{center}

\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-Wong.tex <==
\newpage\section{Wong}\label{wong}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––-––––––––––––>
%<––––––––––––––––––––    Wong   (5,5)-cages  –––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––-–––––––>
\begin{NewMacroBox}{grWong}{\oarg{options}}

\medskip
From MathWord : \url{http://mathworld.wolfram.com/WongGraph.html} 

\emph{The Wong graph is one of the four $(5,5)$-cage graphs. Like the other -cages, the Wong graph has 30 nodes. It has 75 edges, girth 5, diameter 3, chromatic number 4.}
\href{http://mathworld.wolfram.com/topics/GraphTheory.html}%
           {\textcolor{blue}{MathWorld}} by \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}   
\end{NewMacroBox}


\subsection{\tkzname{Wong graph}}
You can see the cage definition here : \ref{cage}

\bigskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=90,scale=.6]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{blue}
   \grWong[RA=7]
 \end{tikzpicture}
\end{tkzexample} 
\end{center}


\endinput

==> tkz-berge/NamedGraphs/doc/latex/NamedGraphs-couverture.tex <==
\thispagestyle{empty}
\null\vfill
\begin{center}
\textcolor{Brown}{\fontsize{30}{30}\selectfont{\upshape Gallery of named graphs}}

\vspace{0.25cm}
\hfill\textcolor{Brown}{\fontsize{14}{14}\selectfont{\upshape with tkz-berge.sty by Alain Matthes}}
\end{center}

\vspace{3cm}
\begin{tikzpicture}[scale=5]
   \SetVertexNoLabel
   \tikzstyle{VertexStyle} = [draw,
                              shape        = circle,
                              shading      = ball,
                              ball color   = red!50,
                              inner sep    = 10pt,
                              outer sep    = 0pt]
    \tikzstyle{EdgeStyle} = [thick,line width= 2pt,color=red]
    \draw[fill  = white,color = white] circle (0.55cm);
    \draw (0,0)  node[circle,draw,shade,
                      ball color    = orange,
                      minimum size = 3cm] (am){\textbf{AlterMundus}};
     \grIcosahedral[RA=1.4,RB=0.8]
\end{tikzpicture}  
\vfill\newpage\null\thispagestyle{empty}
\endinput



==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-1-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.7]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{7}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-1-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{8}
  \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-1-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
  \grAndrasfai[RA=7]{9}
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-10-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
     \SetVertexNoLabel
     \grLCF[RA=6]{3,-3}{4}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-11-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.6]
    \grDesargues[Math,RA=6]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-11-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \grDesargues[form=2,Math,RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-11-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
   \grLCF[Math,RA=6]{5,-5,9,-9}{5}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-12-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.6]
  \GraphInit[vstyle=Shade]
  \SetGraphShadeColor{red}{Maroon}{fondpaille}
  \SetVertexNoLabel
  \grDoyle[RA=7,RB=5,RC=3]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-12-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetGraphShadeColor{red}{Magenta}{white}
   \SetVertexNoLabel
   \grDoyle[form=2,RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-12-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \SetGraphArtColor{red}{Magenta}{red}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \grDoyle[form=3,RA=7,RB=2]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-13-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.8]
      \GraphInit[vstyle=Art]
      \SetGraphArtColor{blue}{darkgray}
      \grFolkman[RA=6]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-15-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.7]
   \grFranklin[Math,RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-15-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \grLCF[Math,RA=7]{-5,-3,3,5}{3}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-16-0-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{gray}{red}
    \grLCF[Math,RA=6]{-25,7,-7,13,-13,25}{9}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-17-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

  \begin{tikzpicture}
   \grGrotzsch[RA=3,RB=6]{6}%
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-17-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \grGrotzsch[form=2,RA=6,RB=3]{6}%
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-18-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}%
   \GraphInit[vstyle=Shade]
   \grHeawood[RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-18-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \grLCF[RA=7]{5,9}{7}%
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-2-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

 \begin{tikzpicture}[scale=.6]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{red}{olive}
 \grBalaban[form=1,RA=7,RB=3,RC=3]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-2-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

 \begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{gray}{blue!50}
 \grBalaban[form=2,RA=7,RB=7,RC=4,RD=2.5]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-2-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

  \begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{brown}{orange}
  \grBalaban[form=3,RA=7,RB=6.5,RC=5.6,RD=5.6,RE=4.6]
  \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-20-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

 \begin{tikzpicture}[node distance=4cm]
  \grKonisberg
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-21-0-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}


\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-21-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

  \begin{tikzpicture}
    \GraphInit[vstyle=Art]
    \grLCF[prefix=a,RA=6]{-13,-9,7,-7,9,13}{5}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-21-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grCycle[prefix=a,RA=7]{10}
  \EdgeInGraphMod{a}{10}{5}
  \grEmptyCycle[prefix=b,RA=5]{10}
  \grEmptyCycle[prefix=c,RA=3]{10}
  \EdgeInGraphMod{c}{10}{4}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-22-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grMcGee[Math,RA=6]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-22-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grLCF[Math,RA=6]{-12,-6,6,-12,7,-7,-12,6,-6,-12,7,-7}{2}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-22-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Art]
    \grLCF[Math,RA=6]{-12,6,-7,-12,7,-8,11,-6,6,-11,8,%
                      -7,-12,7,-6,-12,7,-11,-8,7,-7,8,11,-7}{1}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetGraphArtColor{red}{olive}
   \SetVertexNoLabel
   \grMobiusKantor[RA=7]
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=22.5]
   \GraphInit[vstyle=Shade]
  \SetGraphArtColor{red!50}{brown!50}
   \SetVertexNoLabel
   \grMobiusKantor[form=2,RA=7,RB=3]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \grMobiusKantor[form=3,RA=7,RB=2]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-4-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
 \grLCF[RA=7]{5,-5}{8}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-5-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
  \grGeneralizedPetersen[RA=7,RB=4]{8}{3}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-6-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \grMobiusLadder[RA=7,RB=2]{8}%
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-23-7-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Shade]
   \grCirculant[RA=7]{16}{1,8}%
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-24-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.7]
   \GraphInit[vstyle=Art]
   \grPappus[RA=7]
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-24-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{olive}
   \grPappus[form=2,RA=7,RB=5,RC=3]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-24-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{gray}{blue}
   \grPappus[form=3,RA=7,RB=5,RC=2.5]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.8]
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{red}{olive}
    \grPetersen[form=1,RA=5,RB=3]%
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}%
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{olive}
   \grPetersen[form=2,RA=7,RB=3]%
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}%
    \GraphInit[vstyle=Art]
    \SetGraphArtColor{red}{olive}
    \grPetersen[form=3,RA=7]%
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-5-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90,scale=.6]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{4pt}
  \grGeneralizedPetersen[RA=5,RB=2]{5}{1}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-6-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
    \renewcommand*{\VertexInnerSep}{8pt}
    \grGeneralizedPetersen[RA=7,RB=4]{5}{2}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-7-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{8pt}
  \grGeneralizedPetersen[RA=7,RB=4]{6}{2}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-8-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \renewcommand*{\VertexInnerSep}{8pt}
  \grGeneralizedPetersen[RA=7,RB=4]{7}{3}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-25-9-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
  \renewcommand*{\VertexInnerSep}{8pt}
  \GraphInit[vstyle=Art]\SetGraphArtColor{red}{olive}
  \grGeneralizedPetersen[RA=7,RB=4]{11}{5}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.6]
      \GraphInit[vstyle=Shade]
      \renewcommand*{\VertexInnerSep}{4pt}
      \SetVertexNoLabel\SetGraphShadeColor{red!50}{black}{red}
      \grTetrahedral[RA=5]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-10-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18]
    \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt}
    \SetGraphArtColor{red!50}{orange}
    \grLCF[RA=7]{-4,-3,4}{6}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-11-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grLCF[RA=7]{-2,2,3}{6}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-12-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18,scale=.6]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grDodecahedral[RA=7,RB=4,RC=2,RD=1]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-13-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
   \grCycle[RA=7,prefix=a]{10}
   \grSQCycle[RA=4,prefix=b]{10}
     \foreach \v in {0,...,9}
       {\Edge(a\v)(b\v)}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-14-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red!50}{orange}
   \grLCF[RA=7]{10,7,4,-4,-7,10,-4,7,-7,4}{2}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18]
     \renewcommand*{\VertexInnerSep}{8pt}
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{red!50}{orange}
     \grLCF[RA=7]{2,-2}{2}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
       \grSQCycle[RA=5]{6}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-4-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \grCubicalGraph[RA=5,RB=2]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-5-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \grCubicalGraph[form=2,RA=7,RB=4]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-6-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=18]
    \GraphInit[vstyle=Art]\renewcommand*{\VertexInnerSep}{8pt}
    \SetGraphArtColor{red!50}{orange}
    \grLCF[RA=7]{3,-3}{4}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-7-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.8]
 \GraphInit[vstyle=Art]\renewcommand*{\VertexInnerSep}{4pt}
 \SetGraphArtColor{red}{orange}
 \grIcosahedral[RA=5,RB=1]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-8-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=-30]
   \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt}
   \SetGraphArtColor{red!50}{orange}
   \grIcosahedral[form=2,RA=8,RB=2,RC=.8]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-26-9-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

 \begin{tikzpicture}
    \GraphInit[vstyle=Art]  \renewcommand*{\VertexInnerSep}{8pt}
    \SetGraphArtColor{red!50}{orange}
    \grIcosahedral[RA=1,RB=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-27-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.6]
  \GraphInit[vstyle=Art]
  \SetGraphArtColor{black}{gray}
  \grRobertson[RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-27-4-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90]
    \GraphInit[vstyle=Art]
    \grLCF[RA=6]{6,12}{15}
    \EdgeInGraphMod{a}{30}{9}{1}{6} \EdgeInGraphMod*{a}{30}{15}{2}{6}
    \EdgeInGraphMod*{a}{30}{9}{3}{6}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-28-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=.7]
   \GraphInit[vstyle=Art]
   \tikzset{VertexStyle/.append style={minimum size=2pt}}
   \SetGraphArtColor{blue}{darkgray}
   \grTutteCoxeter
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-29-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[rotate=90,scale=.6]
   \GraphInit[vstyle=Art]
   \SetGraphArtColor{red}{blue}
   \grWong[RA=7]
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-3-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

 \begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \grCompleteBipartite[RA=2,RB=2,RS=3]{3}{2}
\end{tikzpicture}\hspace*{2cm}
\begin{tikzpicture}
   \GraphInit[vstyle=Art]
   \grCompleteBipartite[RA=2,RB=2,RS=3]{3}{3}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-3-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[scale=1.5]
  \GraphInit[vstyle=Art]
  \grCompleteBipartite[RA=3,RB=2,RS=5]{3}{5}
\end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-4-0-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}[node distance=4cm]
  \GraphInit[vstyle=Shade]
  \Vertex{a0}
  \NOEA(a0){a2}
  \NOEA(a2){a4}
  \NOWE(a0){a1}
  \NOWE(a1){a3}
  \Edges(a0,a1,a3)
  \Edges(a0,a2,a4)
  \Edge(a1)(a2)
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-6-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

    \begin{tikzpicture}
       \grCocktailParty[RA=3,RS=5]{4}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-6-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

   \begin{tikzpicture}
      \grCocktailParty[form=2,RA=4,RS=6]{4}
     \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-7-5-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{blue}{darkgray}
     \grLCF[RA=7]{-13,-9,7,-7,9,13}{5}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-8-1-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

    \begin{tikzpicture}[scale=.7]
       \GraphInit[vstyle=Shade]
       \SetVertexNoLabel
       \SetGraphShadeColor{blue!50!black}{blue}{gray}
       \grChvatal[RA=6,RB=2]
    \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-8-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

    \begin{tikzpicture}
      \GraphInit[vstyle=Art]
      \SetGraphArtColor{blue!50!black}{gray}
      \grChvatal[form=2,RA=7,RB=4,RC=1.4]
    \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-8-3-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

    \begin{tikzpicture}
     \GraphInit[vstyle=Art]
     \SetGraphArtColor{blue!50!black}{gray}
     \grChvatal[form=3,RA=7]
    \end{tikzpicture}

\end{document} 


==> tkz-berge/NamedGraphs/examples/latex/tkzNamed-9-2-0.tex <==
%
% tkz-namedgraphs (27/05/2011)
%
% Coding (utf8) Creator (TeX) Producer (pdfeTeX) 
% Author Alain Matthes
\input{tkzpreamblenamed.ltx}

\begin{document}

\begin{tikzpicture}
  \grCrown[form=2,RA=4,RS=6]{4}
 \end{tikzpicture}

\end{document} 


==> tkz-berge/doc/latex/TKZdoc-berge-classic.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/doc-us/TKZdoc-berge-main.tex
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\section{Classic Graphs}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––     graphes classiques    –––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsubsection{Cycle graph}
\begin{NewMacroBox}{grCycle}{\oarg{local options}\var{order}}

\medskip
\emph{A cycle graph $C_n$ is a graph on $n$ nodes containing a single cycle through all nodes. Cycle graphs can be generated using \tkzcname{grCycle} in   the \tkzname{tkz-berge.sty} package. Special cases include  the triangle graph and  the square graph.}

\medskip
External links :

\medskip
\begin{itemize}

\item \href{http://mathworld.wolfram.com/CycleGraph.html}%
           {\textcolor{blue}{MathWorld - CycleGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}

\item  \href{http://en.wikipedia.org/wiki/Cycle_graph}%
            {\textcolor{blue}{Wikipedia}}

\end{itemize}
\end{NewMacroBox} 

\subsubsection{Special cases : the triangle graph and  the square graph}


\begin{center}
\begin{tkzexample}[small]
\begin{tikzpicture}
    \GraphInit[vstyle=Shade] 
    \grCycle[prefix=a,RA=3]{5}
    \grCycle[x=4,y=3,prefix=b,RA=2]{3}
    \grCycle[prefix=d,y=6,rotation=30,RA=2]{4}
\end{tikzpicture}
\end{tkzexample} 
\end{center}
 
\newpage
\subsubsection{Complete graph} 
\begin{NewMacroBox}{grComplete}{\oarg{local options}\var{order}}

\medskip
\emph{The more simple definition is "an undirected graph with an edge between every pair of vertices"  or a complete graph  is a simple graph  in which each pair of graph vertices is connected by an edge. The complete graph  with  $n$ graph vertices is denoted $K_n$.  This graph has $\frac{n(n-1)}{2}$ undirected edges.\\
Geometrically, $K_3$ relates to a triangle,$ K_4$ a tetrahedron is the tetrahedral graph  as well as the wheel graph , $K_5$ a pentachoron, etc \dots}

\medskip
External links :

\medskip
\begin{itemize}

\item  \href{http://en.wikipedia.org/wiki/Complete_graph}%
            {\textcolor{blue}{Wikipedia}}

\item \href{http://mathworld.wolfram.com/grComplete.html}%
           {\textcolor{blue}{MathWorld - Complete graph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
\end{itemize}
\end{NewMacroBox} 


\subsubsection{Complete Graph order 4}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \renewcommand*{\VertexBallColor}{green!50!black}
  \GraphInit[vstyle=Shade]
  \grComplete[RA=5]{7}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\vfill\newpage\null 

\subsubsection{Complete Graph order 4}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \renewcommand*{\VertexBallColor}{green!50!black}
   \GraphInit[vstyle=Shade]
   \SetVertexNoLabel
   \grComplete[RA=7]{16}
\end{tikzpicture}
\end{tkzexample}
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Circulant graph}
\begin{NewMacroBox}{grCirculant}{\oarg{local options}\var{order}}

\medskip
\emph{The circulant graph  is defined for any order $n$ at least 3, and every subset $L$ of integers which are less than or equal to $n/2$.  A circulant graph is a graph  in which the $i$th graph vertex is adjacent to the ($i+j$)th and ($i-j$)th graph vertices for each $j$ in a list $L$ . The circulant graphs with $L=\{1;\dots;[n/2]\}$  gives the complete graphs  and the circulant graph with $L=\{1\}$  gives the cyclic graphs. The Möbius ladders are examples of circulant graphs.\\
 In graph theory, a graph  whose adjacency matrix is circulant is called a circulant graph.\\
The circulant graph on  vertices on a list of nodes  is implemented as \tkzcname{grCirculant} in the \tkzname{tkz-berge.sty} package.}

\medskip
External links :

\href{http://mathworld.wolfram.com/CirculantGraph.html}%
           {\textcolor{blue}{MathWorld - CirculantGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{E.Weisstein}}
\end{NewMacroBox}

\tikzset{VertexStyle/.style = {shape        = circle,
                               shading      = ball,
                               ball color   = green!40!black,%
                               minimum size = 16pt,%
                               draw}}
\SetUpEdge[style = {thick,%
                    double          = orange,%
                    double distance = 1pt}]

\SetVertexNoLabel
\tikzset{EdgeStyle/.style = {thick,
                             double= orange,
                             double distance = 1pt}} 

\subsubsection{ \opt{Graph  order 5 with L=\{1\}}}

This is a cycle graph.

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCirculant[RA=3]{5}{1}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{\opt{Graph  order 5 with L=\{2\}}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCirculant[RA=3]{5}{2}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{\opt{Graph  order 5 with L=\{1,2\}}}

This graph is complete with an order $5$.

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCirculant[RA=3]{5}{1,2}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{\opt{Graph  order 10 with L=\{1,2,3,4,5\}}}

This graph is also complete

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
    \grCirculant[RA=4]{10}{1,2,3,4,5}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

It's interesting to remark that the numbers 3 and 10 are primer, so if $L=\{3\} $ the graph is containing an Eulerian circuit.
 

\subsubsection{\opt{Graph  order 10 with L=\{3\}}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
    \grCirculant[RA=4]{10}{3}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill\newpage\null 
\tikzset{VertexStyle/.style = {shape           = circle,
                               shading         = ball,
                               ball color      = gray!30,%
                               minimum size    = 24pt,%
                               draw}}
\tikzset{EdgeStyle/.style = {thick,%
                               double          = orange,%
                               double distance = 1pt}} 
\SetVertexMath

\subsubsection{\opt{Graph  order 21 with L=\{1,3,10\}}}

\SetVertexNoLabel
\begin{tikzpicture}
  \grCirculant[Math,RA=7]{21}{1,3,10}
\end{tikzpicture}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––   STAR    –––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\newpage 
\subsubsection{Star graph}  

\begin{NewMacroBox}{grStar}{\oarg{local options}\var{order}}

\medskip
\emph{A star graph $S_n$ is a n-graph   with one node having vertex degree $n-1$  and the other $n-1$   having vertex degree $1$. Star graphs can be generated using \tkzcname{grStar} in   the \tkzname{tkz-berge.sty} package.}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/StarGraph.html}%
           {\textcolor{blue}{MathWorld - StarGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}

\tikzset{VertexStyle/.style = {shape        = circle,
                                 shading      = ball,
                                 ball color   = orange!40!,%
                                 minimum size = 26pt,%
                                 draw}}
\SetUpEdge[style={thick,%
           double          = orange,%
           double distance = 1pt}]
\SetVertexNoLabel
\tikzset{EdgeStyle/.style = {thick,
                             double= orange,
                             double distance = 1pt }}

\subsubsection{Star graph}
\begin{center}
  \begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=30,scale=.8]
  \grStar[RA=7]{8}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Square graph} 

 \begin{NewMacroBox}{grSQCycle}{\oarg{local options}\var{Number}}

\medskip
\emph{A star graph $S_n$ is a n-graph   with one node having vertex degree $n-1$  and the other $n-1$   having vertex degree $1$. Star graphs can be generated using \tkzcname{grStar} in   the \tkzname{tkz-berge.sty} package.}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/SquareGraph.html}%
           {\textcolor{blue}{MathWorld - SquareGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}

\subsubsection{Square Cycle graph}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.8]
  \grSQCycle[RA=7]{10}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––     WHEEL     –––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Wheel graph} 

\begin{NewMacroBox}{grWheel}{\oarg{local options}\var{Number}}

\medskip
\emph{A wheel graph   of order $n$  is a graph that contains a cycle of order $n-1$, and for which every  vertex in the cycle is connected to one other  vertex. The wheel  can be defined as the graph , where  is the singleton graph and  is the cycle graph.}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/WheelGraph.html}%
           {\textcolor{blue}{MathWorld - WheelGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}

\tikzset{VertexStyle/.style = {shape        = circle,
                               shading      = ball,
                               ball color   = orange!40,%
                               minimum size = 24pt,%
                               draw}}
\SetUpEdge[style={thick,%
                  double          = orange,%
                  double distance = 1pt}]

\SetVertexNoLabel
\tikzset{EdgeStyle/.style = {thick,double= orange,double distance = 1pt}}
 
\vfill
\subsubsection{\tkzname{Wheel graph}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[scale=.8]
      \grWheel[RA=7]{13}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––      LADDER        ––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Ladder graph} 

\begin{NewMacroBox}{grLadder}{\oarg{local options}\var{Number}}

\medskip
\begin{tabular}{llc}
 \toprule   
options   & default  & definition                                           \\
\midrule
\TOline{RA     } { |4|    } {radius  circle n°1   }
\TOline{RS     } { |0|    } {distance between two lines } 
\TOline{prefix } { |a|    } {prefix for vertices        } 
\TOline{prefixx} { |b|    } {prefix for vertices        }       
\TOline{Math   } { |false|} {math mode                  }       
\bottomrule     
\end{tabular}

\medskip
\emph{The ladder graph $L_n$ or cyclic ladder graph is  equivalent to the grid graph  having two rails and $n$ rungs between them.}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/LadderGraph.html}%
           {\textcolor{blue}{MathWorld - LadderGraph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}

\vfill
\subsubsection{\tkzname{Ladder graph}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
      \grLadder[RA=2,RS=4]{6}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––  Prism CYCLE LADDER     –––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Prism graph} 

\begin{NewMacroBox}{grPrism}{\oarg{local options}\var{Number}}
  
\medskip
\begin{tabular}{llc}
 \toprule   
options   & default  & definition                                           \\
\midrule
\TOline{RA      } { |4|    }  {radius  circle n°1  }                             
\TOline{RB      } { |3|    }  {radius  circle n°2  }                             
\TOline{prefix  } { |a|    }  {prefix for vertices }                        
\TOline{prefixx } { |b|    }  {prefix for vertices }                 
\TOline{Math    } { |false|}  {math mode           }    
\bottomrule
\end{tabular}

\medskip
\emph{An $n$-prism graph has $2n$  nodes and $3n$ edges, and is equivalent to the generalized Petersen graph with arguments $n$ and $1$. For odd $n$, the $n$-prism is isomorphic to the circulant graph with an order $2n$ and with arguments $2$ and $n$.\\
The 3-prism graph   is the line graph of the complete bipartite graph with arguments $2$ and $3$ . The 4-prism graph  is isomorphic with the cubical graph.}


\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/PrismGraph.html}%
           {\textcolor{blue}{MathWorld - Prism Graph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}

\subsubsection{\tkzname{Cycle Ladder graph}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}[rotate=15,scale=.7]
  \grPrism[RA=6,RB=3]{6}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{\tkzname{Cycle Ladder graph number 3}}
\begin{center}
\begin{tkzexample}[]
\begin{tikzpicture}[scale=.7]
  \grPrism[RA=6,RB=3]{3}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{\tkzname{Cycle Ladder graph number 4}}
\begin{center}
\begin{tkzexample}[]
\begin{tikzpicture}[scale=.7] 
  \grPrism[RA=6,RB=3]{4}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––   bipartite ––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Complete Bipartite graph} 

\begin{NewMacroBox}{grCompleteBipartite}{\oarg{local options}\var{Number 1}\var{Number 2}}

\medskip
\begin{tabular}{llc}
 \toprule   
options   & default  & definition                                           \\
\midrule
\TOline{RA     }{|4|     } {radius  circle n°1}    
\TOline{RB     }{|3|     } {radius  circle n°2 }  
\TOline{RS     }{|1|     } {distance between two lines }
\TOline{form   }{|1|     } {integer to obtain a new embedding of a graph}
\TOline{prefix }{|a|     } {prefix for vertices  }
\TOline{prefixx}{|b|     } {prefix for vertices }
\TOline{Math   }{|false| } {math mode }
\bottomrule
\end{tabular}

\medskip
\emph{A complete bipartite graph is a bipartite graph (i.e., a set of graph vertices decomposed into two disjoint sets such that no two graph vertices within the same set are adjacent) such that every pair of graph vertices in the two sets are adjacent.}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/CompleteBipartiteGraph.html}%
           {\textcolor{blue}{MathWorld - CompleteBipartite Graph}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox}   



\subsubsection{\tkzname{Bipartite graph 1,5}}\label{cl17}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCompleteBipartite[RA=4,RB=2.5,RS=4]{1}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{\tkzname{Bipartite graph 3,5}}\label{bi1}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \grCompleteBipartite[RA=4,RB=3,RS=6]{3}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{Triangular Grid graph} 


\begin{NewMacroBox}{grTriangularGrid}{\oarg{local options}\var{Number}}

\medskip
\begin{tabular}{llc}
 \toprule   
options   & default  & definition                                           \\
\bottomrule
\TOline{RA    }{|4|    }{distance between two vertices   }
\TOline{form  }{|1|    }{integer to obtain a new embedding of a graph} 
\TOline{prefix}{|a|    }{prefix for vertices }
\TOline{Math  }{|false|}{math mode  }
\bottomrule
\end{tabular}

\emph{\tkzname{Number=$n$} is the number of vertices of the first row then the graph order is $\dfrac{n(n-1)}{2} $.
There are three embeddings. You can use the option \tkzname{form} with an integer between $1$ and $3$.}
\end{NewMacroBox} 

\medskip


\subsubsection{\opt{n=8 order=$28$} form 1}\label{cl18a}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \SetVertexLabel
  \grTriangularGrid[prefix=G,Math,RA=1.5]{8}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{\opt{n=6 order=$15$} form 2}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \SetVertexNoLabel
  \grTriangularGrid[RA=2,form=2]{6}%
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{\opt{n=6 order=$15$} form 3}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \SetVertexNoLabel
  \grTriangularGrid[RA=2,form=3]{6}%
\end{tikzpicture}
\end{tkzexample}
\end{center}
%<––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\newpage 
\subsubsection{\tkzname{LCF Lederberg-Coxeter-Fruchte}}   

\begin{NewMacroBox}{grLCF}{\oarg{RA=\meta{Number}}  \var{List of numbers} \var{Number}}
\emph{LCF = Lederberg-Coxeter-Fruchte (see the link below for some examples).}

\medskip
External links :

\medskip
\begin{itemize}
\item \href{http://mathworld.wolfram.com/LCFNotation.html}%
           {\textcolor{blue}{MathWorld-LCF Notation}} by %
      \href{http://en.wikipedia.org/wiki/Eric_W._Weisstein}%
           {\textcolor{blue}{Weisstein}}
\end{itemize}
\end{NewMacroBox} 


\subsubsection{\tkzname{$\big[2,-2\big]^2$}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
       \grLCF[RA=5]{2,-2}{2}%
\end{tikzpicture}
\end{tkzexample}
\end{center}



\subsubsection{\tkzname{$\big[3,-3\big]^4$}}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}%
       \grLCF[RA=5]{3,-3}{4}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Ljubljana graph}
From Wikipedia \url{http://en.wikipedia.org/wiki/Ljubljana_graph}

\emph{The Ljubljana graph was first published in 1993 by Brouwer, Dejter and Thomassen.
In 1972, Bouwer was already talking of a 112-vertices edge- but not vertex-transitive cubic graph found by R. M. Foster, but unpublished. Conder, Malnič, Marušič, Pisanski and Potočnik rediscovered this 112-vertices graph in 2002 and named it the Ljubljana graph after the capital of Slovenia. They proved that it was the unique 112-vertices edge- but not vertex-transitive cubic graph and therefore that was the graph found by Foster.} 

It can be   represented in LCF notation as  :

\[ 
\begin{array}{l}
\Big[ 47, -23, -31, 39, 25, -21, -31, -41, 25, 15, 29, -41, -19, 15, -49, 33, 39, -35, -21, 17,\\ -33, 49, 41, 31, -15, -29, 41, 31, -15, -25, 21, 31, -51, -25, 23, 9, -17, 51, 35, -29, 21,\\ -51, -39, 33, -9, -51, 51, -47, -33, 19, 51, -21,29, 21, -31, -39\Big]^2 
\end{array} 
\]   

   
  \begin{center}
\begin{tikzpicture}
\GraphInit[vstyle=Art]
\SetGraphArtColor{black!50}{darkgray}
\tikzset{VertexStyle/.append style = {
                               minimum size         =  3pt}} 
       \grLCF[RA=7]{47, -23, -31, 39, 25, -21, -31, -41, 25, 15, 29, -41, -19, 15, -49, 33, 39, -35, -21, 17, -33, 49, 41, 31, -15, -29, 41, 31, -15, -25, 21, 31, -51, -25, 23, 9, -17, 51, 35, -29, 21, -51, -39, 33, -9, -51, 51, -47, -33, 19, 51, -21, 29, 21, -31, -39}{2}%  
\end{tikzpicture}
\end{center} 

\begin{tkzexample}[code only]
\GraphInit[vstyle=Art]
\SetGraphArtColor{black!50}{darkgray}
\tikzset{VertexStyle/.append style = {
                               minimum size         =  3pt}} 
\begin{tikzpicture}%
 \grLCF[RA=7]{47, -23, -31, 39, 25, -21, -31, -41, 25, 15, 29, -41, -19, 15,%
  -49, 33, 39, -35, -21, 17, -33, 49, 41, 31, -15, -29, 41, 31, -15, -25, 21,%
   31, -51, -25, 23, 9, -17, 51, 35, -29, 21, -51, -39, 33, -9, -51, 51, -47,%
    -33, 19, 51, -21, 29, 21, -31, -39}{2}%    
\end{tikzpicture}
\end{tkzexample} 
\vfill
\endinput


==> tkz-berge/doc/latex/TKZdoc-berge-installation.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/doc-us/TKZdoc-berge-main.tex

\section{Installation}
\subsection{How to install the package \texttt{\textcolor{red}{berge.sty}}}


It is possible that when you read this document, \tkzname{tkz-berge} is present on the \tkzname{CTAN}\footnote{\tkzname{tkz-berge} is not still a part of \tkzname{TeXLive} but it will  be soon possible to install it with \tkzname{tlmgr}} servers.  If \tkzname{tkz-berge} is not still a part of your distribution, this chapter  shows you how to install it. 

\subsection{With TeXLive under OS X and Linux}\NameDist{TeXLive}

You could simply  create a folder (directory) \tikz[remember picture,baseline=(n1.base)]\node [fill=green!20,draw] (n1) {tkz};  which path is : \colorbox{blue!20}{ texmf/tex/latex/tkz}. 

\colorbox{blue!20}{texmf} is generally the personnal folder. For example the paths of this folder on my two computers are

\medskip
\begin{itemize}\setlength{\itemsep}{10pt}
\item   with OS X\NameSys{OS X} \colorbox{blue!20}{\textbf{/Users/ego/Library/texmf}}; 
\item   with Ubuntu\NameSys{Linux Ubuntu} \colorbox{blue!20}{\textbf{/home/ego/texmf}}.
\end{itemize}

If you choose a custom location for  your files, I suppose that you know why!
The installation that I propose, is valid only for one user.
 

\medskip
\begin{enumerate}
\item Store the files \tikz[remember picture,baseline=(n2.base)]\node [fill=green!20,draw] (n2) {tkz-arith.sty, tkz-graph.sty et tkz-berge.sty}; in the folder  \colorbox{green!50}{prof}. Be careful to have the file \tkzname{tkz-tool-arith.tex}. This file is provided by \tkzname{tkz-base}.
\item Open a terminal, then type \colorbox{red!20}{|sudo texhash|}
\item Check that \tkzname{xkeyval}\index{xkeyval} version 2.5 or more, and \tkzname{Ti\emph{k}Z 2.1}\index{TikZ@Ti\emph{k}Z} are installed because they are obligatory.\\

\end{enumerate}

\medskip
My folder texmf is structured as in the diagram below because I use the \tkzname{CVS}\footnote{You can find the cvs version here : \url{http://www.texample.net/tikz/builds/} without CVS\\ or here with CVS \url{http://sourceforge.net/projects/pgf/}} version of \TIKZ. You don't need all the \tkzname{pgf} folders.

\medskip

\vfill
\begin{tikzpicture} [remember picture,rotate=90] 
% nodes
\node (texmf)   at (4,2)   [draw,fill=blue!20 ] {texmf};

\node (tex)     at (6,0)   [draw ] {tex}; 
\node (doc)     at (2,0)   [draw ] {doc};

\node (texgen)  at (7,-2)  [draw ] {generic};
\node (docgen)  at (0,-2)  [draw ] {generic};

\node (latex)   at (4,-2)  [draw ] {latex}; 

\node (genpgf)  at (7,-4)  [draw] {pgf};
\node (latpgf)  at (5,-4)  [draw] {pgf};
\node (tkz)     at (4,-4)  [draw,fill=green!20 ] {tkz};

\node (docpgf)  at (0,-4)  [draw] {pgf};

\node (tkb)     at (6,-6)  [draw,fill=orange!20]  {tkzbase};
\node (tke)     at (2,-6)  [draw,fill=orange!20]  {tkzeuclide};

\node (tari)    at (7,-11)  [draw,fill=orange!20] {tkz-tools-arith.tex};   
\node (tary)    at (5,-11)  [draw,fill=green!20]  {tkz-arith.sty};
\node (tgra)    at (4,-11)  [draw,fill=green!20]  {tkz-berge.sty}; 
\node (tber)    at (3,-11)  [draw,fill=green!20]  {tkz-graph.sty};

% edges
\draw[-open triangle 90](texmf.north east) -- (tex.south west)    ;
\draw[-open triangle 90](texmf.south east) -- (doc.north west)    ;
                                                                  
\draw[-open triangle 90](tex.north east)   -- (texgen.south west) ;
\draw[-open triangle 90](tex.south east)   -- (latex.north west)  ; 
\draw[-open triangle 90](texgen.east)      -- (genpgf.west)       ;  
                                                                  
\draw[-open triangle 90](doc.south east)   -- (docgen.north west) ; 
\draw[-open triangle 90](docgen.east)      -- (docpgf.west)       ; 

\draw[-open triangle 90](latex.north east) -- (latpgf.south west) ; 
\draw[-open triangle 90](latex.east)       -- (tkz.west)          ;    
 
\draw[-open triangle 90,orange!80](tkz.east) to [out=-90,in=90](tkb.west)  ; 
\draw[-open triangle 90,orange!80](tkz.east) to [out=-90,in=90](tke.west)  ; 
\draw[-open triangle 90,orange!80](tkb.east) to [out=-90,in=90](tari.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tary.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tgra.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tber.west) ;  

\end{tikzpicture}

\begin{tikzpicture}[remember picture,overlay]
        \path[->,thin,green!80,>=latex] (n1) edge [bend left] (tkz);
        \path[->,thin,green!80,>=latex] (n2) edge [bend left] (tgra);
\end{tikzpicture}     

\vfill
\newpage

\subsection{How to work with the tkz-\LaTeX-package under Windows?}
\NameDist{MikTeX}\NameSys{Windows XP}
Download and install the following files (if not yet done):
\begin{enumerate}

  \item the \LaTeX-system MiKTeX from

      \url{http://www.miktex.org/}.

      What file you need (e.g.
      \texttt{basic-miktex-2.7.2904.exe}) and how to install
      this program is explained there in the "Download"
      section of the respective version (current version is
      2.7). In general and as usual in windows, you run the
      setup process by starting the setup file :\newline (e.g.\texttt{basic-miktex-2.7.2904.exe}).

  \item Till Tantau's \LaTeX-package \texttt{pgf-tikZ} from

      \url{http://sourceforge.net/projects/pgf/}

      "For MiKTeX, use the update wizard [of MiKTeX] to
      install the (latest versions of the) packages called
      \texttt{pgf}, \texttt{xcolor}, and \texttt{xkeyval}."
      (cited from the pgf manual, contained in the files
      downloaded).
       \item the sty-files and the doc-files of Alain's tkz-package
            from the CTAN servers or

            \url{http://www.altermundus.fr/pages/download.html}.
                
      or
      
      \url{http://altermundus.com/pages/downloads/index.html}.
      
            To add the files to MiKTeX:

            \begin{itemize}
              \item add a directory \texttt{prof} in the
                  directory \colorbox{blue!30}{\texttt{[MiKTeX-dir]/tex/latex}},
                  e.g. in windows explorer,
              \item copy the sty-files in this directory
                  \texttt{tkz},
              \item update the MiKTeX system, ether by running
                  in a DOS shell the command\newline "\colorbox{red!30}{|mktexlsr -u|}" \newline or by clicking\newline
                  "\colorbox{red!30}{|Start/Programs/Miktex/Settings/General|}", then
                  push the button \colorbox{red!30}{|Refresh FNDB|}.
            \end{itemize}
      \end{enumerate}

\subsection{The next version} 

Actually, the package uses \tkzname{xkeyval}, in the next version I will use \tkzname{pgfkeys}. It's possible that the syntax should be modified. My first idea is to keep \tkzname{tkz-graph} and to create a new name for the next version like  \tkzname{tkz-graph-x}.

Some of the main macros used in the file \tkzname{tkz-tool-arith.tex} are now in the CVS version of PGF. With the next version of PGF, it would be possible to remove the   file \tkzname{tkz-tool-arith.tex}.
\endinput


==> tkz-berge/doc/latex/TKZdoc-berge-macros-e.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/doc-us/TKZdoc-berge-main.tex 

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\section{Macros and Edges in a graph}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Edge in a graph from one vertex \tkzcname{EdgeInGraphFromOneToComp}}

\begin{NewMacroBox}{EdgeInGraphFromOneToComp}{\oarg{local options}\var{prefix}\var{order}\var{from}}
   
\begin{tabular}{llc}
\hline
Arguments   &   & Definition              \\
\midrule
\TAline{order} {}{order of the graph}  
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{llc}
\midrule
options   & default  & definition                                           \\
\midrule
\TOline{RA}     {4}      { radius  circle}            
\TOline{prefix} {a}      {prefix for vertices }       
\TOline{Math}   {false}  {math mode }                
\bottomrule
\end{tabular}

\medskip
\emph{This macro works on an unique graph. |from| is integer. |EdgeInGraph| designs a macro that works only in a graph defined by a prefix. The result is some edges between the vertex |from| and the others vertices. }
\end{NewMacroBox}





\subsubsection{Empty Cycle}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=4,prefix=a]{8}% 
  \EdgeInGraphFromOneToComp{a}{8}{3} 
\end{tikzpicture}
\end{tkzexample}
\end{center}
 
\vfill
\newpage
\subsection{Edges in a graph - a loop \tkzcname{EdgeInGraphLoop}}%
\begin{NewMacroBox}{EdgeInGraphLoop}{\var{prefix}\var{order}}
\emph{This macro is useful with vertices on a circle . |order| in an integer.}
\end{NewMacroBox} 


\subsubsection{Empty Cycle}
\begin{center}
  \begin{tkzexample}[very small]
  \begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=2,prefix=a]{8}% 
  \EdgeInGraphLoop{a}{8} 
  \end{tikzpicture}\end{tkzexample}
\end{center}

\subsubsection{Empty Cycle}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}[node distance=4cm]
 \GraphInit[vstyle=Shade]
 \Vertices{square}{a0,a1,a2,a3}
 \EdgeInGraphLoop{a}{4}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage
\subsection{Edges in a graph - a loop \tkzcname{EdgeInGraphLoop*}}
\begin{NewMacroBox}{EdgeInGraphLoop*}{\var{prefix}\var{order}}

\medskip
\emph{Not exactly a loop, there is no edge between the first and the last vertex.}
\end{NewMacroBox}

\subsubsection{Empty Cycle}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \grEmptyCycle[RA=4,prefix=a]{8}% 
  \EdgeInGraphLoop*{a}{8} 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Path}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
     \grEmptyPath[prefix=h,RA=2,RS=2]{6}
     \EdgeInGraphLoop*{h}{6}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill
\newpage  
\subsection{Sequence of edges in a graph  \tkzcname{EdgeInGraphSeq}}
\begin{NewMacroBox}{EdgeInGraphSeq}{\var{prefix}\var{start}\var{end}}

\medskip
\emph{This macro gives a sequence of edges between |start| and |end|.\\
|start| and |end| are  two integers. }
\end{NewMacroBox} 

\subsubsection{EdgeInGraphSeq}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=2,prefix=a]{8}% 
  \EdgeInGraphSeq{a}{2}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center} 

\newpage
\subsection{Edges in a graph  \tkzcname{EdgeInGraphMod}}
\begin{NewMacroBox}{EdgeInGraphMod}{\var{prefix}\var{order}\var{add}}

\medskip
\emph{This macro works on an unique graph. Edges between $v_i$ and $v_j$ with $i$ in $0,...,(\text{\#2}-1)$  and $j=\text{Mod(i+\#3,\#2)}$.\\
\#2 = |order| and  \#3 = |add|.\\
|Mod| is like |mod| but the result is a positive integer. }
\end{NewMacroBox} 

\subsubsection{EdgeInGraphMod}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=2,prefix=a]{8}% 
  \EdgeInGraphMod{a}{8}{2}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{EdgeInGraphMod 2}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=3,prefix=a]{13}% 
  \EdgeInGraphMod{a}{13}{3}
\end{tikzpicture}
\end{tkzexample}
\end{center}
 
\newpage
\subsection{Edges in a graph  \tkzcname{EdgeInGraphMod*}}
\begin{NewMacroBox}{EdgeInGraphMod*}{\var{prefix}\var{order}\var{add}\var{start}\var{step}}

\medskip
\emph{Edges between $v_i$ and $v_j$ with $i$ in $\#4,\#4+\#5,...,(\text{\#2}-1)$  and $j=\text{Mod(i+\#3,\#2)}$}\\
\#2 = |order|,  \#3 = |add|, \#4 = |start|, \#5 = |step|.\\
\end{NewMacroBox} 

\subsubsection{EdgeInGraphMod*}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[prefix=a]{17}% 
  \EdgeInGraphMod*{a}{17}{5}{1}{2}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage
\subsection{Edges in a graph  \tkzcname{EdgeInGraphModLoop}}
\begin{NewMacroBox}{EdgeInGraphModLoop}{\var{prefix}\var{order}\var{add}\var{start}}

\medskip
\emph{ |order|, |add| and |start| are integers.\\
Edges between $v_i$ and $v_j$ with $i$ from $\#4$, $j=\text{Mod(i+\#3,\#2)}$ and then $i=j$ until $j=\#4$\\
\#2 = |order|,  \#3 = |add| and \#4 = |start|.}
\end{NewMacroBox}

\subsubsection{EdgeInGraphModLoop}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=4]{7} 
  \EdgeInGraphModLoop{a}{7}{2}{1} 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{EdgeInGraphModLoop}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=4]{8} 
  \EdgeInGraphModLoop{a}{8}{2}{1} 
\end{tikzpicture}
\end{tkzexample}
\end{center}


\newpage
\subsection{Edges between two graphs with the same order \tkzcname{EdgeIdentity}}

\begin{NewMacroBox}{EdgeIdentity}{\var{prefix1}\var{prefix2}\var{order}}

\medskip
\emph{|order| is an integer. This macro gives edges between two graphs.\\
Edges between $v_i$ and $v_j$ with $i=j$ in $0,...,(\text{\#3}-1)$.\\
\#3 = |order|.\\}
\end{NewMacroBox}  

\subsubsection{EdgeIdentity}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
    \grEmptyCycle[prefix=v,RA=3]{5}
    \grEmptyCycle[prefix=w,RA=1]{5}
    \EdgeIdentity{v}{w}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}
 
\vfill
\newpage  
\subsection{Edges between two graphs with the same order \tkzcname{EdgeIdentity*}}

\begin{NewMacroBox}{EdgeIdentity*}{\var{prefix1}\var{prefix2}\var{list}}

\medskip
\emph{|list| is a list of  integers. This macro gives edges between two graphs.\\
Edges between $v_i$ and $v_j$ with $i=j$ in |list|.\\}

\end{NewMacroBox}

\subsubsection{EdgeIdentity*}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \begin{scope}[rotate=30]
  \grEmptyCycle[RA=3,prefix=a]{5}%
  \end{scope}
  \grEmptyCycle[RA=5,prefix=b]{5}%
   \EdgeIdentity*{a}{b}{0,...,4}    
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{EdgeIdentity*}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
 \GraphInit[vstyle=Shade]
  \begin{scope}[rotate=30]
  \grEmptyCycle[RA=3,prefix=a]{5}%
  \end{scope}
  \grEmptyCycle[RA=5,prefix=b]{5}%
   \EdgeIdentity*{a}{b}{0,2,4}    
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage
\subsection{Edges between two graphs \tkzcname{EdgeFromOneToAll}}
\begin{NewMacroBox}{EdgeFromOneToAll}{\var{prefix1}\var{prefix2}\var{from}\var{order}}

\medskip
\emph{The graphs must to have the same order. |from| and |order| are integers.}
\end{NewMacroBox}

\subsubsection{EdgeFromOneToAll}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grPath[form=1,RA=2,RS=0]{5}
  \grPath[form=1,prefix=b,RA=2,RS=4]{5}
  \EdgeFromOneToAll{a}{b}{1}{5} 
\end{tikzpicture}\end{tkzexample}
\end{center}

\newpage
\subsection{Edges between two graphs \tkzcname{EdgeFromOneToSeq}}
\begin{NewMacroBox}{EdgeFromOneToSeq}{\var{prefix1}\var{prefix2}\var{from}\var{start}\var{end}}

\medskip
\emph{|from|, |start| and |end| are integers. This macro  builds edges between the vertex with an indice |from| through the vertices with an indice in the sequence |start|,...,|end|.}
\end{NewMacroBox} 

\subsubsection{EdgeFromOneToSeq}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grPath[form=1,RA=2,RS=0]{5}
  \grPath[form=1,prefix=b,RA=2,RS=4]{5}
  \EdgeFromOneToSeq{a}{b}{1}{2}{4} 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage
\subsection{Edges between two graphs \tkzcname{EdgeFromOneToSel}}
\begin{NewMacroBox}{EdgeFromOneToSel}{\var{prefix1}\var{prefix2}\var{from}\var{list}}

\medskip
\emph{This macro  builds edges between the vertex with an indice |from| through the vertices with an indice in the list |list|.}
\end{NewMacroBox} 


\subsubsection{EdgeFromOneToSel}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grPath[form=1,RA=2]{5}
  \grPath[form=1,prefix=b,RA=2,RS=4]{5} 
  \EdgeFromOneToSel{a}{b}{1}{0,2,4} 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage  
\subsection{Edges between two graphs \tkzcname{EdgeFromOneToComp}}
\begin{NewMacroBox}{EdgeFromOneToComp}{\var{prefix1}\var{prefix2}\var{from}\var{order2}}

\medskip
\emph{This macro  builds edges between the vertex with an indice |from| through all the vertices of the second graph, except the vertex with an indice |from|.}
\end{NewMacroBox}  

\subsubsection{EdgeFromOneToComp}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grPath[form=1,RA=2,RS=0]{5}
  \grPath[form=1,prefix=b,RA=2,RS=4]{5}
  \EdgeFromOneToComp{a}{b}{2}{3} 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage  
\subsection{Edges between two graphs \tkzcname{EdgeMod}}%
\begin{NewMacroBox}{EdgeMod}{\var{prefix1}\var{prefix2}\var{order}\var{step}}

\medskip
\emph{This macro works on two graphs with the same order. We get edges between $v_i$ and $v_j$ with $i$ in $0,...,(\text{\#2}-1)$  and $j=\text{Mod(i+\#4,\#3)}$.\\
\#3 = |order| and  \#4 = |step|.}
\end{NewMacroBox}  

\subsubsection{EdgeMod}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
 \GraphInit[vstyle=Shade]
 \grEmptyCycle[prefix=a,RA=6]{9}
 \grEmptyCycle[prefix=b,RA=3]{9}
 \EdgeMod{a}{b}{9}{1}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage  
\subsection{Edges between two graphs \tkzcname{EdgeMod*}}%
\begin{NewMacroBox}{EdgeMod*}{\var{prefix1}\var{prefix2}\var{order}\var{step1}\var{step2}}

\medskip
\emph{This macro works on two graphs with the same order. We get edges between $v_i$ and $v_j$ with $i$ in $0,...,(\text{\#3}-1)$ with a step $\text{\#5}$ and $j=\text{Mod(i+\#4,\#3)}$.\\
\#3 = |order| ,  \#4 = |step1| and \#5 = |step2|.}
\end{NewMacroBox}  


\subsubsection{\tkzcname{EdgeMod*} }%with |step1|=1 and |step2|=2
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
 \GraphInit[vstyle=Shade]
 \grEmptyCycle[prefix=a,RA=6]{8}
 \grEmptyCycle[prefix=b,RA=4]{8}
 \EdgeMod*{a}{b}{8}{1}{2}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{EdgeMod* }%with |step1|=2 and |step2|=1
\begin{center}
\begin{tkzexample}[vbox] 
\begin{tikzpicture}
 \GraphInit[vstyle=Shade]
 \grEmptyCycle[prefix=a,RA=6]{8}
 \grEmptyCycle[prefix=b,RA=2]{8}
 \EdgeMod*{a}{b}{8}{1}{1}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage  
\subsection{Edges between two graphs \tkzcname{EdgeDoubleMod}}%
\begin{NewMacroBox}{EdgeDoubleMod}{\var{prefix1}\var{nb}\var{nb}\var{nb}\var{prefix2}\var{nb}\var{nb}\var{nb}\var{end}}

For the first node,  the numbers are :
\var{order1}\var{start1}\var{add1}

\medskip  
For the second node,  the numbers are :  
\var{order2}\var{start2}\var{add2}\var{end} 
  
\medskip
\emph{Edges between $v_i$ and $v_j$ with $i=\text{Mod(\#3+(\#4*k),\#2)}$ and j=$\text{Mod(\#7+(\#8*k),\#6)}$ $k$ is an integer from $0$ to |end|.\\
\#2 = |order1|,  \#3 = |start1| and \#4 = |add1|.\\
\#6 = |order2|,  \#7 = |start2| and \#8 = |add2|.}
\end{NewMacroBox} 


\subsubsection{EdgeDoubleMod}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
    \begin{scope}[rotate=-90]
      \grEmptyCycle[RA=2,prefix=a]{5}{2}
    \end{scope}
    \begin{scope}[rotate=-18]
      \grEmptyCycle[RA=4,prefix=b]{5}{2}
    \end{scope}
    \EdgeDoubleMod{b}{5}{0}{1}%
                 {a}{5}{2}{1}{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{EdgeDoubleMod with two graphs and different orders}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[prefix=a,RA=5]{10}
  \grEmptyCycle[prefix=b,RA=7]{20}
   \EdgeDoubleMod{a}{10}{0}{1}%
                 {b}{20}{0}{2}{10}
\end{tikzpicture}
\end{tkzexample}
\end{center}
\endinput


==> tkz-berge/doc/latex/TKZdoc-berge-macros.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/doc-us/TKZdoc-berge-main.tex 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\section{Macros and Vertices}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{\tkzcname{grEmptyCycle}}

\begin{NewMacroBox}{grEmptyCycle}{\oarg{local options}\var{order}}
\begin{tabular}{llc}
Arguments   &   & Definition              \\
\midrule
\TAline{order} {}{order of the graph}   
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{llc}

Options   & default  & definition                                           \\
\midrule
\TOline{RA}     {4}      { radius  circle}               
\TOline{prefix} {a}      {prefix for vertices }         
\TOline{Math}   {false}  {math mode }                    
\bottomrule
\end{tabular}

\medskip
\emph{The number of nodes in a graph is called its order. The argument "order" is an integer superior to $1$. |RA| defines the radius of the circle.}
\end{NewMacroBox}


\bigskip
\subsubsection{Empty Cycle}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=1.5]{3}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Cycle  and \tkzcname{SetVertexNoLabel}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \SetVertexNoLabel
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[RA=1.5]{2}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Cycle and \tkzname{Math}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[Math,RA=1.5]{4}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{Empty Cycle, \tkzcname{SetVertexMath} and \tkzname{prefix}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \SetVertexMath
  \GraphInit[vstyle=Shade]
  \grEmptyCycle[prefix=N,RA=1.5]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Cycle and Classic style}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \SetVertexMath
  \GraphInit[vstyle=Classic]
  \grEmptyCycle[RA=1.5]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Cycle and Simple style}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \GraphInit[vstyle=Simple]
  \grEmptyCycle[RA=1.5]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage
\subsection{\tkzcname{grEmptyPath}}
\begin{NewMacroBox}{grEmptyPath}{\oarg{local options}\var{order}}
\begin{tabular}{llc}
\hline
Arguments   &   & Definition              \\
\midrule
\TAline{order} {}{order of the graph}   
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{>{\color{green!50!black}}lllc}
 \toprule 
options   & default  & definition                                           \\
\midrule
\TOline{RA}     {4 cm}{ distance between two vertices}               
\TOline{RS}     {? cm}{ distance between the first line  and the new one}    \\
\TOline{prefix} {a}      {prefix for vertices }          
\TOline{Math}   {false}  {math mode }                   
\bottomrule
\end{tabular}

\medskip
\emph{|Order| is the number of nodes. |RA| defines the radius of the circle.  |RS| defines the distance between the graph and the baseline.}

\end{NewMacroBox}

\bigskip
\tikzset{VertexStyle/.style = {shape        = circle,%
                               shading      = ball,%
                               ball color   = green!30,
                               minimum size = 24pt,
                               draw}}
\tikzset{EdgeStyle=      {color=red!30,
                           double= green!50!black,
                           double distance = 2pt}} 
\SetVertexLabel
\SetVertexMath
\subsubsection{Empty Path,   \tkzname{RA}  and \tkzname{Math}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
   \grEmptyPath[Math,RA=2]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Path,  \tkzname{RA}  and \tkzname{prefix}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
   \grEmptyPath[prefix=h,RA=2]{6}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsubsection{Empty Path, vertical path with \tkzname{form=2}}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
 \grEmptyPath[form=2,prefix=v,RA=2]{3}
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsubsection{Two Empty Paths}
\begin{center}  
\begin{tkzexample}[very small]
\begin{tikzpicture}
    \grEmptyPath[Math,prefix=p,RA=2,RS=0]{5}
    \grEmptyPath[Math,prefix=q,RA=2,RS=3]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\begin{center}  
\begin{tkzexample}[vbox]
\begin{tikzpicture}
    \grEmptyPath[Math,prefix=p,RA=2,RS=0,form=2]{5}
    \grEmptyPath[Math,prefix=q,RA=2,RS=4,form=2]{5}
\end{tikzpicture}
\end{tkzexample}
 \end{center}

\subsubsection{How to move a graph ?}
  \GraphInit[vstyle=Shade]
  \SetGraphShadeColor{blue!60!black!30}{blue}{white}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
     \grPath[Math,prefix=u,RA=2,RS=0]{4}
     \grPath[Math,prefix=v,RA=2,RS=3]{4}
     \begin{scope}[xshift=1 cm]
      \grPath[Math,prefix=t,RA=2,RS=5]{4}
     \end{scope}
     \begin{scope}[shift={(4 cm,8cm)}]
      \grPath[Math,prefix=x,RA=2,RS=0]{4}
     \end{scope}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage 
\subsection{Empty Star}
\begin{NewMacroBox}{grEmptyStar}{\oarg{local options}\var{order}}
\begin{tabular}{llc}
 \toprule 
Arguments   &   & Definition              \\
\midrule
\TAline{order} {}{order of the graph}  
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{>{\color{green!50!black}}lllc}
 \toprule 
options   & default  & definition                                           \\
\midrule
\TOline{RA}     {4 cm}{ radius circle}               
\TOline{prefix} {a}      {prefix for vertices }     
\TOline{Math}   {false}  {math mode }                
\bottomrule
\end{tabular}

\medskip
\emph{|RA| defines the radius of the circle. |order| is an integer and it's the order of the graph.}
\end{NewMacroBox}

\bigskip
\subsubsection{Empty Star}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
  \SetVertexMath
  \grEmptyStar[prefix=s,RA=3]{6}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\newpage 
\subsection{Empty Grid}
\begin{NewMacroBox}{grEmptyGrid}{\oarg{local options}\var{c}\var{r}}
\begin{tabular}{llc}
 \toprule 
Arguments   &   & Definition              \\
\midrule
\TAline{r} {}{number of rows}  
\TAline{c} {} {number of columns}  
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{llc}
 \toprule 
options   & default  & definition                                           \\
\midrule
\TOline{RA}     {4 cm}{ distance between two columns }          
\TOline{RB} {3 cm}      {distance between two rows  }         
\TOline{prefix} {3 cm}      {distance between two rows  }     
\TOline{Math}   {false}  {math mode }                  
\bottomrule
\end{tabular}

\medskip
\emph{|c| and |r| are integers.}

\end{NewMacroBox}

 \bigskip
\subsubsection{Prefix}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
   \tikzset{VertexStyle/.style ={shape        = circle,
                                 shading      = ball,
                                 ball color   = Blue!60,%
                                 minimum size = 24pt,%
                                 draw}}
  \SetVertexMath
  \grEmptyGrid[prefix=G,RA=2,RB=4]{5}{3}
\end{tikzpicture}\end{tkzexample}
\end{center}

\newpage 
\subsection{Empty Ladder}
\begin{NewMacroBox}{grEmptyLadder}{\oarg{local options}\var{c}}
\begin{tabular}{llc}
 \toprule 
Arguments   &   & Definition              \\
\midrule
\TAline{c} {}{number of columns.}  
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{llc}
options   & default  & definition                                           \\
 \midrule 
\TOline{RA}     {4 cm}{ distance between two columns  }           
\TOline{RB}     {3 cm}{ distance between two rows  }               
\TOline{prefix} {a}      {prefix for vertices }         
\TOline{prefix} {b}      {prefix for vertices }         
\TOline{Math}   {false}  {math mode }                    
\bottomrule
\end{tabular}

\medskip
 \emph{ |c| is an integer. There are only two rows with different prefix.}
\end{NewMacroBox}
 
\bigskip
\subsubsection{Empty Ladder}
\begin{center}
\begin{tkzexample}[very small]
\begin{tikzpicture}
   \tikzset{VertexStyle/.style ={shape        = diamond, 
                                 shading      = ball,
                                 ball color   = yellow!60,%
                                 minimum size = 24pt,%
                                 draw}}
   \SetVertexMath
   \grEmptyLadder[RA=2,RB=4]{5}
\end{tikzpicture}
\end{tkzexample}
\end{center}

 
\endinput




==> tkz-berge/doc/latex/TKZdoc-berge-style.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-berge/doc-us/TKZdoc-berge-main.tex 
\section{Macros and Styles}

\subsection{How to change the background color and text color} 

You can use the following macro :

\begin{NewMacroBox}{tkzSetUpColors}{\oarg{local options}}

\begin{tabular}{llc}
  Options   & default  & definition                                  \\
\midrule
\TOline{background}  {white}      {couleur du fond  }             
\TOline{text} {black}   {couleur du texte }                                     
\end{tabular}
\end{NewMacroBox} 




\subsection{Modification of  labels \tkzcname{AssignVertexLabel}}

\begin{NewMacroBox}{AssignVertexLabel}{\oarg{local options}\var{prefix}\var{List of names}}
\begin{tabular}{lll}
  Arguments   &   & example                                  \\
\midrule
\TAline{prefix}        {}    {\tkzcname{AssignVertexLabel\{a\}\{Alter\}}}             
\TAline{List of names} {}    {\tkzcname{AssignVertexLabel\{a\}\{Paris,Lyon\}}}                        
\bottomrule
\end{tabular}

\medskip
\begin{tabular}{llc}
  Options   & default  & definition                                  \\
\midrule
\TOline{size}  {\tkzcname{normalsize}}      {taille de la fonte }             
\TOline{color} {black}   {couleur du texte }                       
\TOline{Math}   {false}  {math mode }                 
\end{tabular}
\end{NewMacroBox}

\medskip
\subsubsection{AssignStyle and \tkzcname{AssignVertexLabel}}
First step : We create an empty graph without labels.

Second step : We place labels with the macro \tkzcname{AssignVertexLabel} \begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetVertexNoLabel
  \grCycle{6}
  \tikzset{AssignStyle/.append style = {below=12pt}}
  \AssignVertexLabel[color = blue,%
                     size  = \footnotesize]{a}{%
   Paris,Lyon,Marseille,Bordeaux,Reims,Saint-Etienne}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\endinput

==> tkz-berge/doc/latex/TKZdoc-gr-installation.tex <==
\chap{Installation}\label{ins}

You could simply  create a folder (directory) \tikz[remember picture,baseline=(n1.base)]\node [fill=green!50,draw] (n1) {prof};  which path is : \colorbox{red!50}{ texmf/tex/latex/prof}. \colorbox{green!50}{texmf} is generally the personnal folder, here ways of this folder on my two computers:

\medskip
\begin{itemize}\setlength{\itemsep}{10pt}
\item   with OS X \colorbox{blue!30}{\textbf{/Users/ego/Library/texmf}}; 
\item   with Ubuntu \colorbox{blue!30}{\textbf{/home/ego/texmf}}.
\end{itemize}

If you choose a custom location for  your files, I suppose that you know why!
The installation that I propose, is valid only for one user.

\medskip
\begin{enumerate}
\item Store the files \tikz[remember picture,baseline=(n2.base)]\node [fill=green!50,draw] (n2) {tkz-arith.sty, tkz-graph.sty and tkz-berge.sty}; in the folder  \colorbox{green!50}{prof}.
\item Open a terminal, then type \colorbox{red!50}{|sudo texhash|}

\medskip
\begin{figure}[htbp]
    \begin{center}
        \includegraphics[scale=.5]{term.pdf}
    \end{center}
\end{figure}

\item Check that \textcolor{red}{xkeyval, ifthen and tikz 2.0} are installed because they are obligatory.
\end{enumerate}

My folder texmf is structured as in the diagram below:

\medskip
\begin{tikzpicture} [remember picture,rotate=90] 

\node (texmf)   at (4,2)    [draw,fill=blue!30 ] {texmf};
\node (tex)     at (6,0)    [draw ]            {tex}; 
\node (doc)     at (0,0)    [draw ]            {doc};
\node (generic) at (7,-4)   [draw ]            {generic};
\node (docgen)  at (0,-4)   [draw ]            {generic};
\node (latex)   at (4,-4)   [draw ]            {latex}; 
\node (pgf)     at (7,-7)   [draw,fill=orange] {pgf};
\node (pre)     at (6,-7)   [draw,fill=orange] {pgf};
\node (xkey)    at (5,-7)   [draw ]            {xkeyval};
\node (four)    at (4,-7)   [draw ]            {fourier};
\node (prof)    at (3,-7)   [draw,fill=green ] {{prof}};
\node (etc)     at (2,-7)   [draw ]            {etc...}; 
\node (dpgf)    at (0,-7)   [draw,fill=orange] {pgf};
\node (cls)     at (8,-11)  [draw,fill=green ] {prof.cls};
\node (qcm)     at (7,-11)  [draw,fill=green ] {alterqcm.sty};
\node (fonc)    at (6,-11)  [draw,fill=orange] {tkz-base.sty};
\node (esp)     at (5,-11)  [draw,fill=orange] {tkz-fct.sty};
\node (tuk)     at (4,-11)  [draw,fill=orange] {tkz-arith.sty};
\node (tab)     at (3,-11)  [draw,fill=orange] {tkz-2d.sty};
\node (base)    at (2,-11)  [draw,fill=orange] {tkz-tab.sty};
\node (gra)     at (1,-11)  [draw,fill=orange] {tkz-berge.sty};
\node (pcfg)    at (0,-11)  [draw,fill=green ] {prof.cfg}; 
\node (ppcfg)   at (-1,-11) [draw,fill=green ] {profparam.cfg};
\node (bbp)     at (-2,-11) [draw,fill=orange] {bbpage.cfg};
\draw (doc.west)        |- (4, 1);
\draw (tex.west)        |- (4, 1);
\draw (latex.west)      |- (6,-2);
\draw (generic.west)    |- (6,-2);
\draw (xkey.west)       |- (5,-6);
\draw (prof.west)       |- (3,-6);
\draw (four.west)       |- (4,-6);
\draw (pre.west)        |- (4,-6); 
\draw (etc.west)        |- (4,-6);
\draw (cls.west)        |- (4,-9);
\draw (qcm.west)        |- (7,-9);
\draw (fonc.west)       |- (6,-9);
\draw (esp.west)        |- (5,-9);
\draw (tuk.west)        |- (4,-9);
\draw (tab.west)        |- (3,-9);
\draw (base.west)       |- (2,-9);
\draw (gra.west)        |- (1,-9);
\draw (pcfg.west)       |- (0,-9);
\draw (ppcfg.west)      |- (-1,-9);
\draw (bbp.west)        |- (4,-9);
\draw[-open triangle 90] (pgf.west)     --  (generic.east);
\draw[-open triangle 90] (4,1)          --  (texmf.east);
\draw[-open triangle 90] (6,-2)         --  (tex.east);
\draw[-open triangle 90] (4,-6)         --  (latex.east);
\draw[-open triangle 90] (3,-9)         --  (prof.east);
\draw[-open triangle 90] (dpgf.west)    --  (docgen.east);
\draw[-open triangle 90] (docgen.west)  --  (doc.east);
\end{tikzpicture}

\begin{tikzpicture}[remember picture,overlay]
        \path[->,thin,red,>=latex] (n1) edge [bend left] (prof);
        \path[->,thin,red,>=latex] (n2) edge [bend left] (prof);
\end{tikzpicture}
\endinput

==> tkz-graph/README <==
% encodage utf8    
--------------------  english readme ----------------------------------------
readme-tkz-graph.txt V 1.00 d 19/09/2018

The package tkz-graph.sty is a collection of some useful macros if you want to
 draw manually a graph of the graph theory. The kind of graphs that I will
  present, are sometimes called combinatorial graphs to distinguish them from
  the graphs of functions. The macros are designed to give math
 teachers (and students) easy access at the programmation of drawing graphs
  with  TikZ.  I therefore hope that my  packages provide  ideal tools for
   teachers wanting to offer their students fine documents of maths.

Licence
-------

This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License Distributed from CTAN
archives in directory macros/latex/base/lppl.txt. 


Features
-------- 

 -- needs etex;
 -- requires and automatically loads  PGF/TikZ 2.1; 
 -- compiles with utf8, pdflatex;
 -- compiles using the chain dvi->dvips->ps2pdf; 
 -- not yet ready for use with TeX and ConText (I need more time and ideas).    
 
Installation  
------------

You can experiment with the tkz-graph package by placing tkz-graph.sty in the directory containing your current tex file.

You can also placing tkz-graph.sty in the directory : 
/texmf/tex/latex/tkz.

 
How to use it
-------------

To use the package tkz-graph, place the following lines in the preamble of
 your LaTeX document.

\usepackage{tkz-graph} 

tkz-graph  loads  TikZ. 

If you use the xcolor package, load that package before tkz-graph to avoid
 package conflicts.

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{amsmath,tkz-graph}


Documentation
-------------  

The documentation is in french.
Documentation for tkz-graph is available on my sites:
 
 http://altermundus.fr (en français) or  http://altermundus.com (in english) 
 Documentation for printing will be ready soon. 
 
Examples
-------- 

 All  examples given in documentation will be stored on my sites as standalone
  files, ready for compilation.


 Alain Matthes
 5 rue de Valence
 Paris 75005  
 
 al (dot) ma (at) mac (dot) com 
 
               


==> tkz-graph/doc/latex/TKZdoc-gr-Dijkstra.tex <==
\section{Dijkstra}

{\large Algorithme de Dijkstra :} Plus courte chaîne du sommet $E$ au sommet $S$.

\medskip 

\subsection{Dijkstra exemple 1}

\medskip 
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
   \GraphInit[vstyle=Dijkstra]
   \SetGraphUnit{4}
   \Vertices{square}{B,C,D,A}
      \SetGraphUnit{2.82}
   \NOWE(B){E}
   \NOEA(C){S}
   \Edge[label=$3$](E)(A)
   \Edge[label=$1$](E)(B)
   \Edge[label=$1$](A)(B)
   \Edge[label=$3$](B)(C)
   \Edge[label=$3$,style={pos=.25}](A)(C)
   \Edge[label=$5$,style={pos=.75}](B)(D)
   \Edge[label=$4$](A)(D)
   \Edge[label=$1$](S)(D)
   \Edge[label=$3$](C)(S)
   \Edge[label=$1$](C)(D)
\end{tikzpicture}
\end{tkzexample}
\end{center}



\def\ry{$\vrule width 5pt$}
\def\iy{$\infty$}

%<–––––––––––––––––——————————————————————————————————————————————————————————>
\vbox{\tabskip=0pt \offinterlineskip
\def\tablerule{\noalign{\hskip\tabskip\hrule}}
\halign to \hsize{\strut#&\vrule # \tabskip=0.6em plus8em&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#\tabskip=0pt\cr\tablerule
&& $E$ &&  $A$   &&  $B$   &&   $C$  &&  $D$   && $S$    && Choix    &\cr\tablerule
&& $0$ && \iy    && \iy    && \iy    && \iy    && \iy    && $E$       &\cr\tablerule
&& \ry && $3(E)$ && $1(E)$ && \iy    && \iy    && \iy    && $B$     &\cr\tablerule
&& \ry && $2(B)$ && \ry    && $4(B)$ && $6(B)$ && \iy    && $A$     &\cr\tablerule
&& \ry && \ry    && \ry    && $4(B)$ && $6(B)$ && \iy    && $C$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && $5(C)$ && $7(C)$ && $D$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && $6(D)$ && $S$    &\cr\tablerule}}
%<–––––––––––––––––——————————————————————————————————————————————————————————>

\medskip

Le plus court chemin est donc $EBCDS$

\vfill\newpage 
\subsection{Dijkstra exemple 2} 

\medskip
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
    \GraphInit[vstyle=Dijkstra]
   \SetGraphUnit{4}
    \Vertices{square}{G,D,A,F}
    \WE(F){H}
    \EA(A){B}
    \EA(D){C}
    \NO(A){E}
    \Edge[label=$1$](H)(F)
    \Edge[label=$4$](G)(F)
    \Edge[label=$2$](H)(G)
    \Edge[label=$2$](G)(D)
    \Edge[label=$3$](D)(C)
    \Edge[label=$4$](F)(E)
    \Edge[label=$3$](A)(D)
    \Edge[label=$2$](A)(E)
    \Edge[label=$1$](A)(B)
    \Edge[label=$2$](A)(C)
    \Edge[label=$2$](C)(B)
    \Edge[label=$3$](E)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}
%<–––––––––––––––––——————————————————————————————————————————————————————————>
\vbox{\tabskip=0pt \offinterlineskip
\def\tablerule{\noalign{\hskip\tabskip\hrule}}
\halign to \hsize{\strut#&\vrule # \tabskip=0.6em plus8em&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#\tabskip=0pt\cr\tablerule
&& $H$ &&  $F$   &&  $G$   &&   $E$  &&  $D$   && $A$    && $C$    && $B$    && Choix   &\cr\tablerule
&& $0$ && \iy    && \iy    && \iy    && \iy    && \iy    && \iy    && \iy    && $H$     &\cr\tablerule
&& \ry && $1(H)$ && $2(H)$ && \iy    && \iy    && \iy    && \iy    && \iy    && $F$     &\cr\tablerule
&& \ry && \ry    && $2(H)$ && $5(F)$ && \iy    && \iy    && \iy    && \iy    && $G$     &\cr\tablerule
&& \ry && \ry    && \ry    && $5(F)$ && $4(G)$ && \iy    && \iy    && \iy    && $D$     &\cr\tablerule
&& \ry && \ry    && \ry    && $5(F)$ && \ry    && $7(D)$ && $7(D)$ && \iy    && $E$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && $7(D)$ && $7(D)$ && $8(E)$ && $A$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && \ry    && $7(D)$ && $8(E)$ && $C$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && \ry    && \ry    && $8(E)$ && $B$     &\cr\tablerule}}
%<–––––––––––––––––——————————————————————————————————————————————————————————>

Le plus court chemin est donc $HFEB$  

\begin{tkzexample}[code only]
\def\ry{$\vrule width 5pt$}
\def\iy{$\infty$} 
\vbox{\tabskip=0pt \offinterlineskip
\def\tablerule{\noalign{\hskip\tabskip\hrule}}
\halign to \hsize{\strut#&\vrule # \tabskip=0.6em plus8em&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#&
\hfil#\hfil& \vrule#\tabskip=0pt\cr\tablerule
&& $H$ &&  $F$   &&  $G$   &&   $E$  &&  $D$   && $A$    && $C$    && $B$%
&& Choix   &\cr\tablerule
&& $0$ && \iy    && \iy    && \iy    && \iy    && \iy    && \iy    && \iy%
&& $H$     &\cr\tablerule
&& \ry && $1(H)$ && $2(H)$ && \iy    && \iy    && \iy    && \iy    && \iy%
&& $F$     &\cr\tablerule
&& \ry && \ry    && $2(H)$ && $5(F)$ && \iy    && \iy    && \iy    && \iy%
&& $G$     &\cr\tablerule
&& \ry && \ry    && \ry    && $5(F)$ && $4(G)$ && \iy    && \iy    && \iy%
&& $D$     &\cr\tablerule
&& \ry && \ry    && \ry    && $5(F)$ && \ry    && $7(D)$ && $7(D)$ && \iy%
&& $E$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && $7(D)$ && $7(D)$ && $8(E)$%
&& $A$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && \ry    && $7(D)$ && $8(E)$%
&& $C$     &\cr\tablerule
&& \ry && \ry    && \ry    && \ry    && \ry    && \ry    && \ry    && $8(E)$%
&& $B$     &\cr\tablerule}} 
\end{tkzexample}
  

\endinput

==> tkz-graph/doc/latex/TKZdoc-gr-Welsh.tex <==
% $Id$
%!TEX root = /Users/ego/Boulot/TKZ/Graph/doc-fr/TKZdoc-gr-main.tex
\section{Colorisation Welsh} 
%<–––––––––––––––––––––––––– graphs with colors ––––––––––––––––––––––––––—––>
Ce chapitre montre comment colorer des sommets. Le plus simple est d'utiliser le style \tkzname{Welsh} et la macro \tkzcname{AddVertexColor} afin de colorer les sommets.

\subsection{La macro \tkzcname{AddVertexColor} } 

\begin{NewMacroBox}{AddVertexColor}{\var{color}\var{List of vertices}}

\medskip
\emph{Cette macro permet de colorer des sommets. Le premier argument est la couleur, le second une liste  de sommets.}
\end{NewMacroBox} 


\subsection{Exemple d'utilisation } 

\medskip
Une compagnie aérienne propose des vols directs entre certaines villes, notées A, B, C, D, E, F et G. Cela conduit au graphe $\mathcal{G}$ suivant, dont les sommets sont les villes et les arêtes représentent les liaisons aériennes :
 
 \begin{center}
\begin{tikzpicture}
\renewcommand*{\VertexLineWidth}{2pt}  
 \GraphInit[vstyle=Welsh]
 \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}  
 \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture} 
\end{center}

\begin{enumerate}

\item Sur les cartes d'embarquement, la compagnie attribue à chaque aéroport une couleur, de sorte que deux aéroports liés par un vol direct aient des couleurs différentes.

 Proposer un coloriage adapté‚ cette condition.
\item Que peut-on en déduire sur le nombre chromatique de $\mathcal{G}$ ?
\end{enumerate}



\begin{center}
\begin{tkzltxexample}[]
\begin{tikzpicture}
\renewcommand*{\VertexLineWidth}{2pt}  
 \GraphInit[vstyle=Welsh]
 \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}  
 \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture} 
\end{tkzltxexample}
\end{center}

\bigskip
\begin{minipage}{7cm}
 \begin{tikzpicture}
\renewcommand*{\VertexLineWidth}{2pt}  
 \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}  
 \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
 \end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{7cm}
 \begin{tabular}{cc}
 \hline
 \itshape Sommet & \itshape Degré \\
 \hline
 B & $5$ \\
 E & $5$ \\
 C & $4$ \\
 D & $4$ \\
 A & $3$ \\
 G & $3$ \\
 F & $2$ \\
 \hline
 \end{tabular}
\end{minipage}

\begin{tkzltxexample}[]
 \begin{tikzpicture}
\renewcommand*{\VertexLineWidth}{2pt}   
 \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
 \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{tkzltxexample}

\bigskip
\begin{minipage}{7cm}
 \begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{tabular}{ccc}
\hline
\itshape Sommet & \itshape Degré & \itshape Couleur\\
\hline
B & $5$ & rouge\\
E & $5$ & \\
C & $4$ & \\
D & $4$ & \\
A & $3$ & \\
G & $3$ & \\
F & $2$ & rouge\\
\hline
\end{tabular}
\end{minipage}

\begin{tkzltxexample}[]
\begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{tkzltxexample}

\bigskip
\begin{minipage}{7cm}
 \begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F} \AddVertexColor{blue}{E,A}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{tabular}{ccc}
\hline
\itshape Sommet & \itshape Degré & \itshape Couleur\\
\hline
B & $5$ & rouge\\
E & $5$ & bleu\\
C & $4$ & \\
D & $4$ & \\
A & $3$ & bleu\\
G & $3$ & \\
F & $2$ & rouge\\
\hline
\end{tabular}
\end{minipage}

\begin{tkzltxexample}[]
\begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F}
  \AddVertexColor{blue}{E,A}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A)
  \Edges(B,E)
\end{tikzpicture}
\end{tkzltxexample}

\bigskip
\begin{minipage}{7cm}
\begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F} \AddVertexColor{blue}{E,A}
  \AddVertexColor{green}{C,G}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{tabular}{ccc}
\hline
\itshape Sommet & \itshape Degré & \itshape Couleur\\
\hline
B & $5$ & rouge\\
E & $5$ & bleu\\
C & $4$ & vert\\
D & $4$ & \\
A & $3$ & bleu\\
G & $3$ & vert\\
F & $2$ & rouge\\
\hline
\end{tabular}
\end{minipage}

\begin{tkzltxexample}[]
\begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F} \AddVertexColor{blue}{E,A}
  \AddVertexColor{green}{C,G}
  \Vertex[Node]{D}}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{tkzltxexample}

\bigskip
\begin{minipage}{7cm}
\begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F}   \AddVertexColor{blue}{E,A}
  \AddVertexColor{green}{C,G} \AddVertexColor{yellow}{D}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A) \Edges(B,E)
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{tabular}{ccc}
\hline
\itshape Sommet & \itshape Degré & \itshape Couleur\\
\hline
B & $5$ & rouge\\
E & $5$ & bleu\\
C & $4$ & vert\\
D & $4$ & jaune\\
A & $3$ & bleu\\
G & $3$ & vert\\
F & $2$ & rouge\\
\hline
\end{tabular}
\end{minipage}

\begin{tkzltxexample}[]
 \begin{tikzpicture}
  \renewcommand*{\VertexLineWidth}{2pt}  
  \GraphInit[vstyle=Welsh]
  \Vertices[unit=3]{circle}{A,B,C,D,E,F,G}   
  \SetVertexNoLabel
  \AddVertexColor{red}{B,F}  \AddVertexColor{blue}{E,A}
  \AddVertexColor{green}{C,G}\AddVertexColor{yellow}{D}
  \Vertex[Node]{D}}
  \Edges(G,E,F,G,B,D,E,C,D,A,C,B,A)\Edges(B,E)
\end{tikzpicture}
\end{tkzltxexample}
\endinput


==> tkz-graph/doc/latex/TKZdoc-gr-annales.tex <==
\section{Annales.}  %<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         Amérique du nord juin 2003
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Amérique du nord juin 2003}

Soit le graphe G joint en annexe constitué des sommets A, B, C, D, E, F et G.

\begin{enumerate} 
\item Quel est son ordre et le degré de chacun de ses sommets ?
\item Reproduire sur la copie et compléter le tableau des distances entre deux sommets de G :

\medskip
\begin{center} 
\begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
Distance    &    A  &   B   &   C   &   D   &   E   &   F   &   G   \\ \hline
A           &    X  &       &       &       &       &       &       \\ \hline
B           &    X  &   X   &       &       &       &       &       \\ \hline
C           &    X  &   X   &   X   &       &       &       &       \\ \hline
D           &    X  &   X   &   X   &   X   &       &       &       \\ \hline
E           &    X  &   X   &   X   &   X   &   X   &       &       \\ \hline
F           &    X  &   X   &   X   &   X   &   X   &   X   &       \\ \hline
G           &    X  &   X   &   X   &   X   &   X   &   X   &   X   \\ \hline
\end{tabular}
\end{center}

\medskip
En déduire le diamètre de ce graphe.
\item 
   \begin{enumerate} 
   \item Donner un sous-graphe complet d'ordre 3 de G.

Qu'en déduire pour le nombre chromatique de G ?
   \item Proposer une coloration du graphe G et en déduire son nombre chromatique.
   \end{enumerate}
\item Donner la matrice M associée à G (vous numéroterez les lignes et les  colonnes dans l'ordre alphabétique).
\item En utilisant la matrice $ M_2$ donnée en annexe 1, déduire le nombre de chaînes de longueur 2 partant de A sans y revenir.
\end{enumerate}

\medskip
\begin{minipage}[]{10cm}
\begin{tikzpicture}
    \Vertex[x=1.3,y=3.8]{A}
    \Vertex[x=4.2,y=5.5]{B}
    \Vertex[x=7.3,y=4]{C}
    \Vertex[x=8.5,y=1.5]{D}
    \Vertex[x=5,y=0]{E}
    \Vertex[x=3.6,y=4]{F}  
    \Vertex[x=0.7,y=1]{G}
    \Edges(A,B,C,D,E,G,A,F,E,C)
    \Edge(B)(F)
\end{tikzpicture}
\end{minipage}
\begin{minipage}[]{5cm}
M$^2 =
\begin{pmatrix}
    3   &   1   &   1   &   0   &   2   &   1   &   0\\
    1   &   3   &   0   &   1   &   2   &   1   &   1\\
    1   &   0   &   3   &   1   &   1   &   2   &   1\\
    0   &   1   &   1   &   2   &   1   &   1   &   1\\
    2   &   2   &   1   &   1   &   4   &   0   &   0\\
    1   &   1   &   2   &   1   &   0   &   3   &   2\\
    0   &   1   &   1   &   1   &   0   &   2   &   2\\
\end{pmatrix}$
\end{minipage}

\medskip
\begin{tkzexample}[code only]
\begin{tikzpicture}
    \Vertex[x=1.3,y=3.8]{A}     \Vertex[x=4.2,y=5.5]{B}
    \Vertex[x=7.3,y=4]{C}       \Vertex[x=8.5,y=1.5]{D}
    \Vertex[x=5,y=0]{E}         \Vertex[x=3.6,y=4]{F}
    \Vertex[x=0.7,y=1]{G}
    \Edges(A,B,C,D,E,G,A,F,E,C) \Edge(B)(F)
\end{tikzpicture}
\end{tkzexample}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         Antilles-Guyane juin 2003
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Antilles-Guyane juin 2003 }\label{ag03} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\begin{enumerate}
\item Un musée est constitué de 9 salles notées A, B, C, D, E, F, G, H et S.

Le plan du musée est représenté ci-dessous :

\medskip
\begin{center}
\begin{tikzpicture}
\draw (0,0) rectangle (8,6);
\draw(2,0)--(2,0.7);
\draw(2,1.3)--(2,2.7);
\draw(2,3.3)--(2,4.7);
\draw(2,5.3)--(2,6);
\draw(4,0)--(4,0.7);
\draw(4,1.3)--(4,2.7);
\draw(4,3.3)--(4,4.7);
\draw(4,5.3)--(4,6);
\draw(6,0)--(6,0.7);
\draw(6,1.3)--(6,2.7);
\draw(6,3.3)--(6,4.7);
\draw(6,5.3)--(6,6);
\draw(2,5.3)--(2,6);
\draw(4,5.3)--(4,6);
\draw(6,5.3)--(6,6);
\draw(2,2)--(2.7,2);
\draw(3.3,2)--(4.7,2);
\draw(5.3,2)--(6,2);
\draw(2,4)--(2.7,4);
\draw(3.3,4)--(4.7,4);
\draw(5.3,4)--(8,4);
\node at (1,3){S};
\node at (3,3){G};
\node at (3,1){D};
\node at (3,5){A};
\node at (5,1){H};
\node at (5,3){E};
\node at (5,5){B};
\node at (7,2){F};
\node at (7,5){C};
\end{tikzpicture}
\end{center}

\medskip
Ainsi, un visiteur qui se trouve dans la salle S peut atteindre directement les salles  A, B ou G. S'il se trouve dans la salle C, il peut se rendre directement dans la salle B, mais pas dans la salle F.

On s'intéresse au parcours d'un visiteur dans ce musée. On ne se préoccupe pas de la manière dont le visiteur accède au musée ni comment il en sort. Cette situation peut être modélisée par un graphe, les sommets étant les noms des salles, les arêtes représentant les portes de communication.

   \begin{enumerate} 
   \item Dessiner un graphe modélisant la situation décrite.
   \item Est-il possible de visiter le musée, en empruntant chaque porte une fois et une seule ?

Justifier en utilisant un théorème du cours sur les graphes.
\item Pour rompre une éventuelle monotonie, le conservateur du musée souhaite différencier chaque salle de sa ou des salles voisines (c'est-à-dire accessibles par une porte)  par la moquette posée au sol. Quel est le nombre minimum de types de moquettes nécessaires pour  répondre à ce souhait ? Justifier.
   \end{enumerate}
\item On note $M$ la matrice à 9 lignes et 9 colonnes associée au graphe précédent, en  convenant de l'ordre suivant des salles S, A, B, C, D, E, F, G, H. Le graphe n'étant pas orienté,  comment cela se traduit-il sur la matrice ?
\item  On donne la matrice :

\[M^4 = 
\begin{pmatrix}
18  &   12  &   11  &   02  &   20  &   12  & 06    & 12    & 12\\
12  &   20  &   03  &   06  &   11  &   20  & 05    & 18    & 05\\
11  &   03  &   16  &   00  &   19  &   03  & 08    & 04    & 12\\
02  &   06  &   00  &   03  &   01  &   07  & 01    & 04    & 01\\
20  &   11  &   19  &   01  &   31  &   09  & 11    & 12    & 19\\
12  &   20  &   03  &   07  &   09  &   28  & 09    & 20    & 09\\
06  &   05  &   08  &   01  &   11  &   09  & 09    & 08    & 09\\
12  &   18  &   04  &   04  &   12  &   20  & 08    & 20    & 06\\
12  &   05  &   12  &   01  &   19  &   09  & 09    & 06    & 17\\
\end{pmatrix}\]

   \begin{enumerate} 
   \item Combien y-a-t-il de chemins qui en 4 étapes, partent de D et reviennent à D ?
   \item Combien y-a-t-il de chemins qui en 4 étapes, partent de S et reviennent à C ? Les citer.
   \item Est-il toujours possible de joindre en 4 étapes deux salles quelconques ? Justifier.
   \end{enumerate}
\end{enumerate}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent, uniquement fait avec tikz sans tkz-berge

\bigskip
\begin{tkzexample}[code only]
\begin{tikzpicture}
  \draw (0,0) rectangle (8,6);
  \draw(2,0)--(2,0.7);
  \draw(2,1.3)--(2,2.7);
  \draw(2,3.3)--(2,4.7);
  \draw(2,5.3)--(2,6);
  \draw(4,0)--(4,0.7);
  \draw(4,1.3)--(4,2.7);
  \draw(4,3.3)--(4,4.7);
  \draw(4,5.3)--(4,6);
  \draw(6,0)--(6,0.7);
  \draw(6,1.3)--(6,2.7);
  \draw(6,3.3)--(6,4.7);
  \draw(6,5.3)--(6,6);
  \draw(2,5.3)--(2,6);
  \draw(4,5.3)--(4,6);
  \draw(6,5.3)--(6,6);
  \draw(2,2)--(2.7,2);
  \draw(3.3,2)--(4.7,2);
  \draw(5.3,2)--(6,2);
  \draw(2,4)--(2.7,4);
  \draw(3.3,4)--(4.7,4);
  \draw(5.3,4)--(8,4);
  \node at (1,3){S};
  \node at (3,3){G};
  \node at (3,1){D};
  \node at (3,5){H};
  \node at (5,1){H};
  \node at (5,3){E};
  \node at (5,5){B};
  \node at (7,2){F};
  \node at (7,5){C};
\end{tikzpicture}
\end{tkzexample}


%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         Asie juin 2003
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Asie juin 2003 }\label{asj03} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>


\bigskip 
\begin{minipage}[l]{0,58\textwidth}
Dans la ville de GRAPHE, on s'intéresse aux principales rues permettant de relier différents lieux ouverts au public, à savoir la mairie (M), le centre commercial (C), la bibliothèque (B), la piscine (P) et le lycée (L). Chacun de ces lieux est désigné par son initiale. Le tableau ci-contre donne les rues existant entre ces lieux.
\end{minipage}\hfill
\begin{minipage}[]{0,38\textwidth}
\begin{center}
     \begin{tabular}{|*{5}{c|} c|} \cline{2-6}
        \multicolumn{1}{c|}{}
          & B   & C & L & M & P \\ \hline
        B &     & X &   & X & X \\ \hline
        C & X   &   & X & X &   \\ \hline
        L &     & X &   & X &   \\ \hline
        M & X   & X & X &   & X \\ \hline
        P & X   &   &   & X &   \\ \hline
    \end{tabular}
\end{center}
\end{minipage}

\medskip
\begin{enumerate} 
\item Dessiner un graphe représentant cette situation.
\item Montrer qu'il est possible de trouver un trajet empruntant une fois et une seule toutes les rues de ce plan. Justifier. Proposer un tel trajet.

Est-il possible d'avoir un trajet partant et arrivant du même lieu et passant une fois et une seule par toutes les rues ?


\begin{minipage}[b]{0,3\textwidth}
\item
 Dimitri habite dans cette ville ; le graphe ci-contre  donne le \textbf{nouveau} plan du quartier avec les sens de circulation dans les différentes rues et le temps de parcours entre les différents lieux.
\end{minipage}
\hspace{1cm}
 \begin{minipage}[c]{0,68\textwidth}
    \begin{tikzpicture}[>=latex]
      \SetGraphUnit{4}
      \tikzset{VertexStyle/.style  = {shape         = circle,
                                      draw          = black,
                                      inner sep     = 2pt,%
                                      minimum size  = 6mm,
                                      outer sep     = 0pt,
                                      fill          = gray!60}}
      \Vertex {P}
      \NOEA(P){B}
      \SOEA(P){M}
      \NOEA(B){D}
      \SOEA(B){C}
      \SOEA(C){L}
      \tikzset{LabelStyle/.style = {fill=white}}
      \tikzset{EdgeStyle/.style  = {<->}}
      \Edge[label=$4$](P)(M)
      \Edge[label=$9$](C)(M)
      \Edge[label=$4$](C)(L)
      \Edge[label=$5$](C)(D)
      \Edge[label=$10$](B)(M)
      \tikzset{EdgeStyle/.style  = {<->,bend right}}
      \Edge[label=$11$](L)(D)
      \tikzset{EdgeStyle/.style  = {->}}
      \Edge[label=$3$](C)(B)
      \Edge[label=$10$](D)(B)
      \Edge[label=$10$](L)(M)
      \Edge[label=$10$](B)(P)
    \end{tikzpicture}
  \end{minipage}
\end{enumerate}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent

\bigskip
\begin{tkzexample}[code only]
\begin{minipage}[c]{0,68\textwidth}
\begin{tikzpicture}[>=latex]
    \SetGraphUnit{4}
    \tikzset{VertexStyle/.style  = {shape         = circle,
                                    draw          = black,
                                    inner sep     = 2pt,%
                                    minimum size  = 6mm,
                                    outer sep     = 0pt,
                                    fill          = gray!60}}
    \Vertex {P}
    \NOEA(P){B}
    \SOEA(P){M}
    \NOEA(B){D}
    \SOEA(B){C}
    \SOEA(C){L}
    \tikzset{LabelStyle/.style = {fill=white}}
    \tikzset{EdgeStyle/.style  = {<->}}
    \Edge[label=$4$](P)(M)
    \Edge[label=$9$](C)(M)
    \Edge[label=$4$](C)(L)
    \Edge[label=$5$](C)(D)
    \Edge[label=$10$](B)(M)
    \tikzset{EdgeStyle/.style  = {<->,bend right}}
    \Edge[label=$11$](L)(D)
    \tikzset{EdgeStyle/.style  = {->}}
    \Edge[label=$3$](C)(B)
    \Edge[label=$10$](D)(B)
    \Edge[label=$10$](L)(M)
    \Edge[label=$10$](B)(P)
\end{tikzpicture}
\end{minipage}
\end{tkzexample}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         France juin 2003
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{France juin 2003 }\label{frj03} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

Un concert de solidarité est organisé dans une grande salle de spectacle. À ce concert sont conviés sept artistes de renommée internationale Luther Allunison (A), John Biaise (B), Phil Colline (C), Bob Ditlâne (D), Jimi Endisque (E), Robert Fripe (F) et Rory Garaguerre (G).

Les différents musiciens invités refusant de jouer avec certains autres, l'organisateur du concert doit prévoir plusieurs parties de spectacle. Les arêtes du  graphe $\Gamma$ ci-dessous indiquent quels sont les musiciens qui refusent de jouer entre eux.

\medskip
\begin{center}
\begin{tikzpicture}
  \SetGraphUnit{4}
  \GraphInit[vstyle=Normal]
  \tikzset{EdgeStyle/.style = {line width = 2pt}}
  \tikzset{VertexStyle/.append style = {line width = 2pt}}
  \Vertex{D}
  \SOEA(D){E}
  \EA(E){F}
  \NOEA(F){G}
  \NOWE(G){A}
  \NOWE(A){B}
  \SOWE(B){C}
  \Edges(F,G,A,D,F,B,E,G,C,F,A,E,C,B)
\end{tikzpicture}
\end{center}

\medskip
\begin{enumerate} 
\item Déterminer la matrice associée au graphe $\Gamma$ (les sommets de $\Gamma$ étant classés dans l'ordre alphabétique).
\item Quelle est la nature du sous-graphe de $\Gamma '$ constitué des sommets A, E, F et G ?

Que peut-on en déduire pour le nombre chromatique $\chi(\Gamma)$ du graphe $\Gamma$ ?
\item Quel est le sommet de plus haut degré de $\Gamma$ ?

En déduire un encadrement de $\chi(\Gamma)$.
\item Après avoir classé l'ensemble des sommets de $\Gamma$ par ordre de degré décroissant, colorier le graphe $\Gamma$ figurant en annexe.
\item Combien de parties l'organisateur du concert doit-il  prévoir ?

Proposer une répartition des musiciens pour chacune de ces parties.
\end{enumerate}

\medskip

\begin{tkzexample}[code only]
\begin{tikzpicture}
  \SetGraphUnit{4}
  \GraphInit[vstyle=Normal]
  \tikzset{EdgeStyle/.style = {line width = 2pt}}
  \tikzset{VertexStyle/.append style = {line width = 2pt}}
  \Vertex{D}
  \SOEA(D){E}\EA(E){F}
  \NOEA(F){G}\NOWE(G){A}
  \NOWE(A){B}\SOWE(B){C}
  \Edges(F,G,A,D,F,B,E,G,C,F,A,E,C,B)
\end{tikzpicture}
\end{tkzexample}


%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                        CE juin 2003
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Centres Étrangers juin 2003 }\label{cej03} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\bigskip
Un livreur d'une société de vente à domicile doit, dans son après-midi, charger son camion à l'entrepôt noté A, livrer cinq clients que nous noterons B, C, D, E et F, puis retourner à l'entrepôt. Le réseau routier, tenant compte des sens de circulation, et les temps de parcours (en minutes) sont indiqués sur le graphe G suivant :

\medskip
\begin{center}
  \begin{tikzpicture}[>=latex]
    \SetGraphUnit{4}
    \Vertex {F}
    \NOWE(F){A}
    \NOEA(F){B}
    \SOEA(F){C}
    \SOWE(F){D}
    \SOWE(A){E}
    \tikzstyle{EdgeStyle}=[->]
    \tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=$4$](A)(E)
    \Edge[label=$4$](E)(D)
    \Edge[label=$9$](D)(A)
    \Edge[label=$2$](B)(A)
    \Edge[label=$11$](C)(B)
    \Edge[label=$3$](D)(F)
    \Edge[label=$6$](F)(A)
    \tikzstyle{EdgeStyle}=[->,bend left=15]
    \Edge[label=$2$](D)(C)
    \Edge[label=$2$](C)(D)
    \Edge[label=$3$](F)(B)
    \Edge[label=$3$](B)(F)
    \Edge[label=$6$](F)(C)
    \Edge[label=$6$](C)(F)
  \end{tikzpicture}
\end{center}

\begin{enumerate} 
\item Donner la matrice M associée au graphe G.

On utilisera le modèle suivant :

\begin{center}
    \begin{tabular}{|*{7}{c|}}\cline{2-7}
    \multicolumn{1}{c|}{}%
        & A & B & C & D & E & F \\ \hline
    A   &   &   &   &   &   &   \\ \hline
    B   &   &   &   &   &   &   \\ \hline
    C   &   &   &   &   &   &   \\ \hline
    D   &   &   &   &   &   &   \\ \hline
    E   &   &   &   &   &   &   \\ \hline
    F   &   &   &   &   &   &   \\ \hline
    \end{tabular}
\end{center}

\item  On donne la matrice M$^6$ :

\[\text{M}^6 = 
\begin{pmatrix}
    8   &   6   &   6   &   3   &   4   &   6 \\
    19  &   11  &   12  &   9   &   6   &   16\\
    36  &   28  &   23  &   22  &   18  &   34\\
    37  &   24  &   25  &   17  &   15  &   31\\
    15  &   12  &   9   &   10  &   8   &   15\\
    28  &   22  &   19  &   15  &   15  &   26\\
\end{pmatrix}\]

On s'intéresse aux chemins partant de l'entrepôt A et se terminant en A.

   \begin{enumerate} 
   \item Combien existe-t-il de chemins de longueur 6 reliant A à A ?
   \item Citer ces chemins.
   \item Parmi ceux qui passent par tous les sommets du graphe, lequel minimise le temps de parcours ?
   \item Quelle conséquence peut tirer le livreur du dernier résultat ?
   \end{enumerate}
\item Au départ de sa tournée, le livreur a choisi de suivre l'itinéraire le plus rapide. Malheureusement, le client C n'est pas présent au passage du livreur et celui-ci décide de terminer sa livraison par ce client. Indiquer  quel est le chemin le plus rapide pour revenir à l'entrepôt A à partir de C. La réponse devra être justifiée.
\end{enumerate}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent

\bigskip
\begin{tkzexample}[code only]
\begin{tikzpicture}[>=latex]
  \SetGraphUnit{3}
  \Vertex {F}
  \NOWE(F){A}
  \NOEA(F){B}
  \SOEA(F){C}
  \SOWE(F){D}
  \SOWE(A){E}
  \tikzstyle{EdgeStyle}=[->]
  \tikzstyle{LabelStyle}=[fill=white]
  \Edge[label=$4$](A)(E)
  \Edge[label=$4$](E)(D)
  \Edge[label=$9$](D)(A)
  \Edge[label=$2$](B)(A)
  \Edge[label=$11$](C)(B)
  \Edge[label=$3$](D)(F)
  \Edge[label=$6$](F)(A)
  \tikzstyle{EdgeStyle}=[->,bend left=15]
  \Edge[label=$2$](D)(C)
  \Edge[label=$2$](C)(D)
  \Edge[label=$3$](F)(B)
  \Edge[label=$3$](B)(F)
  \Edge[label=$6$](F)(C)
  \Edge[label=$6$](C)(F)
\end{tikzpicture}
\end{tkzexample}
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         Amérique du Nord mai 2004
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Amérique du Nord juin 2004 }\label{anm04} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>


\textbf{Les parties A et B sont indépendantes.}

\textbf{Partie A}

On considère le graphe G$_{1}$ ci-dessous :

\bigskip

\begin{center}
\begin{tikzpicture}[>=latex]
    \SetGraphUnit{6}
    \Vertex{F}%
    \NOEA(F){B}
    \SOEA(F){E}
    \EA(B){C}
    \EA(E){D}
    \NO(D){A}
    \Edges(B,F,E,D,A,E,B,A,F,B,C,F,D)
\end{tikzpicture}
\end{center}

\medskip

\begin{enumerate}
\item Justifier les affirmations suivantes :

A$_{1}$ : \og le graphe G$_1$ admet au moins une chaîne eulérienne \fg.

A$_{2}$ ; \og La chaîne DABCFBEFAE n'est pas une chaîne eulérienne de G$_1$ \fg.

\item Déterminer un sous-graphe complet de G$_1$, ayant le plus grand ordre possible. En déduire un minorant du nombre chromatique $\gamma$ de ce graphe.

\item Déterminer un majorant de ce nombre chromatique. (On justifiera la réponse).

\item En proposant une coloration du graphe G$_1$, déterminer son nombre chromatique.

\end{enumerate}

\medskip

\textbf{Partie B}

Soit la matrice M d'un graphe orienté G$_2$ dont les sommets A, B, C, D et E sont pris dans l'ordre alphabétique.

On donne \[
    M = 
\begin{pmatrix}
    0   &   1   &   1   &   1   &   0\\
    1   &   0   &   1   &   0   &   1\\
    1   &   1   &   0   &   0   &   1\\
    0   &   1   &   0   &   0   &   1\\
    1   &   1   &   0   &   1   &   0\\
\end{pmatrix}
\]
~et~
\[
    \text{M}^3 = 
\begin{pmatrix}
    6   &   6   &   4   &   5   &   3\\
    5   &   6   &   5   &   3   &   6\\
    5   &   7   &   4   &   3   &   6\\
    3   &   5   &   3   &   3   &   3\\
    6   &   6   &   3   &   3   &   5\\
\end{pmatrix}.
\]
\begin{enumerate}
\item Construire le graphe G$_2$.
\item Déterminer le nombre de chaînes de longueur 3 reliant B à D. Les citer toutes.
\end{enumerate}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent

\bigskip
\begin{tkzexample}[code only]
\begin{tikzpicture}[>=latex]
  \SetGraphUnit{6}
  \Vertex{F}
  \NOEA(F){B}
  \SOEA(F){E}
  \EA(B){C}
  \EA(E){D}
  \NO(D){A}
  \Edges(B,F,E,D,A,E,B,A,F,B,C,F,D)
\end{tikzpicture}
\end{tkzexample}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         CE mai 2004
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Centres étrangers  mai 2004 }\label{cem04} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\bigskip
Un jardinier possède un terrain bien ensoleillé avec une partie plus ombragée.

Il décide d'y organiser des parcelles où il plantera 8 variétés de légumes :

\medskip
\begin{center}\begin{minipage}[t]{0.48\textwidth}
    \begin{itemize}
    \item de l'ail (A),
    \item des courges (Co),
    \item des choux (Ch),
    \item des poireaux (Px),
    \item des pois (Po),
    \item des pommes de terre (Pt),
    \item des radis (R),
    \item et des tomates (T).
    \end{itemize}
\end{minipage}\end{center}

\medskip
Il consulte un almanach où figurent des incompatibilités de plantes, données par les deux tableaux :

\medskip

\begin{minipage}[t]{0.46\textwidth}
\begin{tabular}{|l|l|}\hline
    \multicolumn{2}{|p{7cm}|}{Expositions incompatibles de plantes}\\
\hline
    \multicolumn{1}{|p{3.5cm}|}{Plantes d'ombre partielle}
    &\multicolumn{1}{|p{3.5cm}|}{Plantes de plein soleil}\\ 
\hline
    &                       \\
    &   choux               \\
        pois    &   tomates \\
        radis   &   courges \\
    &                       \\
    &                       \\ 
\hline
    \multicolumn{2}{|p{7cm}|}{Par exemple : les pois sont incompatibles avec les
    choux, les tomates et les courges}\\ \hline
\end{tabular}
\end{minipage}
\hfill
\raisebox{6pt}{\begin{minipage}[t]{0.46\textwidth}
\begin{tabular}{|l|l|}\hline
\multicolumn{2}{|p{7cm}|}{Associations incompatibles de} \\
\multicolumn{2}{|p{7cm}|}{plantes dans une même parcelle}\\ \hline
 pois & ail, poireaux\\ \hline
pommes de & courges, radis et\\
terre & tomates\\ \hline
& tomates, ail\\
choux & poireaux et courges\\ \hline
courges & tomates\\ \hline
\multicolumn{2}{|p{7cm}|}{Par exemple : les pois sont incompatibles avec
l'ail et les poireaux}\\ \hline
\end{tabular}
\end{minipage}}

\medskip

Pour tenir compte de ces incompatibilités le jardinier décide de modéliser la situation sous la forme d'un graphe de huit sommets, chaque sommet représentant un légume.
\medskip
\begin{enumerate}
\item Sur la feuille annexe : compléter le graphe mettant en évidence les incompatibilités d'exposition ou les associations incompatibles indiquées dans les deux tableaux ci-dessus.

\item Calculer la somme des degrés des sommets du graphe, en déduire le nombre de ses arêtes.

\item Rechercher un sous-graphe complet d'ordre 4, qu'en déduit-on pour le nombre chromatique du graphe ?

\item Donner le nombre chromatique du graphe et l'interpréter en nombre minimum de parcelles que le jardinier devra créer.

\item Donner une répartition des plantes pur parcelle de façon à ce que chaque parcelle contienne exactement deux types de plantes et que le nombre de parcelles soit minimum.

\item Donner une répartition des plantes de façon à ce qu'une parcelle contienne trois plantes et que le nombre de parcelles soit minimum.
\end{enumerate}

\medskip
\begin{center}
  \begin{tikzpicture}
     \tikzstyle{VertexStyle}= [shape       = circle,
                               fill         = white,%
                               minimum size = 26pt,%
                               draw]
      \Vertex[x=1,y=0.8]{R}
      \Vertex[x=0.2,y=3.3]{Po}
      \Vertex[x=0,y=2]{Pt}
      \Vertex[x=0.9,y=5]{Px}
      \Vertex[x=3.5,y=5]{A}
      \Vertex[x=5.6,y=3.4]{T}
      \Vertex[x=5.3,y=2]{Co}
      \Vertex[x=3.3,y=0.2]{Ch}
      \Edges(Po,Px,Po,A,Po,T,Po,Co,Po,Ch)
    \end{tikzpicture}
\end{center}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent

\bigskip
\begin{tkzexample}[code only]
\begin{tikzpicture}
 \tikzstyle{VertexStyle}= [shape       = circle,
                           fill         = white,%
                           minimum size = 26pt,%
                           draw]
  \Vertex[x=1,y=0.8]{R}
  \Vertex[x=0.2,y=3.3]{Po}
  \Vertex[x=0,y=2]{Pt}
  \Vertex[x=0.9,y=5]{Px}
  \Vertex[x=3.5,y=5]{A}
  \Vertex[x=5.6,y=3.4]{T}
  \Vertex[x=5.3,y=2]{Co}
  \Vertex[x=3.3,y=0.2]{Ch}
  \Edges(Po,Px,Po,A,Po,T,Po,Co,Po,Ch)
\end{tikzpicture}
\end{tkzexample}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         France mai 2004
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{France  juin 2004}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

Le graphe ci-dessous indique, sans respecter d'échelle, les parcours possibles entre les sept bâtiments d'une entreprise importante.

\medskip
\begin{tikzpicture}
  \SetGraphUnit{5}
  \Vertex{A}
  \NOEA(F){B}
  \SOEA(F){E}
  \EA(B){C}
  \EA(E){D}
  \NO(D){A}
  \Edges(F,E,F,D,F,C,F,A,F,B,A,E,E,D,D,A,B,A,C,B,E,B)
\end{tikzpicture}

Un agent de sécurité effectue régulièrement des rondes de surveillance. Ses temps de parcours en minutes entre deux bâtiments sont les
suivants :

\medskip
\begin{center}
\begin{minipage}{0.5\textwidth}
    \begin{itemize}
    \item AB : 16 minutes ;
    \item AG : 12 minutes ;
    \item BC : 8 minutes ;
    \item BE : 12 minutes ;
    \item BG : 8 minutes ;
    \item CD : 7 minutes ;
    \item CE : 4 minutes ;
    \item CG : 10 minutes ;
    \item DE : 2 minutes ;
    \item EF : 8 minutes ;
    \item EG : 15 minutes ;
    \item FG : 8 minutes.
    \end{itemize}
\end{minipage}
\end{center}

\medskip
Sur chaque arête, les temps de parcours sont indépendants du sens de parcours.

\begin{enumerate}
\item En justifiant la réponse, montrer qu'il est possible que l'agent de sécurité passe une fois et une seule par tous les chemins de cette usine. Donner un exemple de trajet.

\item L'agent de sécurité peut-il revenir à son point de départ après avoir parcouru une fois et une seule tous les chemins ? Justifier la réponse.

\item Tous les matins, l'agent de sécurité part du bâtiment A et se rend au bâtiment D.

En utilisant un algorithme que l'on explicitera, déterminer le chemin qu'il doit suivre pour que son temps de parcours soit le plus court possible, et donner ce temps de parcours.
\end{enumerate}

\medskip
\begin{tkzexample}[code only]
\begin{tikzpicture}
   \SetGraphUnit{5}
    \Vertex{A}   \NOEA(F){B}  \SOEA(F){E}
    \EA(B){C}    \EA(E){D}    \NO(D){A}
    \Edges(F,E,F,D,F,C,F,A,F,B,A,E,E,D,D,A,B,A,C,B,E,B)
\end{tikzpicture}
\end{tkzexample}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                         La Reunion mai 2004
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{La Réunion juin 2004 }\label{larj04} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>


\textbf{Partie A}

On note $G$ le graphe représenté ci-dessous et $M$ sa matrice obtenue en prenant les sommets dans l'ordre alphabétique. La matrice $M^3$ est également donnée.

\medskip
\begin{center}
\begin{tikzpicture}[>=latex]
    \SetGraphUnit{4.5}
    \Vertex {e}
    \NOEA(e){f}
    \SOEA(e){d}
    \SOEA(f){h}
    \Vertex[position={above of=e,yshift=2cm}]{g}
    \Vertex[position={left  of=g,xshift=-1cm}]{c} 
    \Vertex[position={left  of=d,xshift=-2cm}]{a} 
    \SOWE(c){b}
    \Edges(a,c,g)  \Edges(d,h,f,e,d,a,e,g,a,b,c,e)
    \Edge[style={bend left}](g)(h)
\end{tikzpicture}
\end{center}

\bigskip
\begin{center}
 $M^3 = \begin{pmatrix}
    10  &   8   &   11  &   10  &   12  &   5   &   13  &   4\\
    8   &   2   &   7   &   3   &   5   &   2   &   4   &   3\\
    11  &   7   &   8   &   6   &   12  &   3   &   10  &   5\\
    10  &   3   &   6   &   2   &   11  &   1   &   4   &   8\\
    12  &   5   &   12  &   11  &   8   &   8   &   13  &   3\\
    5   &   2   &   3   &   1   &   8   &   0   &   2   &   6\\
    13  &   4   &   10  &   4   &   13  &   2   &   6   &   9\\
    4   &   3   &   5   &   8   &   3   &   6   &   9   &   0\\
\end{pmatrix}$
\end{center}


\bigskip
Dire, en justifiant votre réponse, si les affirmations suivantes sont vraies ou
 fausses :

\begin{enumerate}
\item L'ordre du graphe est égal au plus grand des degrés des sommets.
\item Le graphe $G$ contient un sous-graphe complet d'ordre $3$.
\item Les sommets de $G$ peuvent être coloriés avec trois couleurs sans que deux sommets adjacents soient de même couleur.
\item Il est possible de parcourir ce graphe en passant une fois et une seule par chaque arête.
\item Il existe au moins un chemin de longueur $3$ qui relie chaque sommet à chacun  des sept autres sommets du graphe.
\item il y a $72$ chemins de longueur $3$ qui relient le sommet $e$ à chacun des huit sommets du graphe.
\end{enumerate}

\newpage

\textbf{ Partie B}

Le graphe suivant représente un réseau de lignes d'autobus. Les sommets du graphe désignent les arrêts. Les poids des arêtes sont les durées de parcours,  en minutes, entre deux arrêts (correspondances comprises).

\medskip
\begin{center}
\begin{tikzpicture}[>=latex]
      \SetGraphUnit{4.5}
    \Vertex {e}
    \NOEA(e){f}
    \SOEA(e){d}
    \SOEA(f){h}
    \Vertex[position={above  of=e,yshift=2cm}]{g}
    \Vertex[position={left  of=g,xshift=-1cm}]{c}
    \Vertex[position={left  of=d,xshift=-2cm}]{a}
    \SOWE(c){b}
    \tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=$3$](a)(b)
    \Edge[label=$11$](a)(c)
    \Edge[label=$6$](a)(e)
    \Edge[label=$17$](a)(d)
    \Edge[style={pos=.25},label=$20$](a)(g)
    \Edge[label=$5$](c)(b)
    \Edge[label=$6$](c)(e)
    \Edge[label=$7$](c)(g)
    \Edge[label=$7$](f)(e)
    \Edge[label=$3$](d)(e)
    \Edge[label=$9$](d)(h)
    \Edge[label=$6$](g)(e)
    \Edge[style={bend left},label=$11$](g)(h)
    \Edge[label=$4$](f)(h)
\end{tikzpicture}
\end{center}

\medskip
Déterminer, à l'aide d'un algorithme, la durée minimum pour aller de l'arrêt $a$  à l'arrêt $h$ et donner ce trajet.
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Code du graphe précédent

\medskip
\begin{tkzexample}[code only]
\begin{tikzpicture}[>=latex]
    \SetGraphUnit{4.5}
    \Vertex {e}
    \NOEA(e){f}
    \SOEA(e){d}
    \SOEA(f){h}
    \Vertex[position={above of=e,yshift=2cm}]{g}
    \Vertex[position={left  of=g,xshift=-1cm}]{c} 
    \Vertex[position={left  of=d,xshift=-2cm}]{a} 
    \SOWE(c){b}
    \Edges(a,c,g)  \Edges(d,h,f,e,d,a,e,g,a,b,c,e)
    \Edge[style={bend left}](g)(h)
\end{tikzpicture}
\end{tkzexample}

et

\begin{tkzexample}[code only]
\begin{tikzpicture}[>=latex]
    \SetGraphUnit{4.5}
    \Vertex {e}
    \NOEA(e){f}
    \SOEA(e){d}
    \SOEA(f){h}
    \Vertex[position={above  of=e,yshift=2cm}]{g}
    \Vertex[position={left  of=g,xshift=-1cm}]{c}
    \Vertex[position={left  of=d,xshift=-2cm}]{a}
    \SOWE(c){b}
    \tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=$3$](a)(b)
    \Edge[label=$11$](a)(c)
    \Edge[label=$6$](a)(e)
    \Edge[label=$17$](a)(d)
    \Edge[style={pos=.25},label=$20$](a)(g)
    \Edge[label=$5$](c)(b)
    \Edge[label=$6$](c)(e)
    \Edge[label=$7$](c)(g)
    \Edge[label=$7$](f)(e)
    \Edge[label=$3$](d)(e)
    \Edge[label=$9$](d)(h)
    \Edge[label=$6$](g)(e)
    \Edge[style={bend left},label=$11$](g)(h)
    \Edge[label=$4$](f)(h)
\end{tikzpicture}
\end{tkzexample}

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Amérique du Sud Nov 2006}\label{amsn06} 
\begin{enumerate}
\item À l'occasion de la coupe du monde de football 2006 en Allemagne, une agence touristique organise des voyages en car à travers les différentes villes où se joueront les matchs d'une équipe nationale.

Les routes empruntées par les cars sont représentées par le graphe ci-dessous. Le long de chaque arête figure la distance en kilomètres séparant les villes.
Les lettres B, D, F, H, K, M, N et S représentent les villes Berlin, Dortmnd, Francfort, Hambourg, Kaiserslautern, Munich, Nuremberg et Stuttgart.

\bigskip

\begin{center}
\begin{tikzpicture}
  \Vertex[x=0 ,y=0]{K}
  \Vertex[x=0 ,y=2]{F}
  \Vertex[x=-1,y=4]{D}
  \Vertex[x=3 ,y=7]{H}
  \Vertex[x=8 ,y=5]{B}
  \Vertex[x=9 ,y=2]{N}
  \Vertex[x=5 ,y=0]{M}
  \Vertex[x=3 ,y=1]{S}
  \tikzstyle{LabelStyle}=[fill=white,sloped]
  \tikzstyle{EdgeStyle}=[bend left]
  \Edge[label=$120$](K)(F)
  \Edge[label=$650$](H)(S)
  \Edge[label=$780$](H)(M) 
  \Edge[label=$490$](D)(B) 
  \Edge[label=$600$](D)(M)
  \Edge[label=$580$](B)(M)
  \Edge[label=$600$](H)(N)
  \Edge[label=$490$](F)(H)
  \tikzstyle{EdgeStyle}=[bend right]
  \Edge[label=$630$](S)(B)
  \Edge[label=$210$](S)(N) 
  \Edge[label=$230$](S)(M) 
\end{tikzpicture}
\end{center}

\bigskip
En précisant la méthode utilisée, déterminer le plus court chemin possible pour aller de Kaiserslautern à Berlin en utilisant les cars de cette agence.
\item Pour des raisons de sécurité, les supporters de certaines équipes nationales participant à la coupe du monde de football en 2006 ne peuvent être logés dans le même hôtel.

On donne ci-dessous le graphe d'incompatibilité entre les supporters de différentes équipes : par exemple, un supporter de l'équipe A ne peut être logé avec un supporter de l'équipe P.

\bigskip
\begin{center}
\begin{tikzpicture}
 \tikzstyle{EdgeStyle}=[bend left]
 \Vertex[x=0,y=0]{G}
 \Vertex[x=0,y=3]{A} 
 \Vertex[x=3,y=5]{P}
 \Vertex[x=4,y=2]{C}
 \Vertex[x=8,y=3]{Q}
 \Vertex[x=7,y=0]{E}
 \Vertex[x=3,y=-1]{R}
 \Edges(G,A,P,Q,E) \Edges(C,A,Q) \Edges(C,R,G) \Edges(P,E,A)
\end{tikzpicture}
\end{center}

\bigskip
\begin{enumerate}
\item  Déterminer le nombre chromatique de ce graphe en justifiant la valeur trouvée. 
\item  Proposer une répartition des supporters par hôtel en utilisant un nombre minimum d'hôtels.
\end{enumerate}
\end{enumerate}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\vfill\newpage\null 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                        Liban juin 2006
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
\subsection{Liban juin 2006 }\label{lib06} 
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

\begin{enumerate}
\item  Dans un parc, il y a cinq bancs reliés entre eux par des allées.

On modélise les bancs par les sommets A, B, C, D, E et les allées par les arêtes du
graphe G ci-dessous :


\medskip
\begin{center}
\begin{tikzpicture}
     \SetGraphUnit{3} 
    \tikzstyle{VertexStyle}=[shape        = circle,
                             fill         = black,
                             minimum size = 20pt,
                             text         = white,
                             draw]   
    \Vertex[L= {\textbf{E}}]{E}
    \NOEA[L  = {\textbf{A}}](E){A}
    \SOEA[L  = {\textbf{D}}](E){D}
    \EA[L    = {\textbf{C}}](D){C}
    \NOEA[L  = {\textbf{B}}](C){B}  
   \tikzstyle{EdgeStyle}=[double           = orange,%
                          double distance  = 1pt,%
                          thick,%
                          bend right       = 20]
    \Edges(B,A,E,D,C,B,D)
\end{tikzpicture}
\end{center}

\medskip

\begin{enumerate}
\item On désire peindre les bancs de façon que deux bancs reliés par une allée soient
toujours de couleurs différentes.

Donner un encadrement du nombre minimal de couleurs nécessaires et justifier.

Déterminer ce nombre.
\item Est-il possible de parcourir toutes les allées de ce parc sans passer deux fois par
la même allée?
\end{enumerate}
\item Une exposition est organisée dans le parc. La fréquentation devenant trop importante, on décide d'instaurer un plan de circulation : certaines allées deviennent à sens unique, d'autres restent à double sens. Par exemple la circulation dans l'allée
située entre les bancs B et C pourra se faire de B vers C et de C vers B, alors que la circulation dans l'allée située entre les bancs A et B ne pourra se faire que de A vers B. Le graphe G$'$ ci-dessous modélise cette nouvelle situation :

\medskip
\begin{center}
\begin{tikzpicture}
     \SetGraphUnit{3} 
    \tikzstyle{VertexStyle}=[shape        = circle,
                             fill         = black,
                             minimum size = 20pt,
                             text         = white,
                             draw]   
    \tikzstyle{TempStyle}=[double           = orange,%
                           double distance  = 1pt]
    \Vertex[L= {\textbf{E}}]{E}
    \NOEA[L  = {\textbf{A}}](E){A}
    \SOEA[L  = {\textbf{D}}](E){D}
    \EA[L    = {\textbf{C}}](D){C}
    \NOEA[L  = {\textbf{B}}](C){B}  
    \tikzstyle{EdgeStyle}=[TempStyle,%
                           post,%
                           bend right      = 20]
    \Edges(A,E,D,C,B,D)
    \tikzstyle{EdgeStyle}=[TempStyle,%
                           pre,%
                           bend right      = 20]
    \Edges(B,A) 
    \tikzstyle{EdgeStyle}=[TempStyle,%
                           pre,%
                           bend left       = 20]
    \Edges(A,E,D,C,B)
\end{tikzpicture}
\end{center}

\begin{enumerate}
\item Donner la matrice M associée au graphe G$'$. (On ordonnera les sommets
par ordre alphabétique).
\item On donne M$^5
= \begin{pmatrix}
1& 6& 9& 6& 10\\
4& 5& 7& 11& 5\\
4& 6& 6& 11& 5\\
1& 5& 10& 6& 10\\
6& 5& 5& 14& 2\\
\end{pmatrix}$

Combien y a-t-il de chemins de longueur 5 permettant de se rendre du
sommet D au sommet B ?

Les donner tous.
\item Montrer qu'il existe un seul cycle de longueur 5 passant par le sommet A.

Quel est ce cycle ?

En est-il de même pour le sommet B ?
 \end{enumerate}
\end{enumerate}

\vfill\newpage\null
Code des graphes précédents

\begin{tkzexample}[code only]
\begin{tikzpicture}
   \SetGraphUnit{3} 
   \tikzstyle{VertexStyle}=[shape        = circle,
                            fill         = black,
                            minimum size = 20pt,
                            text         = white,
                            draw]
   \Vertex[L= {\textbf{E}}]{E}
   \NOEA[L  = {\textbf{A}}](E){A}
   \SOEA[L  = {\textbf{D}}](E){D}
   \EA[L    = {\textbf{C}}](D){C}
   \NOEA[L  = {\textbf{B}}](C){B} 
   \tikzstyle{EdgeStyle}=[double           = orange,
                          double distance  = 1pt,
                          thick,
                          bend right       = 20]
    \Edges(B,A,E,D,C,B,D)
\end{tikzpicture}
\end{tkzexample}

\begin{tkzexample}[code only]
\begin{tikzpicture}
     \SetGraphUnit{3} 
    \tikzstyle{VertexStyle}=[shape        = circle,
                             fill         = black,
                             minimum size = 20pt,
                             text         = white,
                             draw]
    \tikzstyle{TempStyle}=[double           = orange,
                           double distance  = 1pt]
    \Vertex[L= {\textbf{E}}]{E}
    \NOEA[L  = {\textbf{A}}](E){A}
    \SOEA[L  = {\textbf{D}}](E){D}
    \EA[L    = {\textbf{C}}](D){C}
    \NOEA[L  = {\textbf{B}}](C){B}
    \tikzstyle{EdgeStyle}=[TempStyle,
                           post,
                           bend right      = 20]
    \Edges(A,E,D,C,B,D)
    \tikzstyle{EdgeStyle}=[TempStyle,%
                           pre,%
                           bend right      = 20]
    \Edges(B,A) 
    \tikzstyle{EdgeStyle}=[TempStyle,%
                           pre,%
                           bend left       = 20]
    \Edges(A,E,D,C,B)
\end{tikzpicture}
\end{tkzexample}


\endinput

==> tkz-graph/doc/latex/TKZdoc-gr-couverture.tex <==
% $Id$
\thispagestyle{empty}
\null\vfill
\begin{center}
\textcolor{Brown}{\fontsize{30}{30}\selectfont{\upshape tkz-graph.sty}}

\vspace{0.25cm}
\hfill\textcolor{Brown}{\fontsize{14}{14}\selectfont{\upshape   Alain Matthes}}
\end{center}

\vspace{3cm}
\begin{center} 
\begin{tikzpicture}[scale=5]
   \SetVertexNoLabel
   \tikzstyle{VertexStyle}=[draw,
                            shape        = circle,
                            shading      = ball,
                            ball color   = blue!50,
                            inner sep    = 10pt,
                            outer sep    = 0pt]
    \tikzstyle{EdgeStyle}= [thick,
                            double = blue,%
                            double distance = 1pt] 
    \draw[fill  = white,color = white] circle (0.55cm);
    \draw (0,0)  node[circle,draw,shade,
                      ball color    = orange,
                      minimum size = 3cm] (am){\textbf{AlterMundus}};
     \grIcosahedral[RA=1.4,RB=0.8]
\end{tikzpicture}
\end{center} 
\vfill\newpage\null\thispagestyle{empty}
\endinput



==> tkz-graph/doc/latex/TKZdoc-gr-edge.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex

% $Id$
\section{Edge avec tkz-graph}

\begin{NewMacroBox}{Edge}{\oarg{local options}\varp{Vertex A}\varp{Vertex B}}

\begin{tabular}{lllc} 
options              & défaut     & définition       \\ \midrule
\TOline{local}       {false}      {booléen désactive EdgeStyle } 
\TOline{color}       {\textbackslash EdgeColor}  {couleur de l'arête}       
\TOline{lw}          {\textbackslash EdgeLineWidth} {épaisseur de l'arête.} 
\TOline{label}       {\{\}}    {le label}                        
\TOline{labeltext}   {black}    {couleur du texte}               
\TOline{labelcolor}  {white}    {couleur du fond du label }      
\TOline{labelstyle}  {\{\}}  {modication du style du label}      
\TOline{style}       {pos=.5}   {modification du style général}                  \bottomrule
\end{tabular}

\medskip
\emph{Cette macro permet de tracer une arête entre deux sommets. Dans les exemples et dans le chapitre sur les styles, l'usage des styles est expliqué.  }
\end{NewMacroBox}



\medskip
\subsection{Utilisation de \addbs{Edge}}
 On peut remarquer qu'il y a deux sortes d'arêtes au niveau de la forme  : les segments et les arcs. De plus, ces arêtes peuvent avoir un label. La notion de style est importante car on peut définir pour toutes les arêtes un même style dès le début.

par défaut :

\begin{tkzexample}[latex=8cm, small]
\begin{tikzpicture}
  \SetGraphUnit{4}
  \Vertex{a}
  \EA(a){b} 
  \SO[unit=2](a){c}
  \EA(c){d}
 {\SetGraphUnit{2}  
  \SO(c){e}}
  \EA(e){f}
  \Edge(a)(b)
  \tikzset{EdgeStyle/.style = {-,bend left}}
  \Edge(c)(d)
  \tikzset{EdgeStyle/.style = {->,bend right=60}}
  \Edge(e)(f)
\end{tikzpicture}
\end{tkzexample}




\vfill
\newpage

\subsection{Arête particulière la boucle : \tkzname{Loop}} 

\begin{NewMacroBox}{Loop}{\oarg{local options}\varp{Vertex}}
\begin{tabular}{lllc}
options              & défaut     & définition       \\
\midrule
\TOline{color}       {black  }  {} 
\TOline{lw}          {0.8pt  }  {} 
\TOline{label}       {\{\}     }  {} 
\TOline{labelstyle}  {\{\}     }  {} 
\TOline{style}       {\{\}     }  {} 
\end{tabular}
\end{NewMacroBox}

\subsubsection{Exemple avec \tkzcname{Loop}}  
\begin{center}
\begin{tkzexample}[vbox, small]
\begin{tikzpicture}
 \useasboundingbox (-1,-2) rectangle (8,2);
 \SetVertexSimple
 \SetGraphUnit{5}  
 \Vertex{A}
 \EA(A){B}
 \Edge[style={->}](A)(B) 
 \Loop[dist=3cm,dir=EA,style={thick,->}](B)  
 \Loop[dist=5cm,dir=WE,style={thick,->}](A)
\end{tikzpicture}
\end{tkzexample} 
\end{center}

\vfill
\newpage
\subsection{Multiple arêtes  \tkzcname{Edges}}  

\begin{NewMacroBox}{Edges}{\oarg{local options}\varp{Vertex A,Vertex B,\dots}}

\begin{tabular}{llc}
options              & défaut     & définition       \\
\midrule
\TOline{color}    {black} {}
\TOline{lw}       {thick} {}
\TOline{label}    {\{\} } {}      
\TOline{labelstyle}{\{\}} {}     
\TOline{style}    {\{\} } {}      
\bottomrule
\end{tabular}

\medskip
\emph{ Cette macro permet de définir une série d'arêtes en une seule fois.}
\end{NewMacroBox} 

\subsubsection{Exemple avec \tkzcname{Edges}}    
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetGraphUnit{4}
  \GraphInit[vstyle=Art]
  \Vertices{circle}{a0,a1,a2,a3,a4,a5,a6,a7} 
  \Edges(a0,a3,a6,a1,a4,a7,a2,a5,a0)
\end{tikzpicture}
\end{tkzexample}
\end{center} 


\endinput


==> tkz-graph/doc/latex/TKZdoc-gr-installation.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex
% $Id$

\section{Installation}

Il est possible que lorsque vous lirez ce document, \tkzname{tkz-graph} soit présent sur les serveurs du \tkzname{CTAN}\footnote{\tkzname{tkz-graph} ne fait pas encore partie de \tkzname{TeXLive} mais il sera bientôt possible de l'installer avec \emph{tlmgr}}.  Si   \tkzname{tkz-graph} ne fait pas encore partie de votre distribution, cette section vous montre comment l'installer. 

\subsection{Avec TeXLive sous OS X, Linux et Windows}\NameDist{TeXLive}
Créer un dossier \tikz[remember picture,baseline=(n1.base)]\node [fill=green!20,draw] (n1) {tkz};  avec comme chemin : \colorbox{blue!20}{ texmf/tex/latex/tkz}.

 \colorbox{blue!20}{texmf} est un dossier personnel, voici les chemins de ce dossier sur mes deux ordinateurs:

\medskip
\begin{itemize}\setlength{\itemsep}{10pt}

\item   sous OS X\NameSys{OS X} \colorbox{blue!20}{\textbf{/Users/ego/Library/texmf}}; 

\item   sous Ubuntu\NameSys{Linux Ubuntu} \colorbox{blue!20}{\textbf{/home/ego/texmf}}.

\end{itemize} 

 Sous Windows je ne connais pas cette distribution sous ce système, mais je suppose que l'installation doit ressembler à ce qui se passe sous Linux et OS X.  
 
\medskip
\begin{enumerate}
\item Placez \tikz[remember picture,baseline=(n2.base)]\node [fill=green!20,draw] (n2) {tkz-graph.sty}; dans le dossier \colorbox{green!20}{tkz}.
\item Ouvrir un terminal, puis faire \colorbox{red!30}{|sudo texhash|}
\item Vérifier que \tkzname{xkeyval}\index{xkeyval} version 2.5 minimum et \tkzname{Ti\emph{k}Z 2.1}\index{TikZ@Ti\emph{k}Z} sont installés car ils sont obligatoires, pour le bon fonctionnement de \tkzname{tkz-graph}.
\end{enumerate}
Mon dossier texmf est structuré ainsi : 

\emph{Attention, la présence dans mon dossier texmf, des fichiers de \PGF, s'explique par l'utilisation de la version CVS de \PGF}.

\vfill
\begin{tikzpicture} [remember picture,rotate=90] 
% nodes
\node (texmf)   at (4,2)   [draw,fill=blue!20 ] {texmf};

\node (tex)     at (6,0)   [draw ] {tex}; 
\node (doc)     at (2,0)   [draw ] {doc};

\node (texgen)  at (7,-2)  [draw ] {generic};
\node (docgen)  at (0,-2)  [draw ] {generic};

\node (latex)   at (4,-2)  [draw ] {latex}; 

\node (genpgf)  at (7,-4)  [draw] {pgf};
\node (latpgf)  at (5,-4)  [draw] {pgf};
\node (tkz)     at (4,-4)  [draw,fill=green!20 ] {tkz};

\node (docpgf)  at (0,-4)  [draw] {pgf};

\node (tkb)     at (6,-6)  [draw,fill=orange!20]  {tkzbase};
\node (tke)     at (2,-6)  [draw,fill=orange!20]  {tkzeuclide};

\node (tari)    at (7,-11)  [draw,fill=orange!20] {tkz-tools-arith.tex};   
\node (tary)    at (5,-11)  [draw,fill=green!20]  {tkz-arith.sty};
\node (tgra)    at (4,-11)  [draw,fill=green!20]  {tkz-graph.sty}; 
\node (tber)    at (3,-11)  [draw,fill=green!20]  {tkz-berge.sty};

% edges
\draw[-open triangle 90](texmf.north east) -- (tex.south west)    ;
\draw[-open triangle 90](texmf.south east) -- (doc.north west)    ;
                                                                  
\draw[-open triangle 90](tex.north east)   -- (texgen.south west) ;
\draw[-open triangle 90](tex.south east)   -- (latex.north west)  ; 
\draw[-open triangle 90](texgen.east)      -- (genpgf.west)       ;  
                                                                  
\draw[-open triangle 90](doc.south east)   -- (docgen.north west) ; 
\draw[-open triangle 90](docgen.east)      -- (docpgf.west)       ; 

\draw[-open triangle 90](latex.north east) -- (latpgf.south west) ; 
\draw[-open triangle 90](latex.east)       -- (tkz.west)          ;    
 
\draw[-open triangle 90,orange!80](tkz.east) to [out=-90,in=90](tkb.west)  ; 
\draw[-open triangle 90,orange!80](tkz.east) to [out=-90,in=90](tke.west)  ; 
\draw[-open triangle 90,orange!80](tkb.east) to [out=-90,in=90](tari.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tary.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tgra.west) ; 
\draw[-open triangle 90,green!80](tkz.east) to [out=-90,in=90](tber.west) ;  

\end{tikzpicture}

\begin{tikzpicture}[remember picture,overlay]
        \path[->,thin,green!80,>=latex] (n1) edge [bend left] (tkz);
        \path[->,thin,green!80,>=latex] (n2) edge [bend left] (tgra);
\end{tikzpicture}     

\vfill
\newpage
\subsection{Avec MikTeX sous Windows XP}\NameDist{MikTeX}\NameSys{Windows XP}

Il est fort possible que lorsque vous lirez ces lignes, il soit possible d'installer \tkzname{tkz-graph} automatiquement à l'aide du manager de MikTeX.

Un utilisateur de mes packages \tkzimp{Wolfgang Buechel} a eu la gentillesse de me faire parvenir ce qui suit, et cela permet d'installer manuellement mon package~:

Pour ajouter \tkzname{tkz-graph.sty} à MiKTeX\footnote{Essai réalisé avec la version \tkzname{2.7}}:

\begin{itemize}\setlength{\itemsep}{10pt}
  \item ajouter un dossier \tkzname{tkz} dans le dossier
       \colorbox{blue!30}{\texttt{[MiKTeX-dir]/tex/latex}};
  \item copier \tkzname{tkz-graph.sty} dans ce dossier;
  \item mettre à jour  MiKTeX, pour cela dans shell DOS lancer la commande   \colorbox{red!30}{|mktexlsr -u|}  ou bien encore, choisir \colorbox{red!30}{|Start/Programs/Miktex/Settings/General|}
puis appuyer sur le bouton  \colorbox{red!30}{|Refresh FNDB|}.
\end{itemize}


\endinput


==> tkz-graph/doc/latex/TKZdoc-gr-label.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex

% $Id$
\section{Les labels}
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%                             Options sur les labels
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
Rappel : Si aucun label n'est donné alors l'affichage du label est celui de la référence du \tkzname{vertex}. Il est possible de modifier localement  le comportemnt des labels

\subsection{Options concernant les labels}

L'option suivante permet de définir un label, celui-ci peut être en mode texte ou bien en mode math. 

\subsubsection{Option \tkzname{L}} 

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \Vertex[L=$\alpha$] {a}
   \EA[unit=4](a){b}
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Option \tkzname{Math}} 
Le label est en mode math. Il est inutile de placer L en mode math si l'option est utilisée.

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \Vertex[Math] {A_1}
   \Vertex[Math,L=\alpha,x=4,y=0] {a}
\end{tikzpicture}
\end{tkzexample}


\subsubsection{Suppression d'un  label, Option \tkzname{NoLabel}} 
Cette option supprime l'affichage du label. Il est préférable d'utiliser \tkzname{SetVertexNoLabel} si on veut généraliser à tous les sommets.   

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \SetGraphUnit{4}
   \Vertex[NoLabel]{A}
   \EA[NoLabel](A){B}  
\end{tikzpicture}
\end{tkzexample} 

\subsubsection{Option \tkzname{LabelOut}, \tkzname{Lpos} et \tkzname{Ldist}}

La première option permet de placer le label hors du node, la deuxième positionne le label autour du sommet et la dernière spécifie la distance entre le label et le sommet.

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
      \Vertex[LabelOut]{A}
      \Vertex[LabelOut,Lpos=60,
              Ldist=.5cm,x=2,y=0]{B}
      \Vertex[LabelOut,Lpos=60,x=4,y=0]{C}
\end{tikzpicture}
\end{tkzexample}  


\vfill\newpage 
On peut souhaiter appliquer une option pour tous les sommets.  

\subsection{\tkzcname{SetVertexNoLabel}}
On peut souhaiter ne pas avoir de label pour tous les sommets avec un style prédéfini. 

\begin{NewMacroBox}{SetVertexNoLabel}{}
\emph{ Cette macro permet de supprimer les labels sur tous les sommets. Elle agit globalement sur tous les sommets. Elle correspond à l'option  \tkzname{NoLabel}.}
\end{NewMacroBox}
 
\subsubsection{Suppression des labels} 

\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetGraphUnit{4}
  \SetVertexNoLabel
  \Vertex{A}\EA(A){B}
\end{tikzpicture}
\end{tkzexample}   


\subsection{\tkzcname{SetVertexMath} } 
\begin{NewMacroBox}{SetVertexMath}{}
\emph{Cette macro permet d'appliquer l'option \tkzname{Math} à plusieurs  sommets. Elle agit globalement sur tous les sommets. Elle correspond à l'option  \tkzname{Math}}
\end{NewMacroBox}

\begin{tkzexample}[latex=7cm,small]
	\begin{tikzpicture}
  \SetVertexMath
  \Vertex {A_1}  \EA[unit=3](A_1){A_2}\texttt{}
\end{tikzpicture}
\end{tkzexample} 

\subsection{\tkzcname{SetVertexLabel}}  
\begin{NewMacroBox}{SetVertexLabel}{}
\emph{ Cette macro autorise les labels. Elle agit globalement sur tous les sommets.}
\end{NewMacroBox} 

\subsubsection{Labels  supprimés puis autorisés.} 
 Dans l'exemple qui suit, les labels sont supprimés puis autorisés.
 
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
  \SetVertexNoLabel     
  \SetGraphUnit{2} 
  \Vertex {A}      \EA(A){B}
  \SetVertexLabel  \EA(B){C}
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Label en dehors du sommet \tkzcname{SetVertexLabelOut}}

\begin{NewMacroBox}{SetVertexLabelOut}{}
\emph{\tkzcname{SetVertexLabelOut} Dans les exemples précédents, les sommets sont des petits disques colorés, généralement en noir et dans ce cas par défaut le label est à l'extérieur.  On peut contrôler la position à l'aide des labels avec   \tkzname{Ldist} et\tkzname{Lpos}.}
\end{NewMacroBox}

\begin{NewMacroBox}{SetVertexLabelIn}{}
\emph{\tkzcname{SetVertexLabelIn} permet d'écrire le label dans le sommet.}
\end{NewMacroBox}   

Cette macro permet d'appliquer l'option à plusieurs  sommets. \tkzcname{SetVertexLabelIn} annule l'effet.

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
  \SetGraphUnit{3}
  \SetVertexLabelOut
  \Vertex {A}    \EA(A){B}
  \SetVertexLabelIn  \SO[unit=3](B){C}
\end{tikzpicture}
\end{tkzexample}

\endinput  




% \subsection{\tkzname{NoLabel} } 
% 
%  \tkzname{NoLabel} Cela permet de supprimer le nom d'un sommet
% 
% \begin{tkzexample}[vbox]
% \begin{tikzpicture}
%      \SetGraphUnit{4}
% \tikzset{VertexStyle/.style = {shape        = circle,
%                           inner sep    = 0pt,
%                           outer sep    = 0pt,
%                           fill         = yellow,%
%                           minimum size = 16pt,%
%                           draw}}
% \Vertex[NoLabel]{A}\EA[NoLabel](A){B}
% \end{tikzpicture}
% \end{tkzexample}
% 




==> tkz-graph/doc/latex/TKZdoc-gr-prob.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/Graph/doc-fr/TKZdoc-gr-main.tex
% $Id$     
\section{Graphes probabilistes }
%<–––––––––––––––––––––––––– graphes probabilistes ––––––––––––––––––––––––––>
%<–––––––––––––––––——————————————————————————————————————————————————————————>
%<–––––––––––––––––——————————————————————————————————————————————————————————>
\subsection{La macro \tkzcname{grProb} } 
\begin{NewMacroBox}{grProb}{\oarg{local options} \var{left} \var{right} \var{N}\var{S}\var{W}\var{E}}

\begin{tabular}{lll}
Arguments   &   & Définition              \\
  \midrule
  \TAline{Vertex-left} {}{Nom du sommet à gauche}  
  \TAline{Vertex-right} {}{Nom du sommet à droite}  
  \TAline{label N} {}{Étiquette située en haut}  
  \TAline{label S} {}{Étiquette située en bas}   
  \TAline{label W} {}{Étiquette située à gauche} 
  \TAline{label E} {}{Étiquette située à droite} 
 \bottomrule
  \end{tabular}

\medskip
\begin{tabular}{lll}
options & défaut & définition                              \\ 
\midrule
\TOline{unit}      {4cm} {distance entre les sommets      } 
\TOline{LposA}     {180} {angle si label extérieur en A   } 
\TOline{LposB}     {0  }  {angle si label extérieur en B  } 
\TOline{Ldist}     {0cm} {écart entre le node et le label } 
\TOline{LoopDist}  {4cm} {longueur des boucles            }  
\bottomrule
\end{tabular}

\medskip
\emph{Cette macro permet de créer un graphe probabiliste d'ordre 2. }
\end{NewMacroBox}

\subsection{Utilisation de  \tkzcname{grProb} } 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \useasboundingbox (-2.5,-2) rectangle (7.5,2);
  \grProb{A}{B}{NO}{SO}{WE}{EA}
\end{tikzpicture}
\end{tkzexample}
\end{center}  

\begin{tkzexample}[latex=5cm]
\begin{tikzpicture}[scale=.5]
  \useasboundingbox (-2.5,-2) rectangle (5,2);
  \grProb[unit=4]{\Rain}{\Sun}{0,4}{0,3}{0,6}{0,7}
\end{tikzpicture}
\end{tkzexample}
 


                  

\subsection{\tkzcname{grProb} et le style par défaut }
\begin{center}
\begin{tkzexample}[latex=5cm]
\begin{tikzpicture}[scale=.5]
  \useasboundingbox (-2.5,-2) rectangle (5,2);
  \grProb{A}{B}{0,8}{0,6}{0,2}{0,4}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{\tkzcname{grProb} et le style « Simple »}
\begin{center}
\begin{tkzexample}[latex=5cm]
\begin{tikzpicture}[scale=.5] 
\useasboundingbox (-2.5,-2) rectangle (5,2);
\SetVertexSimple
\grProb[Ldist=0.2cm]{Paris}{Lyon}%
  {\scriptstyle\dfrac{2}{3}}{\scriptstyle\dfrac{3}{4}}%
  {\scriptstyle\dfrac{1}{3}}{\scriptstyle\dfrac{1}{4}}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{Utilisation d'un style personnalisé}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
 \useasboundingbox (-2.5,-2.5) rectangle (7.5,2.5);
 \tikzset{VertexStyle/.style = {shape        = circle, 
                                shading      = ball,
                                ball color    = Orange,
                                minimum size = 20pt,
                                draw,color=white}}
 \tikzset{LabelStyle/.style = {draw,color=orange,fill=white}}
 \tikzset{EdgeStyle/.style = {->, thick,
                              double          = orange, 
                              double distance = 1pt}}

\grProb[Ldist=0.1cm,LposA=0,LposB=180]%
            {Paris}{Lyon}%
            {\scriptstyle\dfrac{2}{3}}{\scriptstyle\dfrac{3}{4}}%
            {\scriptstyle\dfrac{1}{3}}{\scriptstyle\dfrac{1}{4}}%
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill
\newpage
\subsection{La macro \tkzcname{grProbThree}}

\begin{NewMacroBox}{grProbThree}{\oarg{local options} \var{right} \var{up}\var{down} \var{rr/ru/rd}\var{uu/ud/ur}\var{dd/dr/du}}

\begin{tabular}{llc}
Arguments   &   & Définition              \\
\midrule
\TAline{Vertex-right} {}{Nom du sommet à droite} 
\TAline{Vertex-up}    {}{Nom du sommet en haut}  
\TAline{Vertex-down}  {}{Nom du sommet en bas}   
\TAline{rr/ru/rd}     {}{arête partant de r vers r etc\dots}  
\TAline{uu/ud/ur}     {}{arête partant de u vers u etc\dots}  
\TAline{dd/dr/du}     {}{arête partant de d vers d etc\dots}  
\bottomrule
\end{tabular}
    
\medskip
\begin{tabular}{llc}
Options & Défaut & Définition                              \\ 
\midrule
\TOline{unit}  {4cm} {distance entre les sommets      }    
\TOline{LposA}     {180} {angle si label extérieur en A   }
\TOline{LposB}     {0  }  {angle si label extérieur en B  }
\TOline{Ldist}     {0cm} {écart entre le node et le label }
\TOline{LoopDist}  {4cm} {longueur des boucles            } 
\bottomrule
\end{tabular}
    
\medskip   
\emph{Cette macro permet de créer un graphe probabiliste d'ordre 3. }
\end{NewMacroBox} 

\subsubsection{Graphe probabiliste d'ordre 3}
\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}[scale=.75]
 \tikzset{LabelStyle/.style = {draw,fill=white}}
 \grProbThree[unit=4]{\Rain}{\Sun}{\Cloud}
  {0.1/0.3/0.6}{0.2/0.3/0.5}{0.25/0.35/0.4}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\endinput


==> tkz-graph/doc/latex/TKZdoc-gr-style.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex

% $Id$
\section{Modification des styles des sommets} 


Différentes méthodes sont possibles mais il faut distinguer une utilisation globale ou locale. 

Les trois principaux styles sont \tkzname{VertexStyle}, \tkzname{EdgeStyle} et \tkzname{LabelStyle}. Le dernier est attaché aux étiquettes que peuvent avoir les arêtes.    

\begin{enumerate}
\item \tkzcname{GraphInit} permet de choisir un style prédfini et il est possible de retoucher ces styles en modifiant les valeurs choisies par défaut.
\item Les styles  des sommets, des arêtes et étiquettes peuvent être personnalisés avec \tkzname{VertexStyle}, \tkzname{EdgeStyle} et \tkzname{LabelStyle}. On peut redéfinir ces styles  avec  \tkzcname{tikzset\{VertexStyle/.append style = \{ ... \}\}} ou bien \tkzcname{tikzset\{VertexStyle/.style = \{ ... \}\}}.  La première méthode modifie un style existant alors que la seconde  définit un style .
\item On peut utiliser les anciennes macros : \tkzcname{SetVertexSimple}, \tkzcname{SetVertexNormal}, \tkzcname{SetUpVertex} et \tkzcname{SetUpEdge} .

\end{enumerate}

\medskip  
Il est possible de mélanger tout cela en sachant que la dernière définition d'un style l'emporte.

\medskip
\begin{NewMacroBox}{GraphInit}{\oarg{local options}}
\begin{tabular}{llc}
Options           & Défaut  & Définition \\ \midrule
\TOline{vstyle}   {Normal}   {}           \bottomrule
\end{tabular}

\medskip 
Les possibilités pour \tkzname{vstyle} sont :

\begin{enumerate}
  \item  Empty,
  \item  Hasse,
  \item  Simple,
  \item  Classic,
  \item  Normal,
  \item  Shade,
  \item  Dijkstra
  \item  Welsh,
  \item  Art,
  \item  Shade Art.
\end{enumerate}

\emph{Il y a pour le moment 10 styles pré-définis. Il est possible de modifier les valeurs par défaut.}
\end{NewMacroBox} 


Utilisation des  styles pré-définis

\begin{enumerate}
\item GraphInit par défaut

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3}    
  \GraphInit[vstyle=Normal]
  \Vertex{A}\EA(A){B}
  \Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Empty|}

\begin{center}
\begin{tkzexample}[latex=7cm]
 \begin{tikzpicture}
   \SetGraphUnit{3} 
   \GraphInit[vstyle=Empty] 
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Hasse|}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Hasse]
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Simple|}

\begin{center}
\begin{tkzexample}[latex=7cm]
 \begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Simple]
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et   \tkzname{|vstyle=Classic|}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Classic]
  \Vertex[Lpos=-90]{A}
  \EA[Lpos=-90](A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

  \item GraphInit et   \tkzname{|vstyle=Normal|}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Normal]
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Classic]
  \Vertex[Lpos=-90]{Paris}
  \EA[Lpos=-90](Paris){Berlin}
  \Edge (Paris)(Berlin)
\end{tikzpicture}
\end{tkzexample}
\end{center}  

\item GraphInit et  \tkzname{|vstyle=Shade|} 

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Shade]
  \Vertex{A}\EA(A){B}\Edge(A)(B) 
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Dijkstra|}

\begin{center}
\begin{tkzexample}[latex=7cm]  
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Dijkstra]
  \Vertex{A}\EA(A){B}\Edge[label=$7$](A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Welsh|}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Welsh]
  \Vertex[Lpos=-90]{A}
  \EA[Lpos=-90](A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Art|}
\begin{center} 
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Art]
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\item GraphInit et  \tkzname{|vstyle=Shade Art|}
\begin{center} 
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
  \SetGraphUnit{3} 
  \GraphInit[vstyle=Shade Art]
  \Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}
\end{center}    
\end{enumerate}

\newpage
\tkzname{|vstyle|}  est basé sur les macros  suivantes qui peuvent être redéfinies.

\medskip 
\begin{tabular}{lc}\toprule
Commandes pour les styles   & utilisation      \\  \midrule
|\newcommand*{\VertexInnerSep}{0pt} |         &\\
|\newcommand*{\VertexOuterSep}{0pt} |         &\\
|\newcommand*{\VertexDistance}{3cm} |         &\\
|\newcommand*{\VertexShape}{circle}|          &\\
|\newcommand*{\VertexLineWidth}{0.8pt}|         &\\
|\newcommand*{\VertexLineColor}{black}|       &\\
|\newcommand*{\VertexLightFillColor}{white}|  &\\
|\newcommand*{\VertexDarkFillColor}{black}|   &\\
|\newcommand*{\VertexTextColor}{black}|       &\\
|\newcommand*{\VertexFillColor}{black}|       &\\
|\newcommand*{\VertexBallColor}{orange}|      &\\
|\newcommand*{\VertexBigMinSize}{24pt}|       &\\
|\newcommand*{\VertexInterMinSize}{18pt}|     &\\
|\newcommand*{\VertexSmallMinSize}{12pt}|     &\\
|\newcommand*{\EdgeFillColor}{orange}|        &\\
|\newcommand*{\EdgeArtColor}{orange}|         &\\
|\newcommand*{\EdgeColor}{black}|             &\\
|\newcommand*{\EdgeDoubleDistance}{1pt}|      &\\
|\newcommand*{\EdgeLineWidth}{0.8pt}|         &\\ \bottomrule
\end{tabular}



\subsection{Modification de \tkzname{vstyle=Art}}
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetGraphUnit{3}
  \GraphInit[vstyle=Art]
  \renewcommand*{\VertexInnerSep}{8pt} 
  \renewcommand*{\EdgeLineWidth}{3pt}
  \renewcommand*{\VertexBallColor}{blue!50}
  \Vertices{circle}{A,B,C,D,E}
  \Edges(A,B,C,D,E,A,C,E,B,D)
\end{tikzpicture}
\end{tkzexample}
\end{center} 


\vfill
\newpage

\subsection{Modification du style \tkzname{VertexStyle} par défaut}

Il est possible de redéfinir le style  \tkzcname{SetVertexSimple}.

Par défaut :

\begin{tkzltxexample}[]
\tikzset{VertexStyle/.style = {  
                             shape        = circle,
                             fill         = black,
                             inner sep    = 0pt,
                             outer sep    = 0pt,
                             minimum size = 8pt,
                             draw]
\end{tkzltxexample}

maintenant si on utilise ceci :

\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
   \SetVertexSimple  
   \tikzset{VertexStyle/.style = {
     shape        = rectangle,
     fill         = red,%
     inner sep    = 0pt,
     outer sep    = 0pt,
     minimum size = 10pt,
     draw}}
 \SetGraphUnit{3}
 \Vertex{A}\EA(A){B}
\end{tikzpicture}
\end{tkzexample}

\subsection{Modification d'un style \tkzname{VertexStyle}}

C'est le style par défaut pour les sommets mais on peut le modifier. Voici quelques exemples utilisés plus tard dans ce document

par défaut :

\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
\SetGraphUnit{3}
\tikzset{VertexStyle/.style = {% 
      shape        = circle,
      shading      = ball,
      ball color   = Orange,
      minimum size = 20pt,draw}}
 \SetVertexNoLabel
 \Vertex{A}\EA[unit=3](A){B}
\end{tikzpicture}
\end{tkzexample}

  ou bien encore:

\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
\SetGraphUnit{4}
\tikzset{VertexStyle/.style = {% 
      shape        = circle, 
      shading      = ball,
      ball color   = green!40!black,%
      minimum size = 30pt,draw}}
\SetVertexNoLabel
\Vertex{A}\EA[unit=3](A){B}
\end{tikzpicture}
\end{tkzexample}
 \vfill
\newpage   

\begin{NewMacroBox}{SetVertexSimple}{\oarg{local options}}

\medskip
\emph{Il est possible de modifier les styles prédéfinis. La macro \tkzcname{SetVertexSimple} permet d'affiner le style \og Simple \fg des sommets.}  
\begin{tabular}{llc}
  \toprule
options   & default  & definition           \\ \midrule
\TOline{Shape}     {\textbackslash VertexShape       }{} 
\TOline{MinSize}   {\textbackslash VertexSmallMinSize}{} 
\TOline{LineWidth} {\textbackslash VertexLineWidth   }{}  
\TOline{LineColor} {\textbackslash VertexLineColor   }{} 
\TOline{FillColor} {\textbackslash VertexFillColor   }{}  \bottomrule
\end{tabular}
\end{NewMacroBox}

\medskip
\subsection{Autre style \tkzcname{SetVertexSimple}}

\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
 \SetVertexSimple[Shape=diamond,
                  FillColor=blue!50]
 \Vertices[unit=3]{circle}{A,B,C,D,E}
 \Edges(A,B,C,D,E,A,C,E,B,D) 
\end{tikzpicture}
\end{tkzexample} 
\end{center}

\subsection{\tkzcname{SetVertexSimple}, \tkzname{inner sep} et \tkzname{outer sep}}
\begin{center}
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
\SetGraphUnit{3} 
\SetVertexSimple[MinSize    = 12pt,
                 LineWidth  = 4pt,
                 LineColor  = red,%
                 FillColor  = blue!60]
\tikzset{VertexStyle/.append style =
     {inner sep      = 0pt,%
      outer sep      = 2pt}}
\Vertices{circle}{A,B,C,D,E}
\Edges(A,B,C,D,E,A,C,E,B,D)
\end{tikzpicture}
\end{tkzexample}
\end{center}
 
\vfill
\newpage
\begin{NewMacroBox}{SetVertexNormal}{\oarg{local options}}
\begin{tabular}{llc} 
Options            & Défaut               & Définition   \\ \midrule
\TOline{color}      {\textbackslash EdgeColor        } {} 
\TOline{label}      {no default } {} 
\TOline{labelstyle} {no default    } {}  
\TOline{labeltext}  {\textbackslash LabelTextColor    } {} 
\TOline{labelcolor} {\textbackslash LabelFillColor    } {} 
\TOline{style}      {no default    } {} 
\TOline{lw}         {\textbackslash EdgeLineWidth    } {} 
 \bottomrule
\end{tabular}

\medskip
\emph{Macro semblable à la précédente.}
\end{NewMacroBox}

\subsection{Autre style \tkzcname{SetVertexNormal}} 
\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetGraphUnit{3}
  \SetVertexNormal[Shape     = rectangle,%
                   LineWidth = 2pt,%
                   FillColor = green!50]
  \Vertices{circle}{A,B,C,D,E}
  \Edges(A,B,C,D,E,A,C,E,B,D) 
\end{tikzpicture}
\end{tkzexample}
\end{center}


\vfill\newpage
\begin{NewMacroBox}{SetUpVertex}{\oarg{local options}}
\begin{tabular}{llc}
Options         & Défaut  & Définition                       \\ \midrule
\TOline{Lpos}    {-90  }   {position label externe      }     
\TOline{Ldist}   {0cm  }   {distance du label           }     
\TOline{style}   {{}   }   {permet d'affiner le style   }     
\TOline{NoLabel} {false}   {supprime le label           }     
\TOline{LabelOut}{false}   {Label externe               }      \bottomrule
\end{tabular}

\medskip
\emph{Cette macro permet de modifier les options précédentes. }
\end{NewMacroBox}

\subsection{\tkzcname{SetUpVertex}} 

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
  \SetGraphUnit{3}
  \SetUpVertex[Lpos=-60,LabelOut]
  \Vertex{A}\EA(A){B}
\end{tikzpicture}
\end{tkzexample} 


\subsection{\tkzcname{SetUpVertex} et \tkzcname{tikzset}} 

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
\SetGraphUnit{4}
\SetVertexLabel
\SetUpVertex[Lpos=-60,LabelOut]
\tikzset{VertexStyle/.append style =
 {outer sep    = .5\pgflinewidth}}
\renewcommand*{\VertexLineWidth}{6pt}
\Vertex{A}\EA(A){B}\Edge(A)(B)
\end{tikzpicture}
\end{tkzexample}

\vfill\newpage 
\section{Modification des styles des arêtes} 
 
\subsection{Utilisation de l'option \tkzname{style} de la macro \tkzcname{Edge}} 

\subsubsection{Exemple 1}
\begin{tkzexample}[latex=8cm, small]
\begin{tikzpicture}
  \SetGraphUnit{4}  
  \Vertex{e}
  \EA(e){f}
  \Edge(f)(e)
  \Edge[style={bend left}](f)(e)
  \Edge[style={bend right}](f)(e)
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Exemple 2} 
\begin{tkzexample}[latex=8cm, small]
\begin{tikzpicture}
  \SetGraphUnit{4}  
  \Vertex{e}
  \EA(e){f}
  \Edge[style={->,bend left}](f)(e)
  \Edge[style={<-,bend right}](f)(e)
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Exemple 3} 
\begin{tkzexample}[latex=8cm, small]
\begin{tikzpicture}
  \SetGraphUnit{4}  
  \Vertex{a}
  \EA(a){b}
  \NO(b){c}
  \SetUpEdge[style={->,bend right,ultra thick},
             color=red]
  \Edge(a)(b)
  \Edge(b)(c)
  \Edge(c)(a)
\end{tikzpicture}
\end{tkzexample}  

\newpage 
\subsection{Modification des styles par défaut \tkzcname{SetUpEdge}} 

Cette macro a une action globale et permet de rédéfinir un style.

\begin{NewMacroBox}{SetUpEdge}{\oarg{local options}}
\begin{tabular}{llc}
Options         & Défaut  & Définition                       \\ 
\midrule
\TOline{lw}   {-90  }   {position label externe      } 
\TOline{color}{\textbackslash EdgeLineWidth}   {position label externe      }     
\TOline{label}   {0cm  }   {distance du label           }     
\TOline{labelstyle}   {{}   }   {permet d'affiner le style   }     
\TOline{labeltext} {false}   {supprime le label           }     
\TOline{style}{false}   {Label externe               }      \bottomrule
\end{tabular}

\medskip
\emph{Cette macro permet de modifier les options précédentes. }
\end{NewMacroBox}


\subsubsection{Utilisation de \tkzcname{SetUpEdge} Exemple 1} 
\begin{center}
{   \tikzset{VertexStyle/.style = {shape         = circle,
                                   draw          = black,
                                   fill          = orange,
                                   inner sep     = 2pt,
                                   outer sep     = 0.5pt,
                                   minimum size  = 6mm,
                                   line width    = 1pt}}
     \tikzset{every to/.style = {line width    = 2pt,
                                   color        = orange}}  
\begin{tkzexample}[vbox]
 \begin{tikzpicture} 
     \SetGraphUnit{4}     \SetUpEdge[lw=3pt]
     \Vertex{A}
     \EA (A){B}     \NO (B){C}
     \SO (B){D}     \EA (B){E}
     \Edges(A,B,C,A,D,E,C)
   \end{tikzpicture}
\end{tkzexample}
}
\end{center}


\subsubsection{Utilisation de \tkzcname{SetUpEdge} Exemple 2} 
{ \tikzset{VertexStyle/.style = { 
           shape        = circle,
           draw         = black,
           fill         = orange,
           inner sep    = 2pt,
           outer sep    = 1pt,
           minimum size = 6mm,
           line width   = 2pt}}   
\begin{tkzexample}[latex=7cm]
\begin{tikzpicture}
    \SetGraphUnit{3}
    \SetUpEdge[lw=1.5pt]
    \Vertex{A}
    \EA(A){B}   \WE(A){C}   \NO(A){D}
    \SO(A){E}   \NOEA(A){F} \NOWE(A){G} 
    \SOEA(A){H} \SOWE(A){I}
    \foreach \v in {B,C,D,E,F,G,H,I}{%
      \Edge(A)(\v)};
 \end{tikzpicture} 
\end{tkzexample} } 

\subsection{Arête avec label  \tkzname{LabelStyle}}


\begin{tkzexample}[latex=7cm, small]
\begin{tikzpicture}
 \SetGraphUnit{4}  
 \tikzset{VertexStyle/.style = 
  {draw,
   shape           = circle,
   shading         = ball,
   ball color      = green!40!black,
   minimum size    = 24pt,
   color           = white}}
  \tikzset{EdgeStyle/.style   =
   {->,bend right,
    thick,
    double          = orange,
    double distance = 1pt}}
  \Vertex{a}
  \EA(a){b}
  \NO(b){c}
  \tikzset{LabelStyle/.style =
   {fill=white}}
  \Edge[label=$1$](a)(b)
  \Edge[label=$2$](b)(c)
  \Edge[label=$3$](c)(a)
\end{tikzpicture}
\end{tkzexample}


\subsection{Utiliser un style intermédiaire}
 
\begin{tkzltxexample}[]
  \SetGraphUnit{4}
  \tikzset{VertexStyle/.style   = {shape           = circle,
                                   shading         = ball,
                                   ball color      = Maroon!50,
                                   minimum size    = 24pt,
                                   draw}}
  \tikzset{TempEdgeStyle/.style = {ultra thick,
                                   double          = Maroon!50,
                                   double distance = 2pt}}
  \tikzset{LabelStyle/.style    = {color           = brown,
                                   text=black}} 
\end{tkzltxexample} 


\begin{center}
   \SetGraphUnit{4}
  \tikzset{VertexStyle/.style   = {shape           = circle,
                                   shading         = ball,
                                   ball color      = Maroon!50,
                                   minimum size    = 24pt,
                                   draw}}
  \tikzset{TempEdgeStyle/.style = {ultra thick,
                                   double          = Maroon!50,
                                   double distance = 2pt}}
  \tikzset{LabelStyle/.style    = {color           = brown,
                                   text=black}} 
\begin{tkzexample}[latex=7cm, small] 
\begin{tikzpicture}[scale=.8]
  \Vertex{A}
  \EA(A){B}  \EA(B){C}
  \SetGraphUnit{8}  
  \NO(B){D}   
  \tikzset{EdgeStyle/.style = {TempEdgeStyle}} 
  \Edge[label=1](B)(D)
  \tikzset{EdgeStyle/.style = {TempEdgeStyle,bend left}}
  \Edge[label=4](A)(B)  \Edge[label=5](B)(A)
  \Edge[label=6](B)(C)  \Edge[label=7](C)(B)
  \Edge[label=2](A)(D)  \Edge[label=3](D)(C)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\vfill\newpage

\section{Changement de couleurs dans les styles prédéfinis}
Trois macros sont proposées 

\subsection{\tkzcname{SetGraphShadeColor}}
\begin{NewMacroBox}{SetGraphShadeColor}{\var{ball color}\var{color}\var{double}}
\emph{\tkzcname{SetGraphShadeColor} permet de modifier les couleurs pour le style \tkzname{Shade}.}
\end{NewMacroBox}

\subsubsection{Exemple}
Cet exemmple utilise une macrio de \tkzname{tkz-berge}\NamePack{tkz-berge} 
\begin{center}
\begin{tkzexample}[latex=7cm]
	\begin{tikzpicture}
	   \GraphInit[vstyle=Shade]
	   \SetGraphUnit{4} 
	   \SetVertexNoLabel 
	   \SetGraphShadeColor{red!50}{black}{red} 
     \Vertices{circle}{A,B,C,D,E} 
     \Edges(A,B,C,D,E,A,C,E,B,D)
	\end{tikzpicture}
\end{tkzexample}

\end{center}  

\newpage
\subsection{\tkzcname{SetGraphArtColor}} 
\begin{NewMacroBox}{SetGraphArtColor}{\var{ball color}\var{color}}
\emph{\tkzcname{SetGraphArtColor} permet de modifier les couleurs pour le style \tkzname{Art}.}
\end{NewMacroBox}

\subsubsection{Exemple} 
\begin{center}
	\begin{tkzexample}[vbox]
	\begin{tikzpicture}
	    \SetVertexArt
	    \SetGraphArtColor{green!40!black}{magenta}
		  \SetGraphUnit{4} 
		  \SetVertexNoLabel 
	    \Vertices{circle}{A,B,C,D,E} 
	    \Edges(A,B,C,D,E,A,C,E,B,D)
	\end{tikzpicture}  
	\end{tkzexample} 
\end{center}
 

\vfill\newpage  
\subsection{\tkzcname{SetGraphColor}}
\begin{NewMacroBox}{SetGraphColor}{\var{fill color}\var{color}}
\emph{\tkzcname{SetGraphColor} permet de modifier les couleurs pour le style \tkzname{Normal}.}
\end{NewMacroBox}
 

\subsubsection{Exemple avec \tkzcname{SetGraphColor}} 
\begin{center}
	\begin{tkzexample}[vbox]
	\begin{tikzpicture}
	    \SetGraphColor{yellow}{blue}{maagenta}
		  \SetGraphUnit{4} 
		  \SetVertexNoLabel 
	    \Vertices{circle}{A,B,C,D,E} 
	    \Edges(A,B,C,D,E,A,C,E,B,D)   
	\end{tikzpicture} 
	\end{tkzexample}
\end{center}
 


\newpage

\subsection{Variation I autour des styles}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetVertexNormal[Shape      = circle,
                   FillColor  = orange,
                   LineWidth  = 2pt]
  \SetUpEdge[lw         = 1.5pt,
             color      = black,
             labelcolor = white,
             labeltext  = red,
             labelstyle = {sloped,draw,text=blue}]
   \Vertex[x=0 ,y=0]{K}
   \Vertex[x=0 ,y=2]{F}
   \Vertex[x=-1,y=4]{D}
   \Vertex[x=3 ,y=7]{H}
   \Vertex[x=8 ,y=5]{B}
   \Vertex[x=9 ,y=2]{N}
   \Vertex[x=5 ,y=0]{M}
   \Vertex[x=3 ,y=1]{S}
   \tikzset{EdgeStyle/.append style = {bend left}}
   \Edge[label = $120$](K)(F)
   \Edge[label = $650$](H)(S)
   \Edge[label = $780$](H)(M)
   \Edge[label = $490$](D)(B)
   \Edge[label = $600$](D)(M)
   \Edge[label = $580$](B)(M)
   \Edge[label = $600$](H)(N)
   \Edge[label = $490$](F)(H)
   \tikzset{EdgeStyle/.append style = {bend right}}
   \Edge[label = $630$](S)(B)
   \Edge[label = $210$](S)(N)
   \Edge[label = $230$](S)(M)
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsection{Variation II autour des styles} 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
  \SetVertexNormal[Shape      = circle,
                   FillColor  = orange,
                   LineWidth  = 2pt]
  \SetUpEdge[lw         = 1.5pt,
             color      = black,
             labelcolor = white,
             labeltext  = red,
             labelstyle = {sloped,draw,text=blue}]
 \tikzstyle{EdgeStyle}=[bend left]
 \Vertex[x=0, y=0]{G}
 \Vertex[x=0, y=3]{A} 
 \Vertex[x=3, y=5]{P}
 \Vertex[x=4, y=2]{C}
 \Vertex[x=8, y=3]{Q}
 \Vertex[x=7, y=0]{E}
 \Vertex[x=3, y=-1]{R}
 \Edges(G,A,P,Q,E) \Edges(C,A,Q) \Edges(C,R,G) \Edges(P,E,A)
\end{tikzpicture}
\end{tkzexample} 
\end{center}

\subsection{Variation III autour des styles} 

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture} 
  \GraphInit[vstyle=Shade]
  \SetGraphUnit{3}
  \Vertex{e}
  \NOEA(e){f}\SOEA(e){d}
  \SOEA(f){h}\NOWE(f){g}    
  \WE(g){c}  \SOWE(e){a}  \SOWE(c){b}
  \tikzstyle{LabelStyle}=[fill=white]
  \tikzstyle{EdgeStyle}=[color=red]
  \Edge[label=$3$](a)(b)
  \Edge[label=$11$](a)(c)
  \Edge[label=$6$](a)(e)
  \Edge[label=$17$](a)(d)
  \Edge[style={pos=.25},label=$20$](a)(g)
  \Edge[label=$5$](c)(b)
  \Edge[label=$6$](c)(e)
  \Edge[label=$7$](c)(g)
  \Edge[label=$7$](f)(e)
  \Edge[label=$3$](d)(e)
  \Edge[label=$9$](d)(h)
  \Edge[label=$6$](g)(e)
  \Edge[style={bend left,out=45,in=135},label=$11$](g)(h)
  \Edge[label=$4$](f)(h)    
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{Variation IV autour des styles}

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}
 \SetUpEdge[lw         = 1.5pt,
            color      = orange,
            labelcolor = gray!30,
            labelstyle = {draw}]
     \SetGraphUnit{3}   
  \GraphInit[vstyle=Normal]
  \Vertex{P}
  \NOEA(P){B}
  \SOEA(P){M} 
  \NOEA(B){D}
  \SOEA(B){C}
  \SOEA(C){L} 
  \tikzset{EdgeStyle/.style={->}}
  \Edge[label=$3$](C)(B)
  \Edge[label=$10$](D)(B)
  \Edge[label=$10$](L)(M)
  \Edge[label=$10$](B)(P)
  \tikzset{EdgeStyle/.style={<->}}
  \Edge[label=$4$](P)(M)
  \Edge[label=$9$](C)(M)
  \Edge[label=$4$](C)(L)
  \Edge[label=$5$](C)(D)
  \Edge[label=$10$](B)(M)
  \tikzset{EdgeStyle/.style={<->,relative=false,in=0,out=60}}
  \Edge[label=$11$](L)(D)
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{Variation V autour des styles}  

\begin{center}
\begin{tkzexample}[vbox]
\begin{tikzpicture}

 \SetUpEdge[lw         = 1.5pt,
            color      = orange,
            labelcolor = white]   
  \GraphInit[vstyle=Normal] \SetGraphUnit{3} 
  \tikzset{VertexStyle/.append  style={fill    = red!50}}
  \Vertex{P}
  \NOEA(P){B}  \SOEA(P){M} \NOEA(B){D}
  \SOEA(B){C}  \SOEA(C){L} 
  \tikzset{EdgeStyle/.style={->}}
  \Edge[label=$3$](C)(B)
  \Edge[label=$10$](D)(B)
  \Edge[label=$10$](L)(M)
  \Edge[label=$10$](B)(P)
  \tikzset{EdgeStyle/.style={<->}}
  \Edge[label=$4$](P)(M)
  \Edge[label=$9$](C)(M)
  \Edge[label=$4$](C)(L)
  \Edge[label=$5$](C)(D)
  \Edge[label=$10$](B)(M)
  \tikzset{EdgeStyle/.style={<->,relative=false,in=0,out=60}}
  \Edge[label=$11$](L)(D)
\end{tikzpicture}
\end{tkzexample}
\end{center}
\endinput


==> tkz-graph/doc/latex/TKZdoc-gr-vertex.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex

% $Id$
\section{Vertex}
% The ( < name >) is a name for later reference and it is optional. You may also add the option name=< name > 
% to the < option > list; it has the same eﬀect.
%<------------------------------------------------------------------------–> 
C'est bien évidemment la macro essentielle qui permet de placer des sommets. Les sommets peuvent être placés avec un système de coordonnées rectangulaires ou bien polaires ou encore relativement les uns par rapport aux autres. Quelques dispositions particulières sont également possibles.

\subsection{\tkzcname{Vertex}}
\begin{NewMacroBox}{Vertex}{\oarg{local options}\var{Name}}
Un sommet se caractérise par~:
\begin{itemize}
\item   sa référence,
\item   sa position,
\item   son label,
\item   et le style.
\end{itemize}

\medskip
Un argument non vide \IargName{Vertex}{Name} est obligatoire. Cet argument définit le nom de référence du  node. C'est celui que l'on doit utiliser dans toute création de sommet (\tkzcname{Vertex}) Il ne faut pas le confondre avec  le \tkzname{label} (étiquette) qui sera utilisé pour l'affichage.
On peut vouloir afficher $M_1$ alors que le nom lui sera $M1$.

\medskip
Des options sont utilisées pour définir les quatre premières caractéristiques. Les styles texte et graphique sont traités séparément.  

\medskip
\begin{tabular}{llc}
\midrule
Options   & Défaut  & Définition              \\
\midrule
\TOline{x}        {\{\}}{abscisse}  
\TOline{y}        {\{\}}{ordonnée}   
\TOline{a}        {\{\}}{angle}     
\TOline{d}        {\{\}}{distance}   
\TOline{Node}     {false}{utilisation d'une référence déjà définie}   
\TOline{position} {\{\}}{style qui permet un positionnement relatif }   
\TOline{dir} {\textbackslash EA}{direction pour un positionnement relatif }   
\midrule 
\TOline{empty}    {false}{booléen permettant de ne pas afficher le sommet}   
\midrule 
\TOline{NoLabel} {false}{booléen supprime le label}  
\TOline{LabelOut}{false}{booléen Label extérieur au node}  
\TOline{L}       {\{\}}{Le label}  
\TOline{Math}     {false}{booléen qui affiche le label en mode math} 
\TOline{Ldist}   {0cm  }{distance du label au node} 
\TOline{Lpos}    {0    }{position du label par rapport au node} 
\bottomrule
\end{tabular}

\medskip
\emph{Cette macro permet de définir un sommet qui a un nom \tkzname{name} et un label.\\
Si \tkzname{L}$=${} alors \tkzname{label} = \tkzname{Name} sinon \tkzname{label} = \tkzname{L}.}
\end{NewMacroBox}

\subsubsection{Utilisation de coordonnées cartésiennes} 
\tkzcname{Vertex[x=\meta{number},y=\meta{number}]\var{name}}.  Coordonnées cartésiennes $x$ et $y$.

\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \GraphInit[vstyle=Normal]
   \draw[help lines] (0,0) grid (2,2);
   \Vertex{A} % par défaut x = 0 et y = 0
   \Vertex[x=2 , y=0]{B} \Vertex[x=2 , y=2]{C}
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Utilisation de coordonnées polaires} 

 \tkzcname{Vertex[a=\meta{number},d=\meta{number}]\var{vertex}} Les coordonnées polaires peuvent être aussi utilisées. J'ai utilisé une grille d'aide afin de constater le placement du sommet. 


\begin{tkzexample}[latex=7cm,small] 
\begin{tikzpicture}
   \GraphInit[vstyle=Normal]
   \draw[help lines] (-2,0) grid (2,2);
   \draw[red] (2,0) arc (0:180: 2 cm);
   \Vertex{A}
   \Vertex[a=45 , d=2 cm]{B}
   \Vertex[a=135 , d=2 cm]{C}
\end{tikzpicture}
\end{tkzexample} 
 


 

\subsubsection{Option \tkzname{Node} : utilisation d'une position référencée} 
Cette option permet de placer un sommet sur un Node déjà défini ou bien
 un objet du type \og~coordinate~\fg.
   % pb taile du node pour M ??
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \GraphInit[vstyle=Normal]
   \draw[help lines] (0,0) grid (2,2);
   \Vertex{A} \Vertex[x=2 , y=2]{B}
   %\tkzActivOff  nécessaire avec frenchb et babel
   \tkzActivOff 
   \coordinate (M) at ($ (A)!.5!(B) $){};
   \tkzActivOn
   \Vertex[Node]{M}
\end{tikzpicture}
\end{tkzexample}

\vfill
%<------------------------------------------------------------------------–>
%                             ShortCuts
%<------------------------------------------------------------------------–>

\newpage
\subsection{Raccourcis pour placement relatif}

Pour effectuer des placements relatifs, il est nécessaire de définir une distance unité entre deux sommets. La macro suivante permet de définir cette distance.

\begin{NewMacroBox}{SetGraphUnit}{\var{nombre}}
\emph{Cette macro permet de définir la distance entre deux sommets. La distance se réfère aux centres de ces sommets et le nombre est exprimé en \tkzname{cm}. Par défaut, l'unité est $1$ cm.}

utilisation :\tkzcname{SetGraphUnit\{2\}} 
\end{NewMacroBox}

\begin{NewMacroBox}{ShortCut}{\oarg{local options}\varp{vertex A}\var{vertex B}}
Ces raccourcis permettent de créer un \tkzname{vertex B}  relativement à un 
\tkzname{vertex A}. La distance entre les deux sommets est déterminé par  la valeur de \tkzname{unit} et par les unités de \TIKZ. Horizontalement et verticalement la distance est définie par \tkzname{unit}$\times$\tkzname{x} et 
\tkzname{unit}$\times$\tkzname{y}. La valeur de \tkzname{unit} peut être redéfinie par la macro  \tkzcname{SetGraphUnit} ou bien avec l'option \tkzname{unit}. Avec l'option la définition est locale; avec la macro, la définition est globale mais elle peut être locale si elle est intervient dans un goupe \TEX ou un environnement \tkzname{scope}.
Les raccourcis sont :

\medskip
\begin{tabular}{lll}
\hline
Raccourcis   &   & Définition              \\
\midrule
\TMline{EA}    {}  {à l'est }        
\TMline{WE}    {}  {à l'ouest}         
\TMline{NO}    {}  {au nord}        
\TMline{SO}    {}  {au sud}        
\TMline{NOEA}  {}  {au nord-est soit "nord" puis "est"}  
\TMline{NOWE}  {}  {au nord-ouest soit "nord" puis "ouest" }   
\TMline{SOEA}  {}  {au sud-est soit "sud" puis "est"}  
\TMline{SOWE}  {}  {au sud-ouest soit "sud" puis "ouest"}   
\bottomrule
\end{tabular}

\medskip
\emph{\tkzcname{NOEA} est un raccourci pour \tkzcname{NO}\tkzcname{EA}. par défaut, la distance entre les sommets avec ce raccourci est $\sqrt{2}\times$ \tkzname{unit}=$\sqrt{2}$. Les options sont celles de la macro \tkzcname{Vertex}. }
\end{NewMacroBox} 

Nous allons d'abord modifier la distance entre deux noeuds d'une façon générale avec \tkzcname{SetGraphUnit\{2\}} sinon par défaut \tkzname{unit =1}. 

\subsubsection{Utilisation des raccourcis avec les valeurs par défaut} 
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \draw[help lines] (-1,-1) grid (1,1);
   \GraphInit[vstyle=Normal]
   \Vertex{A}
   \EA(A){B}   \WE(A){C}   \NO(A){D}   \SO(A){E}
   \NOEA(A){F} \NOWE(A){G} \SOEA(A){H} \SOWE(A){I}
   \foreach \v in {B,C,D,E,F,G,H,I}{\Edge(A)(\v)};
\end{tikzpicture}
\end{tkzexample} 


\subsubsection{Modification de l'unité avec  \tkzcname{SetGraphUnit }} 
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \draw[help lines] (-2,-2) grid (2,2);      
   \SetGraphUnit{2}
   \GraphInit[vstyle=Normal]
   \Vertex{A}
   \EA(A){B}   \WE(A){C}   \NO(A){D}   \SO(A){E}
   \NOEA(A){F} \NOWE(A){G} \SOEA(A){H} \SOWE(A){I}
   \foreach \v in {B,C,D,E,F,G,H,I}{\Edge(A)(\v)};
\end{tikzpicture}
\end{tkzexample} 

\subsubsection{Modification des unités de \TIKZ\ : \tkzname{x=2 cm,y=1 cm} } 
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}[x=2 cm,y=1 cm]
   \draw[help lines] (-1,-1) grid (1,1);      
   \GraphInit[vstyle=Normal]
   \Vertex{A}
   \EA(A){B}   \WE(A){C}   \NO(A){D}   \SO(A){E}
   \NOEA(A){F} \NOWE(A){G} \SOEA(A){H} \SOWE(A){I}
   \foreach \v in {B,C,D,E,F,G,H,I}{\Edge(A)(\v)};
\end{tikzpicture}
\end{tkzexample} 


\subsubsection{Exemple classique} 
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \draw[help lines] (-2,-2) grid (4,2);     
  \SetGraphUnit{2}
  \coordinate (O) at (0,0);
  \NOEA(O){A} \NOWE(O){B} \SOEA(O){D} 
  \SOWE(O){C} \NOEA(D){E}
  \Edges(B,C,D,A,E,D,B,A,C)
\end{tikzpicture}
\end{tkzexample}

\subsubsection{Autre exemple classique}   
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \draw[help lines] (0,-2) grid (4,2);
   \SetGraphUnit{2}
   \GraphInit[vstyle=Normal]
   \Vertex{A}
   \EA(A){B} \NO(B){C} \SO(B){D} \EA(B){E}
   \Edges(A,B,C,A,D,E,C)
\end{tikzpicture}
\end{tkzexample}


\subsubsection{Modication locale de \tkzname{unit} avec l'option}
Le plus simple  :
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,3);
  \SetGraphUnit{2}
  \Vertex{A}  \EA(A){B} 
  \NO[unit=3](B){C}
  \NO(A){D}
\end{tikzpicture}
\end{tkzexample} 


\subsubsection{Modication locale de \tkzname{unit} avec l'environnement \tkzname{scope}}
\begin{tkzexample}[latex=7cm,small]   
 \begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,3);
  \SetGraphUnit{2}
  \Vertex{A}  \EA(A){B} 
 \begin{scope}
    \SetGraphUnit{3} \NO(B){C}
 \end{scope}
 \NO(A){D}
\end{tikzpicture}
\end{tkzexample}     

\subsubsection{Modication locale de \tkzname{unit} avec un groupe \TEX}
\begin{tkzexample}[latex=7cm,small]   
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,3);
  \SetGraphUnit{2}
  \Vertex{A}  \EA(A){B} 
 {\SetGraphUnit{3} \NO(B){C}}
 \NO(A){D}
\end{tikzpicture}
\end{tkzexample} 

\endinput



==> tkz-graph/doc/latex/TKZdoc-gr-vertices.tex <==
%!TEX root = /Users/ego/Boulot/TKZ/tkz-graph/doc-fr/TKZdoc-gr-main.tex
% $Id$

%<--------------------------------------------------------------------------->
%                             Vertices
%<--------------------------------------------------------------------------->

\section{Placement de sommets sur une forme géométrique}
Il s'agit ici de placer un groupe de sommets suivant une direction donnée ou bien encore suivant une forme prédéfinie. Les sommets sont placés avec comme support une figure géométrique simple. La macro principale utilise une direction  définie à l'aide de l'option dir, la version étoilée une forme particulière triangulaire, carrée etc...   


\begin{NewMacroBox}{Vertices}{\oarg{local options}\var{type}\var{List of vertices}}
\emph{Il y a donc plusieurs types de formes géométriques, droite, triangle, carrés et cercles. La macro \tkzcname{SetGraphUnit} permet de modifier les  longueurs. Pour les sommets alignés, ceux-ci sont placés suivant une direction donnée par |EA|, |WE|, |NO|, |SO|, |NOEA|, |NOWE|, |SOEA|, |SOWE|.} 

\medskip
\begin{tabular}{llc}
 \toprule
Premier Argument   &            & Définition            \\
\midrule 
\TAline{line  } {} {Sommets alignés, une option détermine la direction} 
\TAline{tr1   } {} {première forme de triangle}   
\TAline{tr2   } {} {deuxième forme de triangle}  
\TAline{tr3   } {} {troisième forme de triangle}  
\TAline{tr4   } {} {quatrième forme de triangle}  
\TAline{square} {} {quatre sommets sur un carré}  
\TAline{circle} {} {sommets sur une cercle}  
\bottomrule
\end{tabular}

\medskip    
\emph{Le second argument est une liste de noms pour les sommets.} 

\medskip    
\begin{tabular}{llc}
\midrule
Options   & Défaut  &      Définition  \\
\midrule
\TOline{dir}  {EA} {permet de placer plusieurs sommets alignés} 
\bottomrule
\end{tabular}

\medskip    
\emph{Les options  sont celles d'un sommet (Vertex).} 
\end{NewMacroBox}    
 

                                                                    
\subsection{\tkzcname{Vertices} à partir d'un sommet défini par des coordonnnées}                 
  
                                                                   
\begin{center}                                                     
\begin{tkzexample}[latex=7cm, ,small]                              
\begin{tikzpicture}
    \SetGraphUnit{2}                       
   \draw[help lines] (0,0) grid (5,2);
   \Vertices[x=1,y=2]{line}{A,B,C}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{\tkzcname{Vertices} à partir d'une position donnée.}

\begin{center}                                                     
\begin{tkzexample}[latex=7cm, ,small] 
\begin{tikzpicture}[rotate=45] 
  \SetGraphUnit{2}
   \draw[help lines] (0,0) grid (5,2);
   \coordinate (A) at (1,1); 
   \Vertices[Node]{line}{A,B,C}
\end{tikzpicture}
\end{tkzexample}
\end{center}

\subsection{Exemples avec une direction } 
 Il s'agit ici de placer une liste de sommets suivant une direction donnée, cette direction est définie à l'aide de l'option \tkzname{dir}.  


\begin{center}
\begin{tkzexample}[latex=7cm, ,small]  
\begin{tikzpicture}
  \GraphInit[vstyle=Art]
  \Vertices[dir=\NOEA]{line}{A,B,C,D}
  \Vertices[dir=\NOWE]{line}{A,E,F,G}
\end{tikzpicture}
\end{tkzexample}
\end{center} 
              

\subsection{Placement sur un triangle }

Il y a différentes possibilités avec une forme triangulaire, mais les triangles sont isocèles rectangles. Voici dans l'ordre les formes \tkzname{tr1}, \tkzname{tr2} , \tkzname{tr3} et \tkzname{tr4}


\begin{tkzexample}[latex=8cm,small]  
\begin{tikzpicture}\SetGraphUnit{2}
     \Vertices{tr1}{A,B,C}
\end{tikzpicture}\hspace*{2cm}
\begin{tikzpicture}\SetGraphUnit{2}
     \Vertices{tr2}{A,B,C}
\end{tikzpicture}
\end{tkzexample}

\begin{tkzexample}[latex=8cm,small]  
\begin{tikzpicture}\SetGraphUnit{2}
     \Vertices{tr3}{A,B,C}
\end{tikzpicture}\hspace*{2cm}
\begin{tikzpicture}\SetGraphUnit{2}
     \Vertices{tr4}{A,B,C}
\end{tikzpicture}
\end{tkzexample}  


\subsection{Utilisation d'un carré}

 
Deux autres possibilités de placer un node. La première utilise un node obtenu à l'aide d'une intersection (voir le pgfmanual). Dans la première, j'ai redéfini la distance unité entre deux sommets à l'aide de   \tkzcname{SetGraphUnit}.

\begin{center}
\begin{tkzexample}[latex=7cm,small]
\begin{tikzpicture}
   \SetGraphUnit{3}
   \GraphInit[vstyle=Shade]
   \Vertices{square}{A,B,C,D}
   \coordinate (E) at (intersection of A--C and B--D);
   \Vertex[Node]{E}% voir option node
\end{tikzpicture}
\end{tkzexample}
\end{center}


\subsection{Utilisation d'un cercle }

\begin{tkzexample}[latex=7cm,small]  
\begin{tikzpicture}
  \SetGraphUnit{2}
  \Vertices{circle}{A,B,C,D}
\end{tikzpicture}
\end{tkzexample} 


\subsection{Utilisation d'un cercle  et positionnement des labels }

\begin{tkzexample}[latex=7cm,small]   
\begin{tikzpicture} \SetGraphUnit{2}
  \GraphInit[vstyle=Classic]
  \Vertices{circle}{A,B,C,D,E,F}
\end{tikzpicture}
\end{tkzexample}



\subsection{Rotation  et labels externes }

|Lpos| = \tkzname{angle de la rotation}. Cela permet de faire une rotation du label autour du centre de chaque sommet et de suivre la rotation du graphe. Il suffit pour comprendre cette option de compiler l'exemple en l'omettant.  


\begin{tkzexample}[latex=7cm,small] 
\begin{tikzpicture}[rotate=90]
  \GraphInit[vstyle=Classic]
  \Vertices[Lpos=90,unit=2]{circle}{A,B,C,D,E,F}
\end{tikzpicture}
\end{tkzexample}


\subsection{Placement sur un cercle }

Avec des labels externes, il faut procéder avec précaution. 

\begin{tkzexample}[latex=7cm,small] 
\begin{tikzpicture}[scale=.5]
 \SetGraphUnit{4}
 \GraphInit[vstyle=Classic] 
 \begin{scope}[rotate=45] 
   \Vertices[Lpos=45]{circle}{C,E,A,B} 
 \end{scope} 
 \NOEA[Lpos=90,unit=2.828](E){D} 
 \Edges(A,B,E,D,C,E,A,C,B) 
\end{tikzpicture}
\end{tkzexample}

  

\endinput

